Rigidity-Aware Detection for 6D Object Pose Estimation

Most recent 6D object pose estimation methods first use object detection to obtain 2D bounding boxes before actually regressing the pose. However, the general object detection methods they use are ill-suited to handle cluttered scenes, thus producing poor initialization to the subsequent pose network. To address this, we propose a rigidity-aware detection method exploiting the fact that, in 6D pose estimation, the target objects are rigid. This lets us introduce an approach to sampling positive object regions from the entire visible object area during training, instead of naively drawing samples from the bounding box center where the object might be occluded. As such, every visible object part can contribute to the final bounding box prediction, yielding better detection robustness. Key to the success of our approach is a visibility map, which we propose to build using a minimum barrier distance between every pixel in the bounding box and the box boundary. Our results on seven challenging 6D pose estimation datasets evidence that our method outperforms general detection frameworks by a large margin. Furthermore, combined with a pose regression network, we obtain state-of-the-art pose estimation results on the challenging BOP benchmark.

==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/compare_atss_ours.tex <==

\begin{tabular}{ccccccl}
%   \multicolumn{2}{c}{Activated cells}  & Results \\
%   \includegraphics[width=0.15\linewidth]{figures/compare_atss_ours/obj1_cropped.png} & 
%   \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj1_atss_foreground_modeling.pdf} &
%   \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj1_distancemap.png} &
  \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj1_atss_activated_cells.pdf} &
  \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj1_ours_activated_cells.pdf} &
  \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj1_detection_results.jpg} \\
%   \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj2_cropped.png} &
%   \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj2_atss_foreground_modeling.pdf} &
%   \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj2_distancemap.png} &
  \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj2_atss_activated_cells.pdf} &
  \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj2_ours_activated_cells.pdf} &
  \includegraphics[width=0.15\textwidth]{figures/compare_atss_ours/obj2_detection_results.jpg} \\
  {\small (a) Baseline strategy} & {\small (b) Our strategy} & {\small (c) Detection results}\\
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/distance_map.tex <==
\begin{tabular}{ccc}
    \includegraphics[width=0.32\linewidth]{figures/distance_map/seeds.pdf} &
    \includegraphics[width=0.32\linewidth]{figures/distance_map/growing.pdf} &
    \includegraphics[width=0.32\linewidth]{figures/distance_map/distance_map.pdf} \\
    {\small (a) Initial seeds} & {\small (b) Seeds growing} & {\small (c) Distance map} \\
\end{tabular}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/distancemap_cases.tex <==
\setlength\tabcolsep{0.5pt}
% \begin{tabular}{cccc}
%     \includegraphics[width=0.25\linewidth, trim=70 125 240 25, clip]{figures/distancemap_cases/000022.png} & 
%     \includegraphics[width=0.25\linewidth, trim=200 300 260 0, clip]{figures/distancemap_cases/000047.png} & 
%     \includegraphics[width=0.25\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000065.png} & 
%     \includegraphics[width=0.25\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000075.png}\\
%     \includegraphics[width=0.25\linewidth, trim=70 125 240 25, clip]{figures/distancemap_cases/000054_000022_2_fuse.png} & 
%     \includegraphics[width=0.25\linewidth, trim=200 300 260 0, clip]{figures/distancemap_cases/000048_000047_2_fuse.png} &
%     \includegraphics[width=0.25\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000049_000065_3_fuse.png} &
%     \includegraphics[width=0.25\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000053_000075_1_fuse.png}\\
%     \multicolumn{2}{c}{\small (a) Simple cases} & \multicolumn{2}{c}{\small (b) Hard cases} & ~\\
% \end{tabular}

\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000065.png} & 
    \includegraphics[width=0.24\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000049_000065_3_fuse.png} &
    \includegraphics[width=0.24\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000075.png} &
    \includegraphics[width=0.24\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000053_000075_1_fuse.png} &
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/fusion.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{2pt}
    \begin{tabular}{cccl}
      \includegraphics[width=0.3\linewidth, clip, trim=150 0 35 0]{figures/fusion/activate_cells.jpg} &
      \includegraphics[width=0.3\linewidth, clip, trim=150 0 35 0]{figures/fusion/cluster.jpg} &
      \includegraphics[width=0.3\linewidth]{figures/fusion/vote.png} &
      \hspace{-2mm}
      \includegraphics[width=0.05\linewidth]{figures/fusion/colormap.pdf}
    \end{tabular}
    \caption{{\bf Combining multiple candidates.} 
          {\bf (a)} During inference, multiple cells of the network will be activated thanks to the proposed mask-based sampling strategy during training. 
          Each network cell will generate one box prediction. Here we visualize the cells by different colors according to the confidence of their corresponding box predictions. Note that the cells with the most confident prediction do not come from the center region here, but from some cells with the most discriminative textures.
          {\bf (b)} With multiple detection candidates from each local cell, we cluster them according to some simple distance threshold to correspond them to different instances.
          {\bf (c)} After a simple fusion of multiple candidate results, we can obtain a single robust result.}
    \label{fig:fusion}
  \end{figure}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/more_visualization.tex <==
\begin{tabular}{cccc}
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000494.jpg} &  
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000521.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000560.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000785.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000494.jpg} &  
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000521.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000560.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000785.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000016_000381.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000018_000246.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000020_000094.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000020_000174.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000016_000381.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000018_000246.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000020_000094.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000020_000174.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000001_000036.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000001_000015.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000003_000014.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000003_000057.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000001_000036.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000001_000015.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000003_000014.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000003_000057.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000053_000103.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000054_000032.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000055_000618.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000056_00075.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000053_000103.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000054_000032.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000055_000618.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000056_000075.jpg} \\ 
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/motiv_old.tex <==

\setlength\tabcolsep{1pt}
\begin{tabular}{ccccc}
  \includegraphics[width=0.24\linewidth, clip, trim=100 0 700 400]{figures/motiv_old/atss_assign_update.jpg} &
  % \hspace{-1.5mm}
  \includegraphics[width=0.24\linewidth, clip, trim=100 0 700 400]{figures/motiv_old/000084_cluster_atss_update.jpg}&
  % \hspace{1mm}
  \includegraphics[width=0.24\linewidth, clip, trim=100 0 700 400]{figures/motiv_old/ours_assign_update.jpg} &
  % \hspace{-1.5mm}
  \includegraphics[width=0.24\linewidth, clip, trim=100 0 700 400]{figures/motiv_old/000084_cluster_ours_update.jpg} &
  \includegraphics[width=0.017\linewidth]{figures/fusion/colormap.pdf} \\
%   % \hspace{mm}
%   \raisebox{-0.5\height}[0pt][0pt]{
%     \includegraphics[width=0.07\linewidth]{figures/fusion/colormap.pdf}
%   }\\
%   \includegraphics[width=0.22\linewidth, clip, trim=350 420 1420 300]{figures/motiv_old/frankfurt_000001_067178_atss_assign.png} &
%   \hspace{-2mm}
%   \includegraphics[width=0.22\linewidth, clip, trim=350 420 1420 300]{figures/motiv_old/frankfurt_000001_067178_atss.jpg} &
%   \hspace{1mm}
%   \includegraphics[width=0.22\linewidth, clip, trim=350 420 1420 300]{figures/motiv_old/frankfurt_000001_067178_ours_assign.png} &
%   \hspace{-2mm}
%   \includegraphics[width=0.22\linewidth, clip, trim=350 420 1420 300]{figures/motiv_old/frankfurt_000001_067178_mask.jpg} \\
  \multicolumn{2}{c}{\small (a) The standard strategy} & \multicolumn{2}{c}{\small (b) The proposed strategy} & ~\\
\end{tabular}



==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/motivation.tex <==
\begin{tabular}{ccc}
        % \includegraphics[width=0.45\linewidth, clip, trim=0 5 0 10]{figures/motivation/coco_occlusion.jpg} &
        \includegraphics[width=0.45\linewidth, clip, trim=60 0 20 0]{figures/motivation/coco_noocclusion.jpg} &
        \includegraphics[width=0.45\linewidth, clip, trim=250 260 100 80]{figures/motivation/6dpose_occlusion.jpg} \\
        {\small (a) General detection} & {\small (b) Detection in 6D pose} \\
        \includegraphics[width=0.45\linewidth, clip, trim=250 200 100 80]{figures/motivation/general_detection_case2_fcos.jpg} &  
        % \includegraphics[width=0.45\linewidth]{figures/motivation/general_pose.png}\\
        % \multicolumn{2}{c}{(a) General detection (ATSS~\cite{ATSS})} \\
        \includegraphics[width=0.45\linewidth, clip, trim=250 200 100 80]{figures/motivation/ours_detection_case2_fcos.jpg} \\
        %  \includegraphics[width=0.32\linewidth,clip,trim=40 40 10 20]{figures/motivation/ours_pose.png} \\
        {\small (c) Baseline detection results} & {\small (d) Our detection results} \\
        \includegraphics[width=0.45\linewidth, clip, trim=250 200 100 80]{figures/motivation/general_pose_case2_fcos.jpg} &
        \includegraphics[width=0.45\linewidth, clip, trim=250 200 100 80]{figures/motivation/ours_pose_case2_fcos.jpg} \\
        {\small (e) Baseline pose results} & {\small (f) Our pose results} \\
        %  {\small (a) Baseline detection} & {\small (b) Our detection} & {\small (c) Pose results}\\
    \end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/figures/qualitative_results.tex <==

\begin{tabular}{cccc}
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/input/000326.png} &
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/input/000326.png} &
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/input/000438.png} &
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/input/000521.png} \\
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/fcos_detection_results/000002_000263.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/fcos_detection_results/000020_000021.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/fcos_detection_results/000001_000013.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/fcos_detection_results/000057_001026.jpg} \\
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/detection_results/000002_000263.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/detection_results/000020_000021.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/detection_results/000001_000013.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/detection_results/000057_001026.jpg} \\
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/wdr_results/000002_000263.png} & 
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/wdr_results/000057_001026.png} &
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/wdr_results/000020_000021.png} & 
    % \includegraphics[width=0.23\linewidth]{figures/qualitative results/wdr_results/000001_000013.png} \\
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/refine_results/000002_000263.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/refine_results/000020_000021.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/refine_results/000001_000013.jpg} &
    \includegraphics[width=0.23\linewidth]{figures/qualitative results/refine_results/000057_001026.jpg} \\

\end{tabular}



==> Rigidity-Aware Detection for 6D Object Pose Estimation/supp_content.tex <==
% !TEX root = ./supplemental.tex
% !TEX spellcheck = en-US

\begin{table*}
    \centering
    % \rowcolors{3}{}{gray!10}
    % \scalebox{0.9}{
    \begin{tabular}{l@{\hspace{3em}}ccc@{\hspace{3em}}ccc@{\hspace{3em}}ccc}
        \toprule
        \multirow{2}{*}{Category}  & \multicolumn{3}{c@{\hspace{3em}}}{FCOSv2~\cite{fcosv2}}                &\multicolumn{3}{c@{\hspace{3em}}}{PAA~\cite{PAA}}             &\multicolumn{3}{c}{\bf Ours}         \\
        ~                           & AP        & AP$_{50}$     & AP$_{75}$     & AP            & AP$_{50}$     & AP$_{75}$ & AP            & AP$_{50}$     & AP$_{75}$ \\
        \midrule
        Toaster                     & {20.9} &{38.4}& {30.5}          & 16.1          & 34.0          & 25.7      & {\bf 31.8}    & {\bf 47.2}    & {\bf 42.3}         \\
        Bottle                      & {38.3}      & {59.4}  & {43.1}          & 37.0          & 58.5          & 41.9        & {\bf 40.5}  & {\bf 60.7}    & {\bf 45.7}     \\
        Skateboard                  & 50.1       & {69.7} & 59.4          & {50.2}  & 69.3  & {60.2}      & {\bf 52.6} & {\bf 71.5}  & {\bf 63.8}        \\
        % bicycle                     &           &               &               & 27.3          &               &           & 29.7          &               &           \\
        Suitcase                    & 34.7      & {52.5}          & 38.8          & {35.1} & 52.0   & {39.0}       & {\bf 36.5}   & {\bf 53.6}    & {\bf 40.7}        \\ 
        Cup                         & 41.3      & 62.3  & {50.6}  & {41.5}  & {62.7}  & {50.6}      & {\bf 42.8}    & {\bf 63.2}    & {\bf 52.2}        \\
        ... & & ... & & & ... & & & ... \\
        \midrule
        Cat                         & {65.7}  & {86.8} & {68.4}          & {\bf 67.2}   & {\bf 88.9} & {\bf 69.8}     & 63.0          & 84.5          & 66.2        \\
        Dog                         & {60.7} & {81.9}   & {62.4}          & {\bf 62.1}    & {\bf 83.2}    & {\bf 63.9}       & 59.3          & 80.8         & 60.7     \\  
        Cow                         & {56.4}      & {72.3}  & {60.5}          & {\bf 58.0}    & {\bf 74.0}    & {\bf 62.8}      & 56.0           & 71.0       & 60.2   \\
        Sheep                       & {51.4} & {71.2}  & {60.7}          & {\bf 51.7}   & {\bf 71.6} & {\bf 61.2}      & 50.0          & 70.3          & 58.6         \\
        Bird                        & {\bf 36.2}& {\bf 54.8}& {\bf 42.3}    & {35.6}  & {54.0}  & 41.4     & 35.1          & 53.5          & {41.6}      \\
        ... & & ... & & & ... & & & ... \\
        \midrule
        {Avg.}                  & 38.9      & \underline{57.5}  & 42.2          & {\bf 40.4}          & {\bf 58.4}          & {\bf 43.9}      & \underline{40.0}    & 57.1  & \underline{43.4}      \\
        \bottomrule
    \end{tabular}
    % }
    \caption{{\bf Evaluation of general detection on COCO.} Although the general detection dataset COCO does not fully match our assumption of rigid targets, our method outperforms the baselines significantly on categories such as toaster, bottle, etc., which are mainly rigid objects, and our method achieves similar performance to the baselines in average accuracy.
    }
    \label{tab:coco_eval}
\end{table*}

\section{Appendix}

\noindent \textbf{General scenario.} Our work is motivated by the rigidity of the targets in 6D object pose estimation. The general scenario, e.g., COCO, does not fully match our assumption. Nevertheless, we report results with the same experimental setting as FCOSv2 and PAA in Table~\ref{tab:coco_eval}. In addition to the average accuracy across the 80 COCO categories, we report the accuracy of the 5 categories on which our method outperforms the baselines the most, and the 5 categories on which our method performs the worst. Our method outperforms the baselines significantly on categories such as toaster, bottle, etc., which are mainly rigid objects. By contrast, the categories on which our method underperforms include cat, dog, etc., which are mainly non-rigid targets and break our assumption. Our method nevertheless achieves similar performance to the baselines in average accuracy.

% \noindent \textbf{Additional qualitative results.}
% In Fig.~\ref{fig:more_vis}, we visualize additional results on the LM-O, T-LESS, IC-BIN, and YCB datasets. These results demonstrate the robustness of our method.

\noindent \textbf{Additional quantitative results.}
We show the detailed object pose results using different metrics on LM-O, T-LESS, TUD-L, IC-BIN, ITODD, HB, and YCB in Table~\ref{tab:compare_lmo},~\ref{tab:compare_tless},~\ref{tab:compare_tudl},~\ref{tab:compare_icbin},~\ref{tab:compare_itodd},~\ref{tab:compare_hb}, and~\ref{tab:compare_ycbv}, respectively.
Our method combined with PFA-Pose~\cite{pfa} outperforms the state of the art in most experimental settings.

\begin{table}[h]
    \centering
    \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_lmo_pose}
    }
    \caption{{\bf Additional object pose results on LM-O.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_lmo}
\end{table}

\begin{table}
    \centering
     \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_tless_pose}
    }
    \caption{{\bf Additional object pose results on T-LESS.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_tless}
\end{table}

\begin{table}
    \centering
     \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_tudl_pose}
    }
    \caption{{\bf Additional object pose results on TUD-L.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_tudl}
\end{table}

\begin{table}
    \centering
     \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_icbin_pose}
    }
    \caption{{\bf Additional object pose results on IC-BIN.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_icbin}
\end{table}

\begin{table}
    \centering
     \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_itodd_pose}
    }
    \caption{{\bf Additional object pose results on ITODD.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_itodd}
\end{table}

\begin{table}
    \centering
    \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_hb_pose}
    }
    \caption{{\bf Additional object pose results on HB.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_hb}
\end{table}

\begin{table}
    \centering
    \scalebox{0.95}{
    % \rowcolors{2}{}{gray!10}
    \input{tabs/compare_ycbv_pose}
    }
    \caption{{\bf Additional object pose results on YCB.}
    % We compare our method with PFA~\cite{pfa}, SurfEmb~\cite{surfemb}, CIR~\cite{coupled_iterative}, Cosypose~\cite{cosypose}, and CDPNv2~\cite{cdpn}.
    }
    \label{tab:compare_ycbv}
\end{table}

% \section{Pose Initialization Performance}
% PFA-Pose~\cite{pfa} relies on WDR-Pose~\cite{wdr}, which works on the whole image, for pose initialization.
% We do some modifications to incorporate our detection method into WDR-Pose.
% The original WDR-Pose uses the multi-level fusion strategy with the help of FPN~\cite{fpn} to handle the large depth range.
% However, the scale change becomes small when operating on the zoomed-in patch. Thus, we remove FPN and the multi-level fusion strategy, and only supervise the predictions from the foreground cells of the last stage of the backbone by the proposed 3D loss, in fact, more similar to Segdriven~\cite{segdriven}. 
% As shown in Table~\ref{tab:compare_estimator}, although the modified WDR-Pose follows a much simpler design philosophy, it outperforms other methods by a large margin with the help of our detection method.

% \noindent \textbf{Detailed detection results.}
% We show the detection results in more detailed metrics, including AP$_{50}$ and AP$_{75}$~\cite{coco, ATSS, PAA}, in Table~\ref{tab:compare_ap50_75}. Consistent with the main paper, our method outperforms other methods significantly, especially in the more strict metric AP$_{75}$.

% \begin{table*}
%     \centering
%     \rowcolors{2}{}{gray!10}
%     \input{tabs/compare_allpose_mspd}
%     \caption{{\bf Comparison against the state of the art on MSPD metric.}}
%     \label{tab:compare_mspd}
% \end{table*}

% \begin{table*}
%     \centering
%     \rowcolors{2}{}{gray!10}
%     \input{tabs/compare_allpose_mssd}
%     \caption{{\bf Comparison against the state of the art on MSSD metric.}}
%     \label{tab:compare_mssd}
% \end{table*}

% \begin{table*}
%     \centering
%     \rowcolors{2}{}{gray!10}
%     \input{tabs/compare_allpose_vsd}
%     \caption{{\bf Comparison against the state of the art on VSD metric.}}
%     \label{tab:compare_vsd}
% \end{table*}



% \begin{table}
%     \centering
%     \rowcolors{2}{}{gray!10}
%     \input{tabs/compare_estimator}
%     \caption{{\bf Comparison against the 6D pose estimation methods without pose refinement.}
%     Cosypose$\dag$ denotes Cosypose without pose refinement.}
%     \label{tab:compare_estimator}
% \end{table}

% \begin{figure*}
%     \centering
%     \setlength\tabcolsep{1pt}
%     \input{figures/more_visualization}
%     \caption{{\bf Additional qualitative results on LM-O, T-LESS, IC-BIN, and YCB-V.} We present the results on different datasets from top to bottom, showing the detection and object pose results for each.}
%     \label{fig:more_vis}
% \end{figure*}

% \begin{figure}
%     \centering
%     \setlength\tabcolsep{1pt}
%     \input{figures/more_visulaization_part2}
%     \caption{{\bf More visualization results on YCB-V.}}
%     \label{fig:more_vis_part2}
% \end{figure}

% \begin{table}
%     \centering
%     \rowcolors{3}{gray!10}{}
%     \input{tabs/compare_detect_more}
%     \caption{{\bf Detailed detection results.}
%     We compare our method with FCOSv2~\cite{fcosv2} and Mask R-CNN~\cite{maskrcnn} in different detection metrics.
%     }
%     \label{tab:compare_ap50_75}
% \end{table}
% \begin{table*}
%     \centering
%     \rowcolors{2}{}{gray!10}
%     \input{tabs/compare_detector_ap50}
%     \caption{{\bf Detection comparison on AP$_{50}$ metric.}}
%     \label{tab:compare_ap50}
% \end{table*}

% \begin{table*}
%     \centering
%     \rowcolors{2}{}{gray!10}
%     \input{tabs/compare_detector_ap75}
%     \caption{{\bf Detection comparison on AP$_{75}$ metric.}}
%     \label{tab:compare_ap75}
% \end{table*}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablate_detector.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Detector                                      & Pose Regressor                              & LM-O          & T-LESS        & TUD-L         & IC-BIN        & ITODD         & HB            & YCB-V         & Avg. \\
    \midrule
    {\bf RADet} & \multirow{3}{*}{WDR~\cite{wdr}}                                 & \textbf{0.614}& \textbf{0.588}& \textbf{0.623}& \textbf{0.514}& \textbf{0.247}& \textbf{0.618}& \textbf{0.605}& \textbf{0.544} \\
    Mask R-CNN~\cite{maskrcnn}  &          & 0.588         & 0.575         & 0.620         & 0.491         & 0.217         & 0.600         & 0.587         & 0.525  \\
    FCOS~\cite{fcosv1}           &         & 0.597         & 0.561         & 0.602         & 0.434         & 0.223         & 0.589         & 0.585         & 0.513 \\
    % -               & Ours                               & 0.614     & 0.678     & 0.796     & 0.514     & 0.247     & 0.618     & 0.709     &      \\
    % -               & Mask R-CNN~\cite{maskrcnn}            & 0.588     & 0.659     & 0.790     & 0.491     & 0.217     & 0.600     & 0.704     &       \\
    % -               & FCOS~\cite{fcosv1}                  & 0.597     & 0.689     & 0.799     & 0.434     & 0.223     & 0.589     & 0.707     &       \\               
    % \midrule
    % \multirow{3}{*}{CosyPose\dag~\cite{cosypose}}& {\bf RADet}                                 & \textbf{0.541}& \textbf{0.542}& \textbf{0.591}& \textbf{0.521}& \textbf{0.139}& \textbf{0.334}& \textbf{0.340}    & \textbf{0.429}   \\
    % ~                                           & Mask R-CNN~\cite{maskrcnn}            & 0.533         & 0.520         & 0.582         & 0.515         & 0.129         & 0.334         & 0.333             & 0.421 \\
    % ~                                           & FCOS~\cite{fcosv1}                    & 0.537         & 0.514         & 0.572         & 0.501         & 0.132         & 0.331         & 0.329             & 0.416  \\
    \midrule
    {\bf RADet} & \multirow{3}{*}{CDPNv2~\cite{cdpn}}                                 & \textbf{0.628}& \textbf{0.414}& \textbf{0.585}& \textbf{0.519}& \textbf{0.102}    & \textbf{0.731}& \textbf{0.397}    & {\bf 0.482}  \\
    Mask R-CNN~\cite{maskrcnn} &           & 0.612         & 0.415         & 0.552         & 0.517         & 0.094             & 0.728         & 0.386             & 0.472  \\
    FCOS~\cite{fcosv1}          &          & 0.624         & 0.407         & 0.575         & 0.473         & \textbf{0.102}    & 0.721         & 0.390             & 0.472  \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablation/activation.tex <==

\begin{tabular}{llccc}
    \toprule
    methods             & fusion        & AP                        &  AP$_{50}$                    & AP$_{75}$ \\
    \midrule
    random$^\dagger$    & \xmark        & 66.8$\pm$0.22             & 86.9 $\pm$0.22                & 75.1$\pm$0.11           \\
    random$^\dagger$    & \cmark        & 66.9$\pm$0.19             & 86.8 $\pm$0.15                & 74.8$\pm$0.14           \\
    all                 & \xmark        & 67.4$\pm$0.29             & 88.5 $\pm$0.21                & 76.1$\pm$0.63           \\
    all                 & \cmark        & 68.1$\pm$0.29             & 88.4 $\pm$0.23                & 76.7$\pm$0.25            \\
    topk                & \xmark        & 67.6$\pm$0.10             & 88.4 $\pm$0.19                & 75.2$\pm$0.16             \\
    topk                & \cmark        & 68.4$\pm$0.13             & 88.4 $\pm$0.18                & 76.6$\pm$0.26  \\
    random              & \xmark        & 69.0$\pm$0.15             & \textbf{88.7 $\pm$0.17}       & 77.5$\pm$0.13           \\
    random              & \cmark        & \textbf{69.6$\pm$0.12}    & 88.5 $\pm$0.19                & \textbf{78.7$\pm$0.25}           \\

    \bottomrule
\end{tabular}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablation/distance_transform_compare.tex <==




% \begin{tabular}{cc|ccc|ccc}
% \hline
%                                                                                         & vote              & AP                    & AP$_{50}$             & AP$_{75}$             & AP$_{s}$              & AP$_{m}$              & AP$_{l}$          \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}geodesic\\ distance\end{tabular}}            &                   & 68.4                  &    86.3               &      77.0             &    -                   &     63.6              &    68.7           \\ 
%                                                                                         &\cmark         & 68.8                  &    86.1               &      78.4             &    -                 &     63.8              &     69.4           \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}minimum\\ barrier\\ distance\end{tabular}}   & \multirow{2}{*}{} &\multirow{2}{*}{69.0}  & \multirow{2}{*}{88.7} & \multirow{2}{*}{77.5} & \multirow{2}{*}{-}     & \multirow{2}{*}{63.7} &\multirow{2}{*}{69.4}\\  
%                                                                                         &                   &                       &                       &                       &                       &                       &                   \\
%                                                                                         & \cmark        &    69.6               &      88.5             &      78.7             &     -                 &        63.9           &     70.0          \\ \hline
% \end{tabular}




\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
    data                                                                           & method                                                                      &fusion                        & AP                                & AP$_{50}$             & AP$_{75}$         \\%&AP$_{s}$           & AP$_{m}$              & AP$_{l}$      \\ \hline
    \midrule
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}real\end{tabular}}                  & \multirow{2}{*}{Geodesic}                                                   &\xmark                        &68.4$\pm$0.20                      &86.3$\pm$0.24          &77.0$\pm$0.36      \\%&-                  &63.6$\pm$0.25          & 68.7$\pm$0.19                         \\ 
                                                                                   &                                                                             &\cmark                        &68.8$\pm$0.17                      &86.1$\pm$\textbf{0.12}          &78.4$\pm$\underline{0.25}      \\%&-                  &63.5$\pm$0.24          & 69.4$\pm$0.14                        \\ \cline{2-9} 
    \cline{2-6} 
                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MinBarrier\end{tabular}}         &\xmark                        &69.0$\pm$0.15                      &\textbf{88.7}$\pm$0.17          &77.5$\pm$0.31      \\%&-                  &63.7$\pm$0.24          &69.4$\pm$0.16                                           \\ 
                                                                                   &                                                                             &\cmark                        &\textbf{69.6}$\pm$\textbf{0.12}    &88.5$\pm$0.19          &\textbf{78.7}$\pm$\textbf{0.25}      \\%&-                  &63.9$\pm$0.15          &70.0$\pm$0.15                                           \\ \hline
    % \midrule                                                                        
    % \multirow{4}{*}{Cityscapes}                                                    & \multirow{2}{*}{Geodesic}                                                   &                           &39.3          &64.2                   &38.9               \\%&17.8               &40.3                   &58.2                         \\ 
    %                                                                                &                                                                             &\cmark                 &39.7          &64.1                   &39.4               \\%&17.7               &40.5                   &58.6                        \\ \cline{2-9} 
    %                                                                                & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Minimum\\ barrier\end{tabular}}  &                           &39.8          &64.7                   &39.7               \\%&18.2               &42.9                   &57.4                         \\ 
    %                                                                                &                                                                             &\cmark                 &40.2          &64.6                   &40.1               \\%&18.4               &43.2                   &57.7                         \\ \hline
    \midrule                                                                               
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}real+sync\end{tabular}}             & \multirow{2}{*}{Geodesic}                                                  &\xmark                         &77.0$\pm$0.13 &92.1$\pm$0.16          &88.9$\pm$0.28      \\%&-                  &75.3$\pm$0.72          &77.6$\pm$0.17                         \\  
                                                                                   &                                                                            &\cmark                         &77.6$\pm$0.08 &92.0$\pm$0.13          &89.8$\pm$0.11      \\%&-                  &75.4$\pm$0.65          &78.3$\pm$0.09                         \\ \cline{2-9} 
    \cline{2-6}                                                                        
                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MinBarrier\end{tabular}}        &\xmark                         &77.8$\pm$0.05 &93.3$\pm$0.07          &89.7$\pm$0.17      \\%&-                  &75.7$\pm$0.64          &78.1$\pm$0.08            \\  
                                                                                   &                                                                            &\cmark                         &\textbf{78.2}$\pm$\textbf{0.07}       &\textbf{93.2}$\pm$\textbf{0.04}          &\textbf{90.1}$\pm$\textbf{0.12}      \\%&-                  &75.8$\pm$0.67          &78.6$\pm$0.05            \\ \hline
    \bottomrule
\end{tabular}
}
   




==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablation/hyper_parameters.tex <==

\begin{center}
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{l|lccc}
            \toprule
            \multicolumn{2}{c}{setting}         & AP                & AP$_{50}$         & AP$_{75}$ \\
            \midrule
            $\mathcal{T} = 0.1$     & $k = 10$  & 84.2               &                   &        \\
            $\mathcal{T} = 0.2$     & $k = 10$  & 84.8              &99.4               &97.1 \\
            $\mathcal{T} = 0.25$    & $k = 10$  &\textbf{85.0}      &\textbf{99.4}      &\textbf{97.4} \\
            $\mathcal{T} = 0.3$     & $k = 10$  &84.8               &99.2               &97.3 \\
            $\mathcal{T} = 0.4$     & $k = 10$  &               &                   & \\
            $\mathcal{T} = 0.5$     & $k = 10$  &                   &                   & \\
            \midrule
            $\mathcal{T} = 0.25$    & $k = 6$   &66.4               &87.9               &74.1 \\
            $\mathcal{T} = 0.25$    & $k = 8$   &66.4               &87.9               &74.1 \\
            $\mathcal{T} = 0.25$    & $k = 10$  &\textbf{69.6}      &\textbf{88.5}      &\textbf{78.7} \\
            $\mathcal{T} = 0.25$    & $k = 12$  &68.4               &87.2               &78.3\\
            $\mathcal{T} = 0.25$    & $k = 14$  &68.4               &87.2               &78.3\\
            $\mathcal{T} = 0.25$    & $k = 16$  &68.4               &87.2               &78.3\\
            \bottomrule
        \end{tabular}
    }
\end{center}


% \begin{tabular}{cccc|cccc|cccc}
%         \toprule
%         $k$                         & AP        & AP$_{50}$     & AP$_{75}$    & $\tau$     & AP        & AP$_{50}$     & AP$_{75}$  & $\alpha$ & AP        & AP$_{50}$     & AP$_{75}$ \\
%         \midrule
%         4                           & 83.4      & 98.4           & 93.5         & 0.1       & 84.1      & 98.5          & 96.0           & 0     & 83.9     & 98.8          & 94.3 \\
%         10                          & 85.0      & 99.4          & 97.4          & 0.2       & 84.7      & 99.3          & 96.8          & 0.1   & 85.0      & 99.4          & 97.4\\
%         32                          & 84.7      & 99.2          & 96.9          & 0.25      & 85.0      & 99.4          & 97.4          & 0.2   & 84.2      & 99.2          & 95.9\\
%         64                          & 84.2      & 98.9          & 96.3          & 0.3       & 84.9      & 99.4          & 97.0          & 0.3   & 83.1      & 98.4          & 93.2\\
%         128                         & 83.5      & 98.5          & 93.7          & 0.4       & 84.0      & 98.6          & 96.6          & 0.4   & 81.2      &               &   \\
%         256                         & 82.2      & 97.6          & 91.2          & 0.5       & 83.3      & 98.1          & 93.8          & 0.5   & 80.4      &               &   \\
%         \bottomrule
%     \end{tabular}
% }

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablation/training_schedule.tex <==
\begin{center}
    \begin{tabular}{ccccc}
        \toprule
        schedule                    & method       & AP                     & AP$_{50}$                 & AP$_{75}$               \\
        \midrule
        \multirow{2}*{$0.5$x}       & ATSS         & 66.3$\pm$0.08          & 84.7$\pm$0.17             &76.5$\pm$0.10          \\
        ~                           & {\bf Ours}          & \textbf{66.9$\pm$0.07} & \textbf{86.9$\pm$0.07}    &\textbf{74.7$\pm$0.08}           \\
        \midrule
        \multirow{2}*{$1$x}         & ATSS         & 68.8$\pm$0.04          & 86.8$\pm$0.08             &78.0$\pm$0.09          \\
        ~                           & {\bf Ours}          & \textbf{69.6$\pm$0.12} & \textbf{88.5$\pm$0.19}    &\textbf{78.7$\pm$0.25}           \\
        \midrule
        \multirow{2}*{$2$x}         & ATSS         & 64.4$\pm$0.68          & 81.3$\pm$0.85             &71.9$\pm$0.83               \\
        ~                           & {\bf Ours}          & \textbf{66.3$\pm$0.18} & \textbf{85.0$\pm$0.16}    &\textbf{73.1$\pm$0.19}            \\
        \bottomrule
        
    \end{tabular}
\end{center}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablation_activation.tex <==
\begin{tabular}{cccc}
    \toprule
    Method          & AP        & AP$_{50}$     & AP$_{75}$ \\
    \midrule
    all & 82.3      & 97.7         & 94.5       \\
    random$\dagger$ & 83.5      & 98.2          & 95.7       \\
    topk            & 84.0      & 99.0          & 96.1      \\
    {\bf random}    & {\bf 85.0}& {\bf 99.4}    & {\bf 97.4}      \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ablation_visibilty_modeling.tex <==
\begin{tabular}{lccc}
    \toprule
    Method                               & AP            & AP$_{50}$     & AP$_{75}$\\
    \midrule
    % box$^\dagger$                        & 81.1            & 97.9         & 88.3 \\
    % box                     & 81.3            & 97.6         & 88.6 \\
    % \textbf{Ours-mask$^\dagger$}        & 68.8            & 86.1         & 78.4         \\ 
    Center$^\dagger$      & 80.0          & 98.6 & 89.1 \\  
    Center                &  80.2         & 98.6  & 89.5\\
    % center filtering$^\dagger$                     & 82.4            & 97.3         & 89.3       \\
    % center filtering                     & 82.5            & 97.1         & 89.5       \\
    {\bf Ours}$^\dagger$                   & 84.2              & 99.3          & 96.2\\
    {\bf Ours}               & \underline{85.0}  & \underline{99.4}& \underline{97.4}        \\
    {\bf Oracle$^\dagger$}             &84.8      & \textbf{99.6} & 97.2\\
    {\bf Oracle}              &\textbf{85.7}      & \textbf{99.6} &\textbf{97.9}\\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/cityscapes_compare.tex <==

\begin{tabular}{lccccccc}
    \toprule
    method                      & backbone             & AP           & AP$_{50}$      & AP$_{75}$      & AP$_{s}$      & AP$_{m}$       & AP$_{l}$        \\
    \midrule
    Faster R-CNN    & ResNet-50           &38.3          & 63.3           & 40.1          &  16.5         &  38.9           & \textbf{60.4}                 \\
    FCOS           & ResNet-50            &38.0          & 63.1           & 38.6           & 17.2          &  38.7          & 55.5            \\ 
    ATSS             & ResNet-50            &39.5          & 63.9           & 40.3           & 16.9          &  40.3          & 57.6            \\ 
    PAA               & ResNet-50            &40.0          & \textbf{65.4}  & \textbf{40.8}  & 15.9          &  40.8          & 59.3            \\ 
    AutoAssign & ResNet-50            &29.5          & 50.7           & 29.3           & 10.9          &  30.3          & 47.2            \\
    \textbf{Ours}               & ResNet-50             &\textbf{40.2} & 64.6           & 40.1           & \textbf{18.4} & \textbf{43.2}  &  57.7     \\
    % \textbf{Mask (oracle)}               & ResNet-50            &\textbf{41.0} &  64.5          &  \textbf{42.5} & \underline{17.8}           & \underline{41.6}          & \textbf{60.6}    \\ 
    \midrule
    Faster R-CNN    & ResNet-101           &37.4          & 62.1          & 39.6           & 13.9          & 37.6            & 59.3                \\
    FCOS           & ResNet-101           &37.5          & 61.8           & 38.1           & 14.7          &  37.3          & 56.6            \\     
    ATSS             & ResNet-101           &38.4          & 62.9           & 38.3           & 15.4          &  39.4          & 57.7            \\ 
    PAA               & ResNet-101           &39.6          & \textbf{64.8}  & 39.5           & 15.5          &  \textbf{42.0} & \textbf{59.5}            \\ 
    AutoAssign & ResNet-101           &31.3          & 54.3           & 30.2           & 9.6           &  31.3          & 50.2            \\   
    \textbf{Ours}                & ResNet-101           &\textbf{39.8} & 63.1           & \textbf{41.4}  & \textbf{16.3} &  41.0          & \textbf{59.5}            \\
    % \textbf{Mask (oracle)}      & ResNet-101           &\textbf{40.6} & \textbf{64.9}           & \underline{41.3}           & \textbf{16.7} & \underline{41.5}  & \textbf{60.9}   \\ 
    \bottomrule
\end{tabular}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/coco_campare_category.tex <==

% \begin{table}
% 	\centering
% 	\tiny
% 	\begin{tabular}{cccc|cccc}
% 		\toprule
% 		                &  PAA       & \textbf{Ours}   	&\textcolor{green}{$\Delta$}    		&				& PAA 	& \textbf{Ours} &\textcolor{green}{$\Delta$}\\
% 		\midrule	
% 		parking meter   &  45.4      & 40.6           	&  \textcolor{green}{-4.8}           	&toaster 		& 22.4   & 31.8        	&\textcolor{green}{+9.4}\\
% 		scissors        &  29.6      & 24.8           	&  \textcolor{green}{-4.8}           	&bottle   		& 36.1   & 38.4        	&\textcolor{green}{+2.3}\\
% 		horse           &  58.1      & 54.7           	&  \textcolor{green}{-3.4}           	&handbag  		& 13.2   & 10.0        	&\textcolor{green}{+3.2}\\
% 		dog             &  62.6      & 59.9           	& \textcolor{green}{-2.7}            	&wine glasses  	& 33.8   & 35.8        	&\textcolor{green}{+2.0}\\
% 		carrot          &  22.5      & 19.8       	  	&\textcolor{green}{-2.7}			   	&skateboard    	& 50.9   & 52.6		   	&\textcolor{green}{+2.7}\\
% 		donut           &  47.3      & 44.8       		&\textcolor{green}{-2.5}				&banana        	& 23.2   & 24.6        	&\textcolor{green}{+1.4}\\
% 		cow             &  57.9      & 55.5             &\textcolor{green}{-2.4}				&car           	& 42.6   & 44.0			&\textcolor{green}{+1.4}\\
% 		keyboard        &  55.1      & 53.0       		&\textcolor{green}{-2.1}				&boat         	& 25.0   & 26.2			&\textcolor{green}{+1.2}\\
% 		umbrella        &  38.1      & 36.1       		&\textcolor{green}{-2.0}				&cell phone     & 34.4   & 33.3			&\textcolor{green}{+1.1}\\
% 		sandwich        &  23.3      & 21.6       		&\textcolor{green}{-1.7}  				&cup           	& 40.8   & 41.9			&\textcolor{green}{+1.1}\\
% 		knife           &  13.8      & 12.1       		&\textcolor{green}{-1.7}				&pizza          & 50.4   & 51.4 		&\textcolor{green}{+1.0}\\
% 		bench           &  23.3      & 21.6       		&\textcolor{green}{-1.7}				&bicycle       	& 29.0   & 29.9			&\textcolor{green}{+0.9}\\
% 		dining table    &  28.7      & 27.2       		&\textcolor{green}{-1.5}				&vase          	& 35.7   & 36.6			&\textcolor{green}{+0.9}\\
% 		hot dog         &  32.5      & 31.3       		&\textcolor{green}{-1.2}				&suitcase      	& 35.6   & 36.5			&\textcolor{green}{+0.9}\\
% 		laptop          &  58.0      & 56.8       		&\textcolor{green}{-1.2}				&fork          	& 26.7   & 27.5			&\textcolor{green}{+0.8}\\
% 		sink            &  36.1      & 35.0      		&\textcolor{green}{-1.1} 				&tie           	& 30.7   & 31.5			&\textcolor{green}{+0.8}\\
% 		% cat             &  68.2      & 67.4       		&\textcolor{green}{}&cell phone    & 33.3   & 34.4\\
% 		% airplane        &  66.6      & 65.6
% 		% bear            &  70.2      & 69.3
% 		% zebra           &  68.7      & 67.9

% 		\bottomrule
		

% 		% \toprule
% 		% PAA better 													& Ours better\\
% 		% \midrule
% 		% parking meter(40.6/45.4)                                 &  toaster(31.8/22.4) \\
% 		% scissors(24.8/29.6)										 &  bottle(38.4/36.1)  \\
% 		% horse(54.7/58.1)                                         &  handbag(13.2/10.0) \\
% 		% dog(59.9/62.6), carrot(19.8/22.5)                        &  wine glass(35.8/33.8)  \\
% 		% donut(44.8/47.3)                                         &  skateboard(52.6/50.9\\
% 		% cow(55.5/57.9)                                           &  banana(24.6/23.2), car(44.0/42.6)\\
% 		% keyboard(53.0/55.1)                                      &  truck(37.2/36.4), boat(26.2/25.0)\\
% 		% umbrella(36.1/38.1)                                      &  cell phone(34.4/33.3), cup(41.9/40.8)\\
% 		% cat(67.4/68.2), sandwich(34.4/36.2)                      &  pizza(51.4/50.4)\\
% 		% knife(12.1/13.8), bench(21.6/23.3)                       &  bicycle(29.9/29.0), vase(36.6/35.7), suitcase(36.5/35.6)\\
% 		% dining table(27.2/28.7)                                  &  fork(27.5/26.7), tie(31.5/30.7)\\
% 		% hot dog(31.3/32.5), laptop(56.8/58.0)                    &  \\
% 		% sink(35.0/36.1)                                          &    \\
% 		% airplane(65.6/66.6)                                      &   \\
% 		% bear(69.3/70.2),                                         &   \\
% 		% zebra(67.9/68.7)                                         &    \\
% 		% \bottomrule

% 	\end{tabular}
% \end{table}



% \begin{table}
%     \centering
%     \tiny
%     \begin{tabular}{cccc|cccc}
%         \toprule
%                 &  PAA       & \textbf{Ours}   	&$\Delta$    		&				& PAA 	& \textbf{Ours} &$\Delta$\\
%         \midrule
%         bottle   		& 36.1  & 38.4     &\textcolor{green}{+2.3}  &car           & 42.6   & 44.0     &\textcolor{green}{+1.4}\\
%         wine glasses  	& 33.8  & 35.8     &\textcolor{green}{+2.0}  &boat         & 25.0   & 26.2	    &\textcolor{green}{+1.2}\\
%         cup           	& 40.8  & 41.9     &\textcolor{green}{+1.1}  &bicycle       & 29.0   & 29.9		&\textcolor{green}{+0.9}\\
%         vase          	& 35.7  & 36.6	   &\textcolor{green}{+0.9}  &truck         & 36.4   & 37.2     &\textcolor{green}{+0.8}\\\cline{1-4}
%         horse           & 58.1  & 54.7     & \textcolor{red}{-3.4}  &airplane      & 66.6   & 65.6     &\textcolor{red}{-1.0}\\\cline{5-8}
%         dog             & 62.6  & 59.9     & \textcolor{red}{-2.7}  &carrot        & 22.5   & 19.8     &\textcolor{red}{-2.7}\\
%         cow             & 57.9  & 55.5     & \textcolor{red}{-2.4}  &donut         & 47.3   & 44.8     &\textcolor{red}{-2.5}\\
%         bear            & 70.2  & 69.3     & \textcolor{red}{-0.9} &sandwich      & 23.3   & 21.6     &\textcolor{red}{-1.7}\\
%         cat             & 68.2  & 67.4     & \textcolor{red}{-0.8} &hot dog       & 32.5   & 31.3     &\textcolor{red}{-1.2}\\
%         zebra           & 68.7  & 67.9     & \textcolor{red}{-0.8} &banana        & 23.2   & 24.6     &\textcolor{green}{+1.4}\\\cline{1-4}
%         scissors        & 29.6  & 24.8     &\textcolor{red}{-4.8} &pizza         & 50.4   & 51.4 	    &\textcolor{green}{+1.0}\\\cline{5-8}
%         knife           & 13.8  & 12.1     &\textcolor{red}{-1.7}   &bench         & 23.3   & 21.6      &\textcolor{red}{-1.7}\\
%         fork          	& 26.7  & 27.5	   &\textcolor{green}{+0.8}   &dining table  & 28.7   & 27.2      &\textcolor{red}{-1.5}\\\cline{1-4}
%         toaster 		& 22.4  & 31.8     &\textcolor{green}{+9.4}   &sink          & 36.1   & 35.0      &\textcolor{red}{-1.1}\\\cline{5-8}
%         skateboard    	& 50.9  & 52.6	   &\textcolor{green}{+2.7} &handbag  		& 13.2   & 10.0    &\textcolor{green}{+3.2}\\
%         suitcase      	& 35.6   & 36.5    &\textcolor{green}{+0.9} &tie           	& 30.7   & 31.5			&\textcolor{green}{+0.8}\\
%         keyboard        & 55.1  & 53.0     &\textcolor{red}{-2.1} &umbrella        &  38.1      & 36.1     &\textcolor{red}{-2.0}\\
%         &&&                                                       &laptop        &  58.0  & 56.8     &\textcolor{red}{-1.2}\\

%         \bottomrule
        

        
%     \end{tabular}

% \end{table}


\begin{table}[h]
    \centering
    
    \resizebox{\linewidth}{!}{
    \small
    \begin{tabular}{cccc|cccc}
        \toprule
                &  PAA       & \textbf{Ours}   	&$\Delta$    		&				& PAA 	& \textbf{Ours} &$\Delta$\\
        \midrule
        toaster 		& 22.4  & 31.8      &\textcolor{green}{+9.4}    & horse             & 58.1  & 54.7     & \textcolor{red}{-3.4}\\
        skateboard    	& 50.9  & 52.6	    &\textcolor{green}{+2.7}    & dog               & 62.6  & 59.9     & \textcolor{red}{-2.7}\\
        suitcase      	& 35.6  & 36.5      &\textcolor{green}{+0.9}    & cow               & 57.9  & 55.5     & \textcolor{red}{-2.4}\\
        keyboard        & 55.1  & 53.0      &\textcolor{red}{-2.1}      & bear              & 70.2  & 69.3     & \textcolor{red}{-0.9}\\\cline{1-4}
        bottle   		& 36.1  & 38.4      &\textcolor{green}{+2.3}    & cat               & 68.2  & 67.4     & \textcolor{red}{-0.8}\\
        wine glasses  	& 33.8  & 35.8      &\textcolor{green}{+2.0}    & zebra             & 68.7  & 67.9     & \textcolor{red}{-0.8}\\\cline{5-8}
        cup           	& 40.8  & 41.9      &\textcolor{green}{+1.1}    & scissors          & 29.6  & 24.8     &\textcolor{red}{-4.8}\\
        vase          	& 35.7  & 36.6	    &\textcolor{green}{+0.9}    & knife             & 13.8  & 12.1     &\textcolor{red}{-1.7}\\\cline{1-4}
        car             & 42.6  & 44.0      &\textcolor{green}{+1.4}    & fork          	& 26.7  & 27.5	   &\textcolor{green}{+0.8}\\\cline{5-8}
        boat            & 25.0  & 26.2	    &\textcolor{green}{+1.2}    & carrot            & 22.5   & 19.8     &\textcolor{red}{-2.7}\\
        bicycle         & 29.0  & 29.9		&\textcolor{green}{+0.9}    & donut             & 47.3   & 44.8     &\textcolor{red}{-2.5}\\
        truck           & 36.4  & 37.2      &\textcolor{green}{+0.8}    & sandwich          & 23.3   & 21.6     &\textcolor{red}{-1.7}\\
        airplane        & 66.6  & 65.6      &\textcolor{red}{-1.0}      & hot dog           & 32.5   & 31.3     &\textcolor{red}{-1.2}\\\cline{1-4}
        handbag  		& 13.2  & 10.0      &\textcolor{green}{+3.2}    & banana            & 23.2   & 24.6     &\textcolor{green}{+1.4}\\
        tie           	& 30.7  & 31.5	    &\textcolor{green}{+0.8}    & pizza             & 50.4   & 51.4 	&\textcolor{green}{+1.0}\\\cline{5-8}
        umbrella        & 38.1  & 36.1      &\textcolor{red}{-2.0}      & bench             & 23.3   & 21.6      &\textcolor{red}{-1.7}\\
        laptop          & 58.0  & 56.8      &\textcolor{red}{-1.2}      & dining table      & 28.7   & 27.2      &\textcolor{red}{-1.5}\\
                        &       &           &                           & sink              & 36.1   & 35.0      &\textcolor{red}{-1.1}\\

        \bottomrule
        

        
    \end{tabular}
    }

\end{table}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/coco_compare.tex <==
\begin{tabular}{cc|ccc|ccc}
    \hline
    method                      & backbone              & AP        & AP$_{50}$ & AP$_{75}$     &AP$_{s}$   &AP$_{m}$   & AP$_{l}$  \\ \hline
    FCOS\cite{fcosv2}           & ResNet-50             & 38.9      &  57.5     & 42.2          &  23.1     & 42.7      &  50.2      \\ 
    ATSS\cite{ATSS}             & ResNet-50             & 39.2      &  57.3     & 42.4          &  22.7     & 43.1      &  51.5    \\ 
    PAA\cite{PAA}               & ResNet-50             & 40.4      &  58.4     & 43.9          &  22.9     & 44.3      &  54.0    \\
    AutoAssign\cite{autoassign} & ResNet-50             & 40.4      &  59.6     & 43.7          &  22.7     & 44.1      &  52.9     \\
    \textbf{Distance}           & ResNet-50             & 40.0      &  57.1     & 43.4          &  23.5     & 43.5      &  51.9     \\\hline
    FCOS\cite{fcosv2}           & ResNet-101            & 43.2      & 62.4      & 46.8          &  26.1     & 46.2      &   52.8    \\ 
    ATSS\cite{ATSS}             & ResNet-101            & 43.6      & 62.1      & 47.4          &  26.1     & 47.0      &   53.6    \\ 
    PAA\cite{PAA}               & ResNet-101            & 44.6      & 63.3      & 48.4          &  26.4     & 48.5      &   56.0    \\
    AutoAssign\cite{autoassign} & ResNet-101            & 44.5      & 64.3      & 48.4          &  25.9     & 47.4      &   55.0    \\
    \textbf{Distance}           & ResNet-101            & 44.1      & 62.2      & 48.1          &  26.7     & 47.2      &   54.8    \\\hline
\end{tabular}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_all_pose.tex <==
% \begin{tabular}{ccc|ccccccc|c}
%     \toprule
%     Method                      & Real              & Data      & LM-O              & T-LESS             & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V             & Avg.          \\
%     \midrule
%     \textbf{Ours+PFA}           & \checkmark         & RGB       & \textbf{0.715}    & \textbf{0.778}    & \textbf{0.839}   & \textbf{0.600}    & 0.353             & \textbf{0.840}    & 0.806             & \textbf{0.704} \\
%     PFA~\cite{pfa}              & \checkmark        & RGB       & 0.676             & -                 & -                 & -                 & -                 & -                 & 0.748             & -     \\
%     SurfEmb~\cite{surfemb}      & \checkmark        & RGB       & 0.663             & 0.770             & 0.805             & 0.588             & \textbf{0.413}    & 0.791             & 0.711             & 0.677             \\
%     CosyPose~\cite{cosypose}    & \checkmark        & RGB       & 0.633             & 0.728             & 0.823             & 0.583             & 0.216             & 0.656             & \textbf{0.821}    & 0.637 \\
%     CDPNv2~\cite{cdpn}          & \checkmark        & RGB       & 0.624             & 0.478             & 0.772             & 0.473             & 0.067              & 0.722             & 0.532             & 0.529 \\
%     Pix2Pose~\cite{pix2pose}    & \checkmark        & RGB       & 0.363             & 0.344             & 0.420             & 0.226             & 0.102             & 0.346             & 0.446             & 0.342 \\
%     \midrule
%     \textbf{Ours+PFA}           &                   & RGB       & \ast              & 0.719             & \textbf{0.733}    & \ast              & \ast              & \ast              & \textbf{0.648}    & \textbf{0.658} \\
%     PFA~\cite{pfa}              &                   & RGB       & \ast              &  -                & -                 & \ast              & \ast              & \ast              & 0.614             & -   \\
%     SurfEmb~\cite{surfemb}      &                   & RGB       & \ast              & \textbf{0.735}    & 0.715             & \ast              & \ast              & \ast              & 0.647             & 0.650 \\
%     CosyPose~\cite{cosypose}    &                   & RGB       & \ast              & 0.640             & 0.685             & \ast              & \ast              & \ast              & 0.574             & 0.570 \\
%     CDPNv2~\cite{cdpn}          &                   & RGB       & \ast              & 0.407             & 0.588             & \ast              & \ast              & \ast              & 0.390             & 0.472 \\
%     \midrule
%     \textbf{Ours+PFA}          & \checkmark         & RGB-D     & \textbf{0.797}    & \textbf{0.850}    & 0.960             & 0.676             & 0.460             & \textbf{0.869}    & 0.888             & \textbf{0.787} \\
%     PFA~\cite{pfa}              & \checkmark        & RGB-D     & 0.751             & -                 &  -                & -                 & -                 & -                 & 0.823             & -\\
%     SurfEmb~\cite{surfemb}      & \checkmark        & RGB-D     & 0.760             & 0.833             & 0.933             & 0.659             & \textbf{0.538}    & 0.866             & 0.824             & 0.773 \\
%     CIR~\cite{coupled_iterative}& \checkmark        & RGB-D     & 0.734             & 0.776             & \textbf{0.968}    & 0.676             & 0.381             & 0.757             & \textbf{0.893}    & 0.741 \\
%     CosyPose+ICP~\cite{cosypose}& \checkmark        & RGB-D     & 0.714             & 0.701             & 0.939             & 0.647             & 0.313             & 0.712             & 0.861             & 0.698 \\
%     Pix2Pose+ICP~\cite{pix2pose}& \checkmark        & RGB-D     & 0.588             & 0.512	            & 0.820	            & 0.390	            & 0.351	            & 0.695	            & 0.780	            & 0.591 \\
%     CDPNv2+ICP~\cite{cdpn}      & \checkmark        & RGB-D     & 0.630             & 0.464             & 0.913             & 0.450             & 0.186             & 0.712             & 0.619            & 0.568 \\
%     \midrule
%     \textbf{Ours+PFA}           &                   & RGB-D     & \ast              & 0.801             & \textbf{0.894}    & \ast              & \ast              & \ast              & \textbf{0.826}    & \textbf{0.762} \\
%     PFA~\cite{pfa}              &                   & RGB-D     & \ast              & -                 &  -                & -                 & -                 & -                 & 0.804             & -\\
%     SurfEmb~\cite{surfemb}      &                   & RGB-D     & \ast              & \textbf{0.828}    & 0.854             & \ast              & \ast              & \ast              & 0.799             & 0.758 \\
%     CDPNv2+ICP~\cite{cdpn}      &                   & RGB-D     & \ast              & 0.435             & 0.791             & \ast              & \ast              & \ast              & 0.532             & 0.534 \\
%     \bottomrule
% \end{tabular}

\begin{tabular}{lll|lllllll|l}
    \toprule
    Method                      & Real              & Data      & LM-O$^{\ast}$              & T-LESS             & TUD-L             & IC-BIN$^{\ast}$            & ITODD$^{\ast}$             & HB$^{\ast}$                & YCB             & Avg.          \\
    \midrule
    \textbf{PFA+Ours}           &                   & RGB       & \textbf{0.715}     & 0.719             & \textbf{0.733}    & \textbf{0.600}& 0.353              & \textbf{0.840}     & \textbf{0.648}    & \textbf{0.658} \\
    PFA~\cite{pfa}              &                   & RGB       & 0.674              &  -                & -                 &  -             & -                   & -              & 0.614             & -   \\
    SurfEmb~\cite{surfemb}      &                   & RGB       & 0.663              & \textbf{0.735}    & 0.715             &  0.588        & \textbf{0.413}     & 0.791               & 0.647             & 0.650 \\
    CosyPose~\cite{cosypose}    &                   & RGB       & 0.633              & 0.640             & 0.685             &  0.473        & 0.216              & 0.656              & 0.574             & 0.570 \\
    CDPNv2~\cite{cdpn}          &                   & RGB       & 0.624              & 0.407             & 0.588             &  0.226        & 0.067              & 0.722               & 0.390             & 0.472 \\
    \midrule
    \textbf{PFA+Ours}           & \checkmark        & RGB       & \textbf{0.715}& \textbf{0.778}& \textbf{0.839}   & \textbf{0.600}& 0.353          & \textbf{0.840}    & 0.806             & \textbf{0.704} \\
    PFA~\cite{pfa}              & \checkmark        & RGB       & 0.674    & -                 & -                 & -                     & -               & -               & 0.748             & -     \\
    SurfEmb~\cite{surfemb}      & \checkmark        & RGB       & 0.663    & 0.770             & 0.805             & 0.588        & \textbf{0.413} & 0.791    & 0.711             & 0.677             \\
    CosyPose~\cite{cosypose}    & \checkmark        & RGB       & 0.633    & 0.728             & 0.823             & 0.583        & 0.216    & 0.656    & \textbf{0.821}    & 0.637 \\
    CDPNv2~\cite{cdpn}          & \checkmark        & RGB       & 0.624    & 0.478             & 0.772             & 0.473        & 0.067     & 0.722     & 0.532             & 0.529 \\
    % Pix2Pose~\cite{pix2pose}    & \checkmark        & RGB       & 0.363             & 0.344             & 0.420             & 0.226                 & 0.102             & 0.346                 & 0.446             & 0.342 \\
    \midrule
    \textbf{PFA+Ours}           &                   & RGBD     & \textbf{0.797}    & 0.801             & \textbf{0.894}    & \textbf{0.676}    & 0.460             & \textbf{0.869}    & \textbf{0.826}    & \textbf{0.762} \\
    PFA~\cite{pfa}              &                   & RGBD     & 0.751             & -                 &  -                & -                 & -                 & -                 & 0.804             & -\\
    SurfEmb~\cite{surfemb}      &                   & RGBD     & 0.760             & \textbf{0.828}    & 0.854             & 0.659             & \textbf{0.538}    & 0.866             & 0.799             & 0.758 \\
    CDPNv2+ICP~\cite{cdpn}      &                   & RGBD     & 0.630             & 0.435             & 0.791             & 0.450             & 0.186             &  0.712            & 0.532             & 0.534 \\
    \midrule
    \textbf{PFA+Ours}           & \checkmark         & RGBD     & \textbf{0.797}    & \textbf{0.850}    & 0.960            & \textbf{0.676}    & 0.460    & \textbf{0.869}& 0.888             & \textbf{0.787} \\
    PFA~\cite{pfa}              & \checkmark        & RGBD     & 0.751    & -                 &  -                & -                 & -                 & -                 & 0.823             & -\\
    SurfEmb~\cite{surfemb}      & \checkmark        & RGBD     & 0.760    & 0.833             & 0.933             & 0.659    & \textbf{0.538}& 0.866& 0.824             & 0.773 \\
    CIR~\cite{coupled_iterative}& \checkmark        & RGBD     & 0.734             & 0.776             & \textbf{0.968}    & \textbf{0.676}    & 0.381             & 0.757             & \textbf{0.893}    & 0.741 \\
    CosyPose+ICP~\cite{cosypose}& \checkmark        & RGBD     & 0.714             & 0.701             & 0.939             & 0.647             & 0.313             & 0.712             & 0.861             & 0.698 \\
    % Pix2Pose+ICP~\cite{pix2pose}& \checkmark        & RGBD     & 0.588             & 0.512	            & 0.820	            & 0.390	            & 0.351	            & 0.695	            & 0.780	            & 0.591 \\
    CDPNv2+ICP~\cite{cdpn}      & \checkmark        & RGBD     & 0.630    & 0.464             & 0.913             & 0.450    & 0.186    & 0.712    & 0.619            & 0.568 \\
    \bottomrule
\end{tabular}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_all_pose_rgb.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Method                      & Real            & LM-O              & T-LESS             & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V             & Avg.          \\
    \midrule
    \textbf{RADet+PFA}          & \checkmark           &\textbf{0.715}     & \textbf{0.778}    & \textbf{0.839}    & \textbf{0.600}    & 0.353             & \textbf{0.840}    & 0.806             & \textbf{0.704} \\
    % \textbf{RADet+WDR}          & \checkmark           & 0.614             & 0.678             & 0.796             & 0.514             & 0.247             & 0.618             & 0.722             & 0.598 \\
    SurfEmb~\cite{surfemb}      & \checkmark           & 0.663             & 0.770             & 0.805             & 0.588             & \textbf{0.413}    & 0.791             & 0.711             & 0.677             \\
    CosyPose~\cite{cosypose}    & \checkmark           & 0.633             & 0.728             & 0.823             & 0.583             & 0.216             & 0.656             & \textbf{0.821}             & 0.637 \\
    CDPNv2~\cite{cdpn}          & \checkmark           & 0.624             & 0.478             & 0.772             & 0.473             & 0.102             & 0.722             & 0.532             & 0.529 \\
    Pix2Pose~\cite{pix2pose}    & \checkmark           & 0.363             & 0.344             & 0.420             & 0.226             & 0.134             & 0.346             & 0.446             & 0.342 \\
    % PFA~\cite{pfa}              & \checkmark           & 0.701             & -                 & -                 & -                 & -                 & -                 & 0.738             & -     \\
    % DPODv2~\cite{dpodv2}        & \checkmark    & RGB       & 0.584             & 0.655             & -                 & -                 & -                 & 0.725             & -                 & -    \\
    % CIR~\cite{coupled_iterative}& \checkmark    & RGB       & 0.655             & 0.715             & -                 &   -               & -                 & -                 & \textbf{0.824}    &   - \\
    \midrule
    \textbf{RADet+PFA}          &                      & \textbf{0.715}    & 0.719             & \textbf{0.733}    & \textbf{0.600}    & 0.353             & \textbf{0.840}    & \textbf{0.648}    & \textbf{0.658} \\
    % \textbf{RADet+WDR}          &                      & 0.614             & 0.588             & 0.623             & 0.514             & 0.247             & 0.618             & 0.605             & 0.544 \\
    PFA~\cite{pfa}              &                      & 0.676             &  -                & -                 & -                 & -                 & -                 & 0.614             & -   \\
    SurfEmb~\cite{surfemb}      &                      & 0.663             & \textbf{0.735}    & 0.715             & 0.588             & \textbf{0.413}    & 0.791             & 0.647             & 0.650 \\
    CosyPose~\cite{cosypose}    &                      & 0.633             & 0.640             & 0.685             & 0.583             & 0.216             & 0.656             & 0.574             & 0.570 \\
    CDPNv2~\cite{cdpn}          &                      & 0.624             & 0.407             & 0.588             & 0.473             & 0.102             & 0.722             & 0.390             & 0.472 \\
    % PFA~\cite{pfa}              &                      & 0.701             &  -                & -                 & -                 & -                 & -                 & 0.615             & -   \\
    % DPODv2~\cite{dpodv2}        &               & RGB       & 0.584             & 0.636             & -                 & -                 & -                 & 0.725             & -                 & -    \\
    % \midrule
    % \textbf{RADet+PFA}          & \checkmark    & RGB-D     & \textbf{0.797}    & \textbf{0.850}    & 0.960             & \textbf{0.676}    & 0.469             & \textbf{0.869}    & 0.888             & \textbf{0.787} \\
    % SurfEmb~\cite{surfemb}      & \checkmark    & RGB-D     & 0.760             & 0.833             & 0.933             & 0.659             & \textbf{0.538}    & 0.866             & 0.824             & 0.773 \\
    % CIR~\cite{coupled_iterative}& \checkmark    & RGB-D     & 0.734             & 0.776             & \textbf{0.968}    & \textbf{0.676}    & 0.381             & 0.757             & \textbf{0.893}    & 0.741 \\
    % CosyPose+ICP~\cite{cosypose}& \checkmark    & RGB-D     & 0.714             & 0.701             & 0.939             & 0.647             & 0.313             & 0.712             & 0.861             & 0.698 \\
    % Pix2Pose+ICP~\cite{pix2pose}& \checkmark    & RGB-D     & 0.588             & 0.512	            & 0.820	            & 0.390	            & 0.351	            & 0.695	            & 0.780	            & 0.591 \\
    % CDPNv2+ICP~\cite{cdpn}      & \checkmark    & RGB-D     & 0.630             & 0.464             & 0.913             & 0.450             & 0.186             & 0.712             & 0.619             & 0.568 \\
    % PFA~\cite{pfa}              &               & RGB-D     & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.822             & -\\
    % % DPODv2~\cite{dpodv2}        & \checkmark    & RGB-D     & 0.700             & 0.720             & -                     & -                 & -                 & 0.840             & -                 & -    \\
    % \midrule
    % \textbf{RADet+PFA}         &                & RGB-D     & \textbf{0.797}    & 0.801             & \textbf{0.894}    & \textbf{0.676}    & 0.469             & \textbf{0.869}    & \textbf{0.826}    & \textbf{0.762} \\
    % SurfEmb~\cite{surfemb}     &                & RGB-D     & 0.760             & \textbf{0.828}    & 0.854             & 0.659             & \textbf{0.538}    & 0.866             & 0.799             & 0.758 \\
    % CDPNv2+ICP~\cite{cdpn}     &                & RGB-D     & 0.630             & 0.435             & 0.791             & 0.450             & 0.186             & 0.712             & 0.532             & 0.534 \\
    % % DPODv2~\cite{dpodv2}       &                & RGB-D     & 0.700             & 0.699             & -                 & -                 & -                 & 0.840             & -                 & -    \\
    % PFA~\cite{pfa}             &                & RGB-D     & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.800             & -\\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_all_pose_rgbd.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Method                      & Real          & LM-O              & T-LESS             & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V             & Avg.          \\
    \midrule
    \textbf{RADet+PFA}          & \checkmark    & \textbf{0.797}    & \textbf{0.850}    & 0.960             & \textbf{0.676}    & 0.469             & \textbf{0.869}    & 0.888             & \textbf{0.787} \\
    SurfEmb~\cite{surfemb}      & \checkmark    & 0.760             & 0.833             & 0.933             & 0.659             & \textbf{0.538}    & 0.866             & 0.824             & 0.773 \\
    CIR~\cite{coupled_iterative}& \checkmark    & 0.734             & 0.776             & \textbf{0.968}    & \textbf{0.676}    & 0.381             & 0.757             & \textbf{0.893}    & 0.741 \\
    CosyPose+ICP~\cite{cosypose}& \checkmark    & 0.714             & 0.701             & 0.939             & 0.647             & 0.313             & 0.712             & 0.861             & 0.698 \\
    Pix2Pose+ICP~\cite{pix2pose}& \checkmark    & 0.588             & 0.512	            & 0.820	            & 0.390	            & 0.351	            & 0.695	            & 0.780	            & 0.591 \\
    CDPNv2+ICP~\cite{cdpn}      & \checkmark    & 0.630             & 0.464             & 0.913             & 0.450             & 0.186             & 0.712             & 0.619             & 0.568 \\
    % PFA~\cite{pfa}              &               & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.822             & -\\
    % DPODv2~\cite{dpodv2}        & \checkmark    & RGB-D     & 0.700             & 0.720             & -                     & -                 & -                 & 0.840             & -                 & -    \\
    \midrule
    \textbf{RADet+PFA}         &                & \textbf{0.797}    & 0.801             & \textbf{0.894}    & \textbf{0.676}    & 0.469             & \textbf{0.869}    & \textbf{0.826}    & \textbf{0.762} \\
    SurfEmb~\cite{surfemb}     &                & 0.760             & \textbf{0.828}    & 0.854             & 0.659             & \textbf{0.538}    & 0.866             & 0.799             & 0.758 \\
    CDPNv2+ICP~\cite{cdpn}     &                & 0.630             & 0.435             & 0.791             & 0.450             & 0.186             & 0.712             & 0.532             & 0.534 \\
    % DPODv2~\cite{dpodv2}       &                & RGB-D     & 0.700             & 0.699             & -                 & -                 & -                 & 0.840             & -                 & -    \\
    % PFA~\cite{pfa}             &                & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.800             & -\\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_allpose_mspd.tex <==
% \begin{tabular}{lll|lllllll|l}
%   \toprule
%   Method                      & Real    & Data        & LM-O$^{\ast}$     & T-LESS            & TUD-L             & IC-BIN$^{\ast}$   & ITODD$^{\ast}$    & HB$^{\ast}$       & YCB-V             & Avg.\\
%   \toprule
%   {\bf PFA + Ours}            &         & RGB         & {\bf 0.876}       & 0.832             & {\bf 0.890}       & {\bf 0.689}       & 0.484             & 0.879             & 0.771             & 0.774\\
%   PFA~\cite{pfa}              &         & RGB         & 0.819             & -                 &   -               &   -               &   -               & -                 & 0.739             &    -       \\
%   SurfEmb~\cite{surfemb}      &         & RGB         & 0.851             & {\bf 0.857}       & 0.889             & 0.678             & {\bf 0.552}       & {\bf 0.888}       & {\bf 0.773}       & {\bf 0.784}     \\
%   Cosypose~\cite{cosypose}    &         & RGB         & 0.812             & 0.761             & 0.847             & 0.675             & 0.300             & 0.721             & 0.653             & 0.681     \\
%   CDPNv2~\cite{cdpn}          &         & RGB         & 0.815             & 0.579             & 0.797             & 0.582             & 0.161             & 0.845             & 0.511             & 0.613     \\
%   \midrule
%   {\bf PFA+Ours}              & \cmark  & RGB         & {\bf 0.876}       & {\bf 0.877}       & {\bf 0.978}       & {\bf 0.689}       & {\bf 0.484}       & {\bf 0.879}       & {\bf 0.856}        & {\bf 0.806}\\
%   PFA~\cite{pfa}              & \cmark  & RGB         & 0.819             & -                 & -                 & -                 & -                 & -                 & 0.810                 & - \\
%   CIR~\cite{coupled_iterative}& \cmark  & RGB         & 0.831             & 0.798             & -                 &  -                &  -                &   -               & 0.852             & -     \\
%   Cosypose~\cite{cosypose}    & \cmark  & RGB         & 0.812             & 0.821             & 0.973             & 0.675             & 0.300             & 0.721             & 0.850             & 0.736\\
%   CDPNv2~\cite{cdpn}          & \cmark  & RGB         & 0.815             & 0.620             & 0.925             & 0.582             & 0.161             & 0.845             & 0.631             & 0.654 \\
%   \midrule
%   {\bf PFA+Ours}              &         & RGB-D       & {\bf 0.890}       & 0.833             & {\bf 0.929}       & {\bf 0.702}       & 0.498             & 0.888             & {\bf 0.819}        & {\bf 0.794}\\
%   PFA~\cite{pfa}              &         & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.793                 & - \\
%   SurfEmb~\cite{surfemb}      &         & RGB-D       & 0.856             & {\bf 0.859}       & 0.905             & 0.680             & {\bf 0.560}       & {\bf 0.893}       & 0.792                 & 0.792     \\
%   CDPNv2+ICP~\cite{cdpn}      &         & RGB-D       & 0.731             & 0.488             & 0.829             & 0.459             & 0.184             & 0.749             & 0.483                 & 0.560 \\
%   \midrule
%   {\bf PFA+Ours}              & \cmark  & RGB-D       & {\bf 0.890}       & {\bf 0.878}       & {\bf 0.989}       & {\bf 0.702}       & {\bf 0.498}       & {\bf 0.888}       & 0.881        & {\bf 0.818}\\
%   PFA~\cite{pfa}              & \cmark  & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.816                 & - \\
%   CIR~\cite{coupled_iterative}&\cmark   & RGB-D       & 0.824             & 0.795             & 0.991             & 0.683             & 0.370             & 0.757             & {\bf 0.885}                 &   0.758\\
%   Cosypose+ICP~\cite{cosypose}&\cmark   & RGB-D       & 0.826             & 0.767             & 0.976             & 0.666             & 0.315             & 0.737             & 0.849                 & 0.734    \\
%   CDPNv2+ICP~\cite{cdpn}      &         & RGB-D       & 0.731             & 0.516             & 0.947             & 0.459             & 0.184             & 0.749             & 0.565                 & 0.593 \\
%   \bottomrule
% \end{tabular}

\begin{tabular}{lll|lllllll|l}
  \toprule
  Method                      & Real    & Data        & LM-O$^{\ast}$     & T-LESS            & TUD-L             & IC-BIN$^{\ast}$   & ITODD$^{\ast}$    & HB$^{\ast}$       & YCB-V             & Avg.\\
  \toprule
  {\bf PFA + Ours}            &         & RGB         & {\bf 0.876}       & 0.832             & {\bf 0.890}       & {\bf 0.689}       & 0.484             & 0.879             & 0.771             & 0.774\\
  PFA                         &         & RGB         & 0.819             & -                 &   -               &   -               &   -               & -                 & 0.739             &    -       \\
  SurfEmb                     &         & RGB         & 0.851             & {\bf 0.857}       & 0.889             & 0.678             & {\bf 0.552}       & {\bf 0.888}       & {\bf 0.773}       & {\bf 0.784}     \\
  Cosypose                    &         & RGB         & 0.812             & 0.761             & 0.847             & 0.675             & 0.300             & 0.721             & 0.653             & 0.681     \\
  CDPNv2                      &          & RGB         & 0.815             & 0.579             & 0.797             & 0.582             & 0.161             & 0.845             & 0.511             & 0.613     \\
  \midrule
  {\bf PFA+Ours}              & \cmark  & RGB         & {\bf 0.876}       & {\bf 0.877}       & {\bf 0.978}       & {\bf 0.689}       & {\bf 0.484}       & {\bf 0.879}       & {\bf 0.856}        & {\bf 0.806}\\
  PFA                         & \cmark  & RGB         & 0.819             & -                 & -                 & -                 & -                 & -                 & 0.810                 & - \\
  CIR                         & \cmark  & RGB         & 0.831             & 0.798             & -                 &  -                &  -                &   -               & 0.852             & -     \\
  Cosypose                    & \cmark  & RGB         & 0.812             & 0.821             & 0.973             & 0.675             & 0.300             & 0.721             & 0.850             & 0.736\\
  CDPNv2                      & \cmark  & RGB         & 0.815             & 0.620             & 0.925             & 0.582             & 0.161             & 0.845             & 0.631             & 0.654 \\
  \midrule
  {\bf PFA+Ours}              &         & RGB-D       & {\bf 0.890}       & 0.833             & {\bf 0.929}       & {\bf 0.702}       & 0.498             & 0.888             & {\bf 0.819}        & {\bf 0.794}\\
  PFA                         &         & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.793                 & - \\
  SurfEmb                     &         & RGB-D       & 0.856             & {\bf 0.859}       & 0.905             & 0.680             & {\bf 0.560}       & {\bf 0.893}       & 0.792                 & 0.792     \\
  CDPNv2+ICP                  &         & RGB-D       & 0.731             & 0.488             & 0.829             & 0.459             & 0.184             & 0.749             & 0.483                 & 0.560 \\
  \midrule
  {\bf PFA+Ours}              & \cmark  & RGB-D       & {\bf 0.890}       & {\bf 0.878}       & {\bf 0.989}       & {\bf 0.702}       & {\bf 0.498}       & {\bf 0.888}       & 0.881        & {\bf 0.818}\\
  PFA                         & \cmark  & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.816                 & - \\
  CIR                         &\cmark   & RGB-D       & 0.824             & 0.795             & 0.991             & 0.683             & 0.370             & 0.757             & {\bf 0.885}                 &   0.758\\
  Cosypose+ICP                &\cmark   & RGB-D       & 0.826             & 0.767             & 0.976             & 0.666             & 0.315             & 0.737             & 0.849                 & 0.734    \\
  CDPNv2+ICP                  & \cmark    & RGB-D       & 0.731             & 0.516             & 0.947             & 0.459             & 0.184             & 0.749             & 0.565                 & 0.593 \\
   \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_allpose_mssd.tex <==
% \begin{tabular}{lll|lllllll|l}
%   \toprule
%   Method                      & Real              & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$    & ITODD$^{\ast}$     & HB$^{\ast}$               & YCB-V             & Avg.\\
%   \midrule
%   {\bf PFA + Ours}            &                   & RGB       & {\bf 0.712}       & 0.682             & {\bf 0.721}       & {\bf 0.589}         & 0.306             & {\bf 0.840}               & {\bf 0.623}       & {\bf 0.639}      \\
%   PFA~\cite{pfa}              &                   & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.585             &    -       \\
%   SurfEmb~\cite{surfemb}      &                   & RGB       & 0.640             & {\bf 0.686}       & 0.687             & 0.573               & {\bf 0.363}       & 0.760                     & 0.620             & 0.618      \\
%   Cosypose~\cite{cosypose}    &                   & RGB       & 0.606             & 0.589             & 0.664             & 0.559               & 0.177             & 0.634                     & 0.554             & 0.540     \\
%   CDPNv2~\cite{cdpn}          &                   & RGB       & 0.612             & 0.338             & 0.577             & 0.438               & 0.087             & 0.708                     & 0.399             & 0.451     \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark            & RGB       & {\bf 0.712}       & {\bf 0.749}       & {\bf 0.820}       & {\bf 0.589}         & {\bf 0.306}       & {\bf 0.840}               & 0.809             & {\bf 0.689}  \\
%   PFA~\cite{pfa}              & \cmark            & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.742             &    -       \\
%   CIR~\cite{coupled_iterative}& \cmark            & RGB       & 0.633             & 0.684             & -                 &  -                  & -                 & -                         & {\bf 0.835}       & -         \\
%   Cosypose~\cite{cosypose}    & \cmark            & RGB       & 0.606             & 0.695             & 0.807             & 0.559               & 0.177             & 0.634                     & 0.842             & 0.617    \\
%   CDPNv2~\cite{cdpn}          & \cmark            & RGB       & 0.612             & 0.426             & 0.793             & 0.438               & 0.087             &0.708                      & 0.570             & 0.519\\
%   \midrule
%   {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.807}       & {\bf 0.930}       & {\bf 0.692}         & 0.495             & {\bf 0.879}               & {\bf 0.867}       & {\bf 0.788}      \\
%   PFA~\cite{pfa}              & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.842            &    -       \\
%   SurfEmb~\cite{surfemb}      & \cmark            & RGB-D     & 0.809             & 0.829             & 0.891             & 0.677               & {\bf 0.558}       & 0.875                     & 0.849             & 0.784      \\
%   CDPNv2+ICP~\cite{cdpn}      & \cmark            & RGB-D     & 0.689             & 0.449             & 0.847             & 0.458               & 0.206             & 0.757                     & 0.603             & 0.573    \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.856}       & {\bf 0.986}       & {\bf 0.692}         & {\bf 0.495}       & {\bf 0.879}               & 0.920             & {\bf 0.810}      \\
%   PFA~\cite{pfa}              & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.852             &    -       \\
%   CIR~\cite{coupled_iterative}& \cmark            & RGB-D     & 0.778             & 0.773             & 0.991             & 0.688               & 0.379             & 0.753                     & {\bf 0.924}       & 0.755 \\ 
%   Cosypose+ICP~\cite{cosypose}&\cmark             & RGB-D     & 0.748             & 0.749             & 0.972             & 0.652               & 0.341             & 0.719                     & 0.903             & 0.726  \\
%   CDPNv2+ICP~\cite{cdpn}      & \cmark            & RGB-D     & 0.689             & 0.489             & 0.962             & 0.458               & 0.206             & 0.757                     & 0.701             & 0.609    \\
%   \bottomrule
% \end{tabular}


\begin{tabular}{lll|lllllll|l}
  \toprule
  Method                      & Real              & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$    & ITODD$^{\ast}$     & HB$^{\ast}$               & YCB-V             & Avg.\\
  \midrule
  {\bf PFA + Ours}            &                   & RGB       & {\bf 0.712}       & 0.682             & {\bf 0.721}       & {\bf 0.589}         & 0.306             & {\bf 0.840}               & {\bf 0.623}       & {\bf 0.639}      \\
  PFA                         &                   & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.585             &    -       \\
  SurfEmb                     &                   & RGB       & 0.640             & {\bf 0.686}       & 0.687             & 0.573               & {\bf 0.363}       & 0.760                     & 0.620             & 0.618      \\
  Cosypose                    &                   & RGB       & 0.606             & 0.589             & 0.664             & 0.559               & 0.177             & 0.634                     & 0.554             & 0.540     \\
  CDPNv2                      &                   & RGB       & 0.612             & 0.338             & 0.577             & 0.438               & 0.087             & 0.708                     & 0.399             & 0.451     \\
  \midrule
  {\bf PFA + Ours}            & \cmark            & RGB       & {\bf 0.712}       & {\bf 0.749}       & {\bf 0.820}       & {\bf 0.589}         & {\bf 0.306}       & {\bf 0.840}               & 0.809             & {\bf 0.689}  \\
  PFA                         & \cmark            & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.742             &    -       \\
  CIR                         & \cmark            & RGB       & 0.633             & 0.684             & -                 &  -                  & -                 & -                         & {\bf 0.835}       & -         \\
  Cosypose                    & \cmark            & RGB       & 0.606             & 0.695             & 0.807             & 0.559               & 0.177             & 0.634                     & 0.842             & 0.617    \\
  CDPNv2                      & \cmark            & RGB       & 0.612             & 0.426             & 0.793             & 0.438               & 0.087             &0.708                      & 0.570             & 0.519\\
  \midrule
  {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.807}       & {\bf 0.930}       & {\bf 0.692}         & 0.495             & {\bf 0.879}               & {\bf 0.867}       & {\bf 0.788}      \\
  PFA                         & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.842            &    -       \\
  SurfEmb                     & \cmark            & RGB-D     & 0.809             & 0.829             & 0.891             & 0.677               & {\bf 0.558}       & 0.875                     & 0.849             & 0.784      \\
  CDPNv2+ICP                  & \cmark            & RGB-D     & 0.689             & 0.449             & 0.847             & 0.458               & 0.206             & 0.757                     & 0.603             & 0.573    \\
  \midrule
  {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.856}       & {\bf 0.986}       & {\bf 0.692}         & {\bf 0.495}       & {\bf 0.879}               & 0.920             & {\bf 0.810}      \\
  PFA                         & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.852             &    -       \\
  CIR                      & \cmark            & RGB-D     & 0.778             & 0.773             & 0.991             & 0.688               & 0.379             & 0.753                     & {\bf 0.924}       & 0.755 \\ 
  Cosypose+ICP                &\cmark             & RGB-D     & 0.748             & 0.749             & 0.972             & 0.652               & 0.341             & 0.719                     & 0.903             & 0.726  \\
  CDPNv2+ICP                  & \cmark            & RGB-D     & 0.689             & 0.489             & 0.962             & 0.458               & 0.206             & 0.757                     & 0.701             & 0.609    \\
  \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_allpose_vsd.tex <==
% \begin{tabular}{lll|lllllll|l}
%   \toprule
%   Method                      & Real        & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$   & ITODD$^{\ast}$      & HB$^{\ast}$         & YCB-V             & Avg.\\
%   \midrule
%   {\bf PFA + Ours}            &             & RGB       & {\bf 0.559}       & {\bf 0.643}       & {\bf 0.594}       & {\bf 0.521}       & 0.269               & {\bf 0.804}         & {\bf 0.550}       & {\bf 0.563}     \\
%   PFA~\cite{pfa}              &             & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.522             &   -       \\
%   SurfEmb~\cite{surfemb}      &             & RGB       & 0.497             & 0.661             & 0.569             & 0.514             & {\bf 0.324}         & 0.725               & 0.548             & 0.548     \\
%   Cosypose~\cite{cosypose}    &             & RGB       & 0.480             & 0.571             & 0.544             & 0.515             & 0.172               & 0.613               & 0.516             & 0.487  \\
%   CDPNv2~\cite{cdpn}          &             & RGB       & 0.445             & 0.303             & 0.391             & 0.399             & 0.059               & 0.614               & 0.260             & 0.353     \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark      & RGB       & {\bf 0.559}       & {\bf 0.709}       & {\bf 0.719}       & {\bf 0.521}       & {\bf 0.269}         & {\bf 0.804}         & 0.751             & {\bf 0.619} \\
%   PFA~\cite{pfa}              & \cmark      & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.694             &   -       \\
%   CIR~\cite{coupled_iterative}& \cmark      & RGB       & 0.501             & 0.663             & -                 & -                 & -                   & -                   & {\bf 0.783}       & -     \\
%   Cosypose~\cite{cosypose}    & \cmark      & RGB       & 0.480             & 0.669             & 0.689             & 0.515             & 0.172               & 0.613               & 0.772             & 0.559  \\
%   % SurfEmb~\cite{surfemb}      & \cmark             & RGB       & 0.497             & -                 & -                 & 0.514                     & 0.324                     &0.725                      & -                 & -     \\
%   CDPNv2~\cite{cdpn}          & \cmark      & RGB       & 0.445             & 0.386             & 0.597             & 0.399             & 0.059               & 0.614               & 0.396             & 0.414 \\
%   \midrule
%   {\bf PFA + Ours}            &             & RGB-D     & {\bf 0.658}       & 0.764             & {\bf 0.821}       & {\bf 0.636}       & {\bf 0.413}         & {\bf 0.839}         & {\bf 0.792}       & {\bf 0.703}     \\
%   PFA~\cite{pfa}              &             & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.775             &   -       \\
%   SurfEmb~\cite{surfemb}      &             & RGB-D     & 0.615             & {\bf 0.797}       & 0.767             & 0.621             & 0.497               & 0.829               & 0.757             & 0.698     \\
%   CDPNv2+ICP~\cite{cdpn}      &             & RGB-D     & 0.469             & 0.368             & 0.698             & 0.433             & 0.168               & 0.629               & 0.511             & 0.468     \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark      & RGB-D     & {\bf 0.658}       & {\bf 0.816}       & 0.904             & 0.636             & {\bf 0.413}         & {\bf 0.839}         & 0.863             & {\bf 0.733}     \\
%   PFA~\cite{pfa}              & \cmark      & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.803             &   -       \\
%   CIR~\cite{coupled_iterative}& \cmark      & RGB-D     & 0.601             & 0.760             & {\bf 0.920}       & {\bf 0.656}       & 0.394               & 0.760               & {\bf 0.871}       & 0.709\\
%   % SurfEmb~\cite{surfemb}      \cmark&             & R-DGB      & 0.615             & -                 & -                 & 0.621                     & 0.497                     & 0.829                     & -                 & 0.698     \\
%   Cosypose+ICP~\cite{cosypose}& \cmark      & RGB-D     & 0.567             & 0.587             & 0.869             & 0.624             & 0.282               & 0.679               & 0.831             & 0.634\\
%   CDPNv2+ICP~\cite{cdpn}      & \cmark      & RGB-D     & 0.469             & 0.385             & 0.832             & 0.433             & 0.168               & 0.629               & 0.590             & 0.501     \\
%   \bottomrule
% \end{tabular}


\begin{tabular}{lll|lllllll|l}
  \toprule
  Method                      & Real        & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$   & ITODD$^{\ast}$      & HB$^{\ast}$         & YCB-V             & Avg.\\
  \midrule
  {\bf PFA + Ours}            &             & RGB       & {\bf 0.559}       & {\bf 0.643}       & {\bf 0.594}       & {\bf 0.521}       & 0.269               & {\bf 0.804}         & {\bf 0.550}       & {\bf 0.563}     \\
  PFA                         &             & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.522             &   -       \\
  SurfEmb                     &             & RGB       & 0.497             & 0.661             & 0.569             & 0.514             & {\bf 0.324}         & 0.725               & 0.548             & 0.548     \\
  Cosypose                    &             & RGB       & 0.480             & 0.571             & 0.544             & 0.515             & 0.172               & 0.613               & 0.516             & 0.487  \\
  CDPNv2                      &             & RGB       & 0.445             & 0.303             & 0.391             & 0.399             & 0.059               & 0.614               & 0.260             & 0.353     \\
  \midrule
  {\bf PFA + Ours}            & \cmark      & RGB       & {\bf 0.559}       & {\bf 0.709}       & {\bf 0.719}       & {\bf 0.521}       & {\bf 0.269}         & {\bf 0.804}         & 0.751             & {\bf 0.619} \\
  PFA                         & \cmark      & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.694             &   -       \\
  CIR                         & \cmark      & RGB       & 0.501             & 0.663             & -                 & -                 & -                   & -                   & {\bf 0.783}       & -     \\
  Cosypose                    & \cmark      & RGB       & 0.480             & 0.669             & 0.689             & 0.515             & 0.172               & 0.613               & 0.772             & 0.559  \\
  % SurfEmb~\cite{surfemb}      & \cmark             & RGB       & 0.497             & -                 & -                 & 0.514                     & 0.324                     &0.725                      & -                 & -     \\
  CDPNv2                      & \cmark      & RGB       & 0.445             & 0.386             & 0.597             & 0.399             & 0.059               & 0.614               & 0.396             & 0.414 \\
  \midrule
  {\bf PFA + Ours}            &             & RGB-D     & {\bf 0.658}       & 0.764             & {\bf 0.821}       & {\bf 0.636}       & 0.413              & {\bf 0.839}         & {\bf 0.792}       & {\bf 0.703}     \\
  PFA                         &             & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.775             &   -       \\
  SurfEmb                     &             & RGB-D     & 0.615             & {\bf 0.797}       & 0.767             & 0.621             & {\bf 0.497}         & 0.829               & 0.757             & 0.698     \\
  CDPNv2+ICP                  &             & RGB-D     & 0.469             & 0.368             & 0.698             & 0.433             & 0.168               & 0.629               & 0.511             & 0.468     \\
  \midrule
  {\bf PFA + Ours}            & \cmark      & RGB-D     & {\bf 0.658}       & {\bf 0.816}       & 0.904             & 0.636             & {\bf 0.413}         & {\bf 0.839}         & 0.863             & {\bf 0.733}     \\
  PFA                         & \cmark      & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.803             &   -       \\
  CIR                         & \cmark      & RGB-D     & 0.601             & 0.760             & {\bf 0.920}       & {\bf 0.656}       & 0.394               & 0.760               & {\bf 0.871}       & 0.709\\
  % SurfEmb~\cite{surfemb}      \cmark&             & R-DGB      & 0.615             & -                 & -                 & 0.621                     & 0.497                     & 0.829                     & -                 & 0.698     \\
  Cosypose+ICP                & \cmark      & RGB-D     & 0.567             & 0.587             & 0.869             & 0.624             & 0.282               & 0.679               & 0.831             & 0.634\\
  CDPNv2+ICP                  & \cmark      & RGB-D     & 0.469             & 0.385             & 0.832             & 0.433             & 0.168               & 0.629               & 0.590             & 0.501     \\
  \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_coco_cityscapes.tex <==
\begin{tabular}{lccc}
    \toprule
    Method                        & AP        & AP$_{50}$ & AP$_{75}$       \\
    \midrule
    FCOS\cite{fcosv2}             & 38.9      &  \underline{57.5}     & 42.2          \\ 
    ATSS\cite{ATSS}             & 39.2      &  57.3     & 42.4          \\ 
    PAA\cite{PAA}                 & {\bf 40.4}      &  {\bf 58.4}     & {\bf 43.9}         \\
    % AutoAssign\cite{autoassign}  & 40.4      &  59.6     & 43.7         \\
    \textbf{Ours}              & \underline{40.0}      &  57.1     & \underline{43.4}      \\
    % \midrule
    % \multirow{5}{*}{Cityscapes} & FCOS~\cite{fcosv2}                &38.0          & 63.1           & 38.6         \\ 
    %     ～                      & ATSS~\cite{ATSS}                  &39.5          & 63.9           & 40.3          \\ 
    %      ～                      &PAA~\cite{PAA}                    &40.0          & \textbf{65.4}  & \textbf{40.8}  \\ 
    %       ～                     &   AutoAssign~\cite{autoassign}   &29.5          & 50.7           & 29.3                     \\
    %                             &\textbf{RADet}                 &\textbf{40.2} & 64.6           & 40.1             \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_detect_more.tex <==
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
%     \multirow{2}{*}{Data}    & \multicolumn{2}{c|}{{\bf Ours}}    &  \multicolumn{2}{c|}{FCOSv2} & \multicolumn{2}{c}{Mask R-CNN} \\
%     ~       & AP$_{50}$     & AP$_{75}$         & AP$_{50}$     & AP$_{75}$      & AP$_{50}$     & AP$_{75}$ \\
%     \midrule
%     LM-O    &{\bf 94.2}     &{\bf 80.7}         &   90.0        & 62.8          &87.2           &  64.7\\
%     T-LESS  & 88.9          & {\bf 86.4}        &{\bf 89.1}          & 80.6          &   83.9        &  75.3  \\
%     TUD-L   & {\bf 100.0}         & {\bf 97.9}        & {\bf 100.0}       & 97.8          & {\bf 100.0}       &    96.8    \\
%     IC-BIN  & {\bf 88.2}          &  {\bf 75.9}       &   50.0        & 27.1          & 74.6          & 39.8   \\
%     ITODD   & {\bf 62.3}    & {\bf 55.4}        & 40.5          & 34.0         & 50.2          & 40.5  \\
%     HB      &{\bf 89.7}     & {\bf 81.7}        &  81.9         & 63.8          & 86.8          & 69.3       \\
%     YCB-V   & {\bf 99.4}    & {\bf 97.4}        & 98.6          & 89.1          &  92.7         & 84.2       \\
%     Avg.    & {\bf 89.0}    & {\bf 82.2}         & 78.6         & 65.0        & 82.2          & 67.2      \\
%     \bottomrule
% \end{tabular}  


% \begin{tabular}{c|ccc|ccc|ccc}
%   \toprule
%   \multirow{2}{*}{Data}    & \multicolumn{3}{c|}{AP}                        &  \multicolumn{3}{c|}{AP$_{50}$}   & \multicolumn{3}{c}{AP$_{75}$} \\
% %   ~                        & Ours & FCOSv2  & Mask R-CNN                    & Ours & FCOSv2  & Mask R-CNN       & Ours & FCOSv2  & Mask R-CNN\\
%     ~           & {\bf Ours} & ~\cite{fcosv2}  & ~\cite{maskrcnn}    & {\bf Ours} & ~\cite{fcosv2}  & ~\cite{maskrcnn} & {\bf Ours} & ~\cite{fcosv2}  & ~\cite{maskrcnn}\\
%   \midrule
%   LM-O                     & {\bf 67.5} &57.0&56.6&{\bf 94.2}     & 90.0          & 87.2          &{\bf 80.7}     & 62.8  & 64.7\\
%   T-LESS                   & {\bf 79.8} &75.0&69.3& 88.9          & {\bf 89.1}    & 83.9          & {\bf 86.4}    & 80.6  & 75.3  \\
%   TUD-L                    & {\bf 86.6} &86.0&82.6& {\bf 100.0}   & {\bf 100.0}   & {\bf 100.0}   & {\bf 97.9}    & 97.8  & 96.8    \\
%   IC-BIN                   & {\bf 63.8 }&27.2&40.1 & {\bf 88.2}    & 50.0          & 74.6          & {\bf 75.9}    & 27.1  & 39.8   \\
%   ITODD                    & {\bf 48.6} &30.4&36.5& {\bf 62.3}    & 40.5          & 50.2          & {\bf 55.4}    & 34.0  & 40.5  \\
%   HB                       &{\bf 73.5}  &60.4&63.5 &{\bf 89.7}     & 81.9          & 86.8          & {\bf 81.7}    & 63.8  & 69.3       \\
%   YCB-V                    &{\bf 85.0}  &80.0& 74.5& {\bf 99.4}    & 98.6          & 92.7          & {\bf 97.4}    & 89.1  & 84.2       \\
%   Avg.                     &{\bf 72.1}  &66.7&60.5& {\bf 89.0}    & 78.6          & 82.2          & {\bf 82.2}    & 65.0  & 67.2      \\
%   \bottomrule
% \end{tabular}


\begin{tabular}{cccc}
  \toprule
  Data        & {\bf Ours}        & \cite{fcosv2}        & ~\cite{maskrcnn}    \\
  \midrule
  \multicolumn{4}{c}{\textit{AP}}\\
  \midrule
  LM-O                     & {\bf 67.5} &57.0&56.6   \\
  T-LESS                   & {\bf 79.8} &75.0&69.3     \\
  TUD-L                    & {\bf 86.6} &86.0&82.6       \\
  IC-BIN                   & {\bf 63.8 }&27.2&40.1      \\
  ITODD                    & {\bf 48.6} &30.4&36.5     \\
  HB                       &{\bf 73.5}  &60.4&63.5          \\
  YCB-V                    &{\bf 85.0}  &80.0& 74.5         \\
  Avg.                     &{\bf 72.1}  &66.7&60.5         \\
  \midrule
  \multicolumn{4}{c}{\textit{AP$_{50}$}}\\
  \midrule
  LM-O                     &{\bf 94.2}     & 90.0          & 87.2        \\
  T-LESS                   & 88.9          & {\bf 89.1}    & 83.9          \\
  TUD-L                    & {\bf 100.0}   & {\bf 100.0}   & {\bf 100.0}     \\
  IC-BIN                   & {\bf 88.2}    & 50.0          & 74.6           \\
  ITODD                    & {\bf 62.3}    & 40.5          & 50.2          \\
  HB                       &{\bf 89.7}     & 81.9          & 86.8               \\
  YCB-V                    & {\bf 99.4}    & 98.6          & 92.7               \\
  Avg.                     & {\bf 89.0}    & 78.6          & 82.2              \\
  \midrule
  \multicolumn{4}{c}{\textit{AP$_{75}$}}\\
  \midrule
  LM-O                    &{\bf 80.7}     & 62.8  & 64.7\\
  T-LESS                  & {\bf 86.4}    & 80.6  & 75.3  \\
  TUD-L                   & {\bf 97.9}    & 97.8  & 96.8    \\
  IC-BIN                   & {\bf 75.9}    & 27.1  & 39.8   \\
  ITODD                   & {\bf 55.4}    & 34.0  & 40.5  \\
  HB                       & {\bf 81.7}    & 63.8  & 69.3       \\
  YCB-V                    & {\bf 97.4}    & 89.1  & 84.2       \\
  Avg.                    & {\bf 82.2}    & 65.0  & 67.2      \\
\bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_detector.tex <==
% \begin{tabular}{cc|ccccccc|c}
%     \toprule
%     Method                      & Real          & LM-O          & T-LESS        & TUD-L         & IC-BIN        & ITODD         & HB            & YCB-V         & Avg.\\
%     \midrule
%     \textbf{RADet}              &               & \textbf{67.5} & \textbf{73.4} & \textbf{66.3} & \textbf{63.8} &\textbf{48.6}  &\textbf{73.5}& \textbf{73.5}& \textbf{66.7}   \\ 
%     % \textbf{RADet-nofusion}          &               & 67.1          & 70.5          & 65.3          & 63.6          & 48.1          & 73.2          & 71.4      & 65.6 \\
%     Mask R-CNN~\cite{maskrcnn}  &               & 56.6          & 67.1          & 66.4          & 40.1          & 36.5         & 63.5         & 59.4         & 55.7     \\
%     FCOS~\cite{fcosv1}          &               & 57.0          & 62.5          & 58.5          & 27.2          & 30.4         & 60.4         & 59.0         & 50.7     \\
%     \midrule
%     \textbf{RADet}              & \checkmark    & \textbf{67.5} & \textbf{79.8}& \textbf{86.6}& \textbf{63.8}& \textbf{48.6}& \textbf{73.5}& \textbf{85.0}& \textbf{72.1}   \\
%     % \textbf{RADet-nofusion}          & \checkmark    & 67.1          & 79.7          & 86.3          & 63.6          & 48.1      & 73.2          & 85.0          & 71.8 \\
%     FCOS~\cite{fcosv1}          & \checkmark    & 57.0         & 75.0         & 86.0         & 27.2         & 30.4         & 60.4         & 80.0         & 66.7     \\
%     Mask R-CNN~\cite{maskrcnn}  & \checkmark    & 56.6         & 69.3         & 82.6         & 40.1         & 36.5         & 63.5         & 74.5         & 60.5     \\   
%     \bottomrule
    
% \end{tabular}

\begin{tabular}{l|ccccccc|c}
    \toprule
    Method                      & LM-O          & T-LESS        & TUD-L         & IC-BIN        & ITODD         & HB            & YCB         & Avg.\\
    \midrule
    \textbf{Ours}              & \textbf{67.5} & \textbf{79.8}& \textbf{86.6}& \textbf{63.8}& \textbf{48.6}& \textbf{73.5}& \textbf{85.0}& \textbf{72.1}   \\
    % \textbf{RADet-nofusion}          & \checkmark    & 67.1          & 79.7          & 86.3          & 63.6          & 48.1      & 73.2          & 85.0          & 71.8 \\
    FCOSv2~\cite{fcosv2}          & 57.0         & 75.0         & 86.0         & 27.2         & 30.4         & 60.4         & 80.0         & 66.7     \\
    Mask R-CNN~\cite{maskrcnn}  & 56.6         & 69.3         & 82.6         & 40.1         & 36.5         & 63.5         & 74.5         & 60.5     \\ 
    \bottomrule
    
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_detector_ap50.tex <==
\begin{tabular}{c|ccccccc|c}
    \toprule
    Method      & LM-O       & T-LESS   & TUD-L     & IC-BIN    & ITODD     & HB        & YCB-V     & Avg.  \\
    \midrule
    Ours        & {\bf 94.2}& 88.9      & {\bf 100.0} & {\bf 88.2}& {\bf 62.3}& {\bf 89.7}& {\bf 99.4}&{\bf 89.0}     \\
    FCOSv2      & 90.0      & {\bf 89.1}& {\bf 100.0} & 50.0      & 40.5      & 81.9      & 98.6      &78.6  \\
    Mask R-CNN  & 87.2      & 83.9      & {\bf 100.0} & 74.6      & 50.2      & 86.8      & 92.7      &82.2    \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_detector_ap75.tex <==
\begin{tabular}{c|ccccccc|c}
    \toprule
    Method      & LM-O          & T-LESS        & TUD-L         & IC-BIN    & ITODD     & HB        & YCB-V         & Avg.  \\
    \midrule
    Ours        & {\bf 80.7}    & {\bf 86.4}    & {\bf 97.9}    & {\bf 75.9}& {\bf 55.4}& {\bf 81.7}& {\bf 97.4}    & {\bf 82.2}     \\
    FCOSv2      & 62.8          & 80.6          & 97.8          & 27.1      & 34.0      & 63.8      & 89.1          & 65.0   \\
    Mask R-CNN  & 64.7          & 75.3          & 96.8          & 39.8      & 40.5      & 69.3      & 84.2          & 67.2  \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_estimator.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Method                      & Real          & LM-O              & T-LESS            & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V     & Avg.\\
    \midrule
    \textbf{WDR+Ours}          &               & 0.614             & \textbf{0.588}    & \textbf{0.623}    & 0.514             & \textbf{0.247}    & 0.618             & \textbf{0.605}    & \textbf{0.544} \\
    CDPNv2~\cite{cdpn}          &               & \textbf{0.624}    & 0.407             & 0.588             & 0.473             & 0.102             & \textbf{0.722}    & 0.390             & 0.472 \\
    EPOS~\cite{epos}            &               & 0.547             & 0.467             & 0.558             & 0.363             & 0.186             & 0.580             & 0.499             & 0.457  \\
    CosyPose\dag~\cite{cosypose}&               & 0.533             & 0.520             & 0.582             & \textbf{0.515}    & 0.129             & 0.334             & 0.333             & 0.421 \\
    \midrule
    \textbf{WDR+Ours}          & \cmark    & 0.614             & \textbf{0.678}    & \textbf{0.796}    & 0.514             & \textbf{0.247}    & 0.618             & \textbf{0.722}    & \textbf{0.598} \\
    CDPNv2~\cite{cdpn}          & \cmark    & \textbf{0.624}    & 0.478             & 0.772             & 0.473             & 0.102             & \textbf{0.722}    & 0.532             & 0.529 \\
    CosyPose\dag~\cite{cosypose}& \cmark    & 0.533             & 0.616             & 0.742             & \textbf{0.515}    & 0.129             & 0.334             & 0.655             & 0.503 \\
    Pix2Pose~\cite{pix2pose}    & \cmark    & 0.363             & 0.344             & 0.420             & 0.226             & 0.134             & 0.346             & 0.446             & 0.342 \\
    % SO-Pose~\cite{so-pose}      & \checkmark    & 0.613             & -                 & -                 & -                 & -                 &   -               & 0.715             & -      \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_hb_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method  &  Avg.     & MSPD      & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.840}& 0.879     & 0.840     &{\bf 0.804}\\
    SurfEmb         & 0.791     &{\bf 0.888}&{\bf 0.760}& 0.725 \\
    Cosypose        & 0.656     & 0.721     & 0.634     & 0.613 \\
    CDPNv2          & 0.722     & 0.845     & 0.708     & 0.614 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.869}& 0.888     &{\bf 0.879}& {\bf 0.839} \\
    SurfEmb         & 0.866     &{\bf 0.893}&0.875      & 0.829 \\
    CIR             &{\bf 0.757}& 0.757     & 0.753     & 0.760 \\
    Cosypose+ICP    & 0.712     & 0.737     & 0.717     & 0.679 \\
    CDPNv2+ICP      & 0.712     & 0.749     & 0.757     & 0.629 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_icbin_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method  &  Avg.     & MSPD      & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.600}&{\bf 0.689}& 0.589     &{\bf 0.521}\\
    SurfEmb         & 0.588     & 0.678     &{\bf 0.573}& 0.514 \\
    Cosypose        & 0.473     & 0.675     & 0.559     & 0.515 \\
    CDPNv2          & 0.226     & 0.582     & 0.438     & 0.399 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.676}&{\bf 0.702}&{\bf 0.692}& 0.636 \\
    SurfEmb         & 0.659     & 0.680     &0.677      & 0,621 \\
    CIR             &{\bf 0.676}& 0.683     & 0.688     &{\bf 0.656} \\
    Cosypose+ICP    & 0.647     & 0.666     & 0.652     & 0.624 \\
    CDPNv2+ICP      & 0.450     & 0.459     & 0.458     & 0.433 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_itodd_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method  &  Avg.     & MSPD      & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  & 0.353     & 0.484     & 0.306     & 0.269 \\
    SurfEmb         &{\bf 0.413}&{\bf 0.552}&{\bf 0.363}&{\bf 0.324} \\
    Cosypose        & 0.216     & 0.300     & 0.177     & 0.172 \\
    CDPNv2          & 0.067     & 0.161     & 0.087     & 0.059 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  & 0.460     & 0.498     & 0.495     & 0.413 \\
    SurfEmb         &{\bf 0.538}&{\bf 0.560}&{\bf 0.558}&{\bf 0.497} \\
    CIR             & 0.381     & 0.370     & 0.379     & 0.394 \\
    Cosypose+ICP    & 0.313     & 0.315     & 0.341     & 0.282 \\
    CDPNv2+ICP      & 0.186     & 0.184     & 0.206     & 0.168 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_lmo_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method  &  Avg.     & MSPD      & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.715}&{\bf 0.876}&{\bf 0.712}&{\bf 0.559} \\
    PFA             & 0.674     & 0.819     & 0.673     & 0.531 \\
    SurfEmb         & 0.663     & 0.851     & 0.649     & 0.497 \\
    CIR             & 0.655     & 0.831     & 0.633     & 0.501 \\
    Cosypose        & 0.633      & 0.812     & 0.606     & 0.480 \\
    CDPNv2          & 0.624     & 0.815     & 0.612     & 0.445 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}} \\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.797}&{\bf 0.890}&{\bf 0.712}&{\bf 0.559} \\
    PFA             & 0.751     & 0.835     & 0.673     & 0.531 \\
    SurfEmb         & 0.760     & 0.856     & 0.649     & 0.497 \\
    CIR             & 0.734     & 0.824     & 0.633     & 0.501 \\
    Cosypose+ICP    & 0.714     & 0.826     & 0.606     & 0.480 \\
    CDPNv2+ICP      & 0.630     & 0.731     & 0.612     & 0.445 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_tless_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method          & Avg.     & MSPD        & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}}\\
    \midrule
    {\bf PFA+Ours}  & 0.719     & 0.832     & 0.682     & 0.643 \\
    SurfEmb         &{\bf 0.735}&{\bf 0.857}&{\bf 0.686}& {\bf 0.661} \\
    Cosypose        & 0.640      & 0.761     & 0.589     & 0.571 \\
    CDPNv2          & 0.407      & 0.579     & 0.338     & 0.303 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (Real+PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.778}&{\bf 0.877}&{\bf 0.749}&{\bf 0.709} \\
    SurfEmb         &  0.770    & -         & -         & - \\
    CIR             &  0.715    & 0.798     & 0.684     & 0.663\\
    Cosypose        &  0.728    & 0.821     & 0.695     & 0.669 \\
    CDPNv2          &  0.478    & 0.620     & 0.426     & 0.386 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}}\\
    \midrule
    {\bf PFA+Ours}  & 0.801     & 0.833     & 0.807     & 0.764 \\
    SurfEmb         &{\bf 0.828}&{\bf 0.859}&{\bf 0.829}& {\bf 0.797} \\
    CDPNv2+ICP      & 0.435     & 0.488     & 0.449     & 0.368 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (Real+PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.850}&{\bf 0.878}&{\bf 0.856}&{\bf 0.816} \\
    SurfEmb         & 0.833     & -         & -         & - \\
    CIR             & 0.776     & 0.795     & 0.773     & 0.760\\
    Cosypose+ICP    & 0.701     & 0.767     & 0.749     & 0.587 \\
    CDPNv2+ICP      & 0.464     & 0.516     & 0.489     & 0.385 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_tudl_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method          & Avg.     & MSPD        & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.733}&{\bf 0.890}&{\bf 0.721}& {\bf 0.594} \\
    SurfEmb         & 0.715     & 0.889     & 0.687     & 0.569 \\
    Cosypose        & 0.685     & 0.847     & 0.664    & 0.544 \\
    CDPNv2          & 0.588     & 0.797     & 0.577     & 0.391 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (Real+PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.839}&{\bf 0.978}&{\bf 0.820}&{\bf 0.719} \\
    SurfEmb         & 0.805     & -         & -         & - \\
    Cosypose        & 0.823     & 0.973     &0.807      &0.689 \\
    CDPNv2          & 0.772     & 0.925     & 0.793     & 0.597 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.894}&{\bf 0.929}&{\bf 0.930}& {\bf 0.821} \\
    SurfEmb         & 0.854     & 0.905     & 0.891     & 0.767 \\
    CDPNv2+ICP      & 0.791     & 0.829     & 0.847     & 0.698 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (Real+PBR)}}\\
    \midrule
    {\bf PFA+Ours}  & 0.960     & 0.989     & 0.986     & 0.904 \\
    CIR             &{\bf 0.968}&{\bf 0.991}&{\bf 0.991}&{\bf 0.920}\\
    SurfEmb         & 0.933     & -         & -         & - \\
    Cosypose+ICP    & 0.939     & 0.976     & 0.972     & 0.869 \\
    CDPNv2+ICP      & 0.913     & 0.947     & 0.962     & 0.832 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_ycbv_lmo.tex <==
\begin{tabular}{c|c|cccccc}
    \toprule
        Data & Metric    &CDPNv2~\cite{cdpn}     & NCF~\cite{ncf}   & SurfEmb~\cite{surfemb}    & CIR~\cite{coupled_iterative}    &PFA~\cite{pfa}   & \textbf{RADet+PFA} \\
    \midrule
        \multirow{4}{*}{LM-O}           & MSPD          & 0.815     & -     & 0.851      & 0.831    & 0.821 &\textbf{0.876}\\
        ~                              & MSSD           & 0.612     & -     & 0.641      & 0.633    & 0.674 &\textbf{0.712} \\
        ~                              & VSD       & 0.445	    & -     & 0.497     & 0.501     & 0.531 & \textbf{0.559} \\
        ~                              & Avg.      & 0.624     & 0.632 & 0.663      & 0.655    & 0.676 & \textbf{0.715}\\
    \midrule
        \multirow{4}{*}{YCB-V}          & MSPD      & 0.511    & -      & \textbf{0.773}      & -     & 0.736      &\underline{0.771}  \\
        ~                              & MSSD      & 0.399    &-       & 0.620      & -     & 0.583      & \textbf{0.623} \\
        ~                              & VSD       & 0.260    &-       & 0.548      & -     & 0.524    & \textbf{0.550}    \\
        ~                               & Avg.      & 0.390    & \textbf{0.673}& 0.647      & -     & 0.614     & \underline{0.648}       \\
    \midrule
        \multirow{4}{*}{\makecell[c]{YCB-V\\(with Real)}}& MSPD     & 0.631 &-     & -        & \underline{0.852}    &  -        & \textbf{0.856}  \\
        ~                                             & MSSD      & 0.570 &-   &  -        & \textbf{0.835}     &    -     &\underline{0.809} \\
        ~                                             & VSD       & 0.396 &-   &  -        & \textbf{0.783}     &    -     & \underline{0.751}    \\
        ~                                           & Avg.      & 0.532 & 0.775    &  0.711    & \textbf{0.824}     &-       & \underline{0.806}       \\
    
    \bottomrule
 \end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/compare_ycbv_pose.tex <==
\begin{tabular}{lcccc}
    \toprule
    Method          & Avg.     & MSPD        & MSSD      & VSD\\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.648}& 0.771     &{\bf 0.623}& {\bf 0.550} \\
    PFA             & 0.614     & 0.739     & 0.585     & 0.522 \\
    SurfEmb         & 0.647      &{\bf 0.773}& 0.620     & 0.548 \\
    Cosypose        & 0.574     & 0.653     & 0.554     & 0.516 \\
    CDPNv2          & 0.390     & 0.511     & 0.399     & 0.260 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB (Real+PBR)}}\\
    \midrule
    {\bf PFA+Ours}  & 0.806     &{\bf 0.856}& 0.809     & 0.751 \\
    PFA             & 0.748     & 0.810     & 0.742     & 0.694 \\
    CIR             &{\bf 0.824}& 0.852     & 0.835     & {\bf 0.783}\\
    SurfEmb         & 0.711     & -         & -         & - \\
    Cosypose        & 0.821     & 0.850     &{\bf 0.842}& 0.772 \\
    CDPNv2          & 0.532     & 0.631     & 0.570     & 0.396 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (PBR)}}\\
    \midrule
    {\bf PFA+Ours}  &{\bf 0.826}&{\bf 0.819}&{\bf 0.867}& {\bf 0.792} \\
    PFA             & 0.804     & 0.793     & 0.842     & 0.775 \\
    SurfEmb         & 0.799     & 0.792     & 0.849     & 0.757 \\
    CDPNv2+ICP      & 0.532     & 0.483     & 0.603     & 0.511 \\
    \midrule
    \multicolumn{5}{c}{\textit{RGB-D (Real+PBR)}}\\
    \midrule
    {\bf PFA+Ours}  & 0.888     & 0.881     & 0.920     & 0.863 \\
    PFA             & 0.823     & 0.816     & 0.852     & 0.803 \\
    CIR             &{\bf 0.893}&{\bf 0.885}& {\bf 0.924}& {\bf 0.871}\\
    SurfEmb         & 0.824       & -         & -         & - \\
    Cosypose+ICP    & 0.861     & 0.849     & 0.903     & 0.831 \\
    CDPNv2+ICP      & 0.619     & 0.565     & 0.701     & 0.590 \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/detector_for_onestage.tex <==
\begin{tabular}{lcccc}
    \toprule
      Method          & Avg.      &  MSPD     & MSSD   & VSD  \\
    \midrule
    \multicolumn{5}{c}{on LM-O}\\
    \midrule
    WDR         & 0.544    & 0.758    & 0.501    & 0.373  \\
    WDR+Detect   & 0.614    & 0.841    & 0.559    & 0.441   \\
    EPOS        & 0.547    & 0.750    & 0.501    & 0.389     \\
    EPOS+Detect  & 0.605    & 0.832    & 0.552    & 0.431     \\
    \midrule
    \multicolumn{5}{c}{on YCB-V}\\
    \midrule
    WDR         & 0.514     & 0.632    & 0.491    & 0.420  \\
    WDR+Detect  & 0.605     & 0.694    & 0.598    & 0.522   \\
    EPOS        & 0.499     & 0.621    & 0.464    & 0.411  \\
    EPOS+Detect & 0.572     & 0.675    & 0.536    & 0.506     \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/detector_for_two_stage.tex <==
\begin{tabular}{lcccc}
    \toprule
      Method          & Avg.      &  MSPD     & MSSD   & VSD  \\
    \midrule
    % WDR + FCOS          & 0.707             & 0.785             & 0.708         & 0.629\\
    % WDR + RCNN          & 0.705             & 0.779             & 0.704         & 0.631\\
    % WDR + GT            & {\bf 0.724}       & {\bf 0.800}       & {\bf 0.723}         & {\bf 0.648} \\
    % WDR + {\bf Ours}    & \underline{0.722}     & \underline{0.798}         & {\bf 0.723}    & \underline{0.647}   \\
    WDR + {\bf Ours}    & {\bf 0.605}  & {\bf 0.694}    & {\bf 0.598}    & {\bf 0.522}    \\
    WDR + RCNN          & 0.587             & 0.673             & 0.580         & 0.508\\
    WDR + FCOSv2          & 0.585             & 0.671            & 0.578        & 0.506\\
    % WDR + GT            & {\bf 0.609}       & {\bf 0.703}       & {\bf 0.600}         & {\bf 0.523} \\ removed ambiguity
    \cmidrule{2-5}
    CDPNv2 + {\bf Ours} & {\bf 0.412}       & {\bf 0.534} & {\bf 0.428}   & {\bf 0.275}\\
    CDPNv2 + FCOSv2       & 0.402             & 0.523             & 0.416         & 0.268 \\
    CDPNv2 + RCNN       & 0.388             & 0.506             & 0.401         & 0.258\\
    % CDPNv2 + GT         & {\bf 0.412}       & {\bf 0.536}       & \underline{0.425}         & {\bf 0.275}\\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/distance_transform_acc.tex <==
\begin{tabular}{c|c}
     &  \\
    LM-O  & 
    YCB-V
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/effect_detect.tex <==
\begin{tabular}{lcccc}
    \toprule
      Method          & Avg.      &  MSPD     & MSSD   & VSD  \\
    % \midrule
    % \multicolumn{5}{c}{on LM-O}\\
    % \midrule
    % WDR         & 0.544    & 0.758    & 0.501    & 0.373  \\
    % Detect + WDR   & 0.614    & 0.841    & 0.559    & 0.441   \\
    % EPOS        & 0.547    & 0.750    & 0.501    & 0.389     \\
    % Detect + EPOS  & 0.605    & 0.832    & 0.552    & 0.431     \\
    % \midrule
    % \multicolumn{5}{c}{on YCB-V}\\
    \midrule
    WDR             & 0.514     & 0.631     & 0.492     & 0.420 \\
    % WDR (960)             & 0.558     & 0.682     & 0.543     & 0.450\\
    % WDR (1280)            & \underline{0.594}     & {\bf 0.719}     & \underline{0.587}     & \underline{0.476}\\
    WDR + FCOS          & 0.707             & 0.785             & 0.708         & 0.629\\
    WDR + RCNN          & 0.705             & 0.779             & 0.704         & 0.631\\
    WDR + GT            & {\bf 0.724}       & {\bf 0.800}       & {\bf 0.723}         & {\bf 0.648} \\
    WDR + {\bf Ours}    & \underline{0.722}     & \underline{0.798}         & {\bf 0.723}    & \underline{0.647}   \\
    \cmidrule{2-5}
    CDPNv2 + FCOS       & 0.402             & 0.523             & 0.416         & 0.268 \\
    CDPNv2 + RCNN       & 0.388             & 0.506             & 0.401         & 0.258\\
    CDPNv2 + GT         & {\bf 0.412}       & {\bf 0.536}       & \underline{0.425}         & {\bf 0.275}\\
    CDPNv2 + {\bf Ours} & {\bf 0.412}       & \underline{0.534} & {\bf 0.428}   & {\bf 0.275}\\

    % EPOS        & 0.499     & 0.621    & 0.464    & 0.411  \\
    % EPOS + {\bf Ours}  & {\bf 0.572}     & {\bf 0.675}    & {\bf 0.536}    & {\bf 0.506}     \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/efficiency.tex <==
\begin{tabular}{ccc}
    \toprule
                    & WDR(1280) & Detect+WDR\\
    \midrule
    \multicolumn{3}{c}{Testing Speed(fps)} \\
    \midrule
    LM-O            & 3.58    & 6.46\\
    YCB-V           &  2.96     & 8.71\\
    \midrule
    \multicolumn{3}{c}{Training Time(hours)}\\
    \midrule
                    & 73.42     &  18.71\\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/resolution_for_wdr.tex <==
\begin{tabular}{ccccc}
    \toprule
    resolution      & Avg.      &  MSPD     & MSSD   & VSD  \\
    % \midrule
    % \multicolumn{5}{c}{on LM-O}\\
    % \midrule
    % 640             & 0.544       &0.758    & 0.501   & 0.373  \\
    % 960             & 0.583       &0.800     & 0.541  & 0.408     \\
    % 1280            & 0.608       &0.829     & 0.566  & 0.430\\
    % \midrule
    % \multicolumn{5}{c}{on YCB-V}\\
    \midrule
    640             & 0.514     & 0.631     & 0.492     & 0.420 \\
    960             & 0.558     & 0.682     & 0.543     & 0.450\\
    1280            & 0.594     & 0.719     & 0.587     & 0.476\\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/time_report.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
        & FCOS & ATSS & PAA & AutoAssign & {\bf Ours} \\
    \midrule
        Timings & {\bf 0.67} & {\bf 0.67}  & 0.90  &  0.95        & \underline{0.80}   \\
    \bottomrule
\end{tabular}
}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/visibilty_modling_acc.tex <==
\begin{tabular}{c|ccccc}
    \toprule
    Threshold($\tau$)  & 0.1   & 0.2   & 0.3   & 0.4   & 0.5 \\
    \midrule    
    LM-O    & 60.3  & 68.8  & 63.4  & 52.7  & 48.3 \\
    YCB-V   & 58.4  & 67.3  & 72.1  & 59.6   & 52.1   \\
    \bottomrule
\end{tabular}

==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ycbv_compare.tex <==

\begin{tabular}{c|c|ccc|cc}
    \hline
    method                      & backbone               & AP           & AP$_{50}$     & AP$_{75}$     & AP$_{m}$      & AP$_{l}$     \\ \hline
    FCOS\cite{fcosv2}           & ResNet-50              & 76.6         & 94.0          &  88.8         & 72.9          &  77.0        \\ 
    ATSS\cite{ATSS}             & ResNet-50              & 76.5         & 92.5          &  89.2         & 77.7          &  76.8        \\ 
    PAA\cite{PAA}           & ResNet-50              & 77.9         & 94.5          &  88.0         &\textbf{78.1}  &  78.2        \\
    AutoAssign\cite{autoassign} & ResNet-50              & 60.6         & 76.0          &  68.0         & 64.4          &  61.2        \\ 
    \textbf{Mask}               & ResNet-50              &\textbf{79.7} &\textbf{96.3}  &\textbf{90.5}  & 74.9          & \textbf{80.1}\\ 
    \textbf{Distance}           & ResNet-50              & 78.2         & 93.2          & 90.1          & 75.8          & 78.6         \\ \hline
    FCOS\cite{fcosv2}           & ResNet-101             & 81.8         & 96.5          &  93.8         & 79.3          &  82.1     \\
    ATSS\cite{ATSS}             & ResNet-101             & 79.9         & 94.5          &  92.2         & 77.2          &  80.4     \\
    PAA\cite{PAA}           & ResNet-101             & 81.3         & 96.9          &  93.9         & 74.3          &  81.6     \\
    AutoAssign\cite{autoassign} & ResNet-101             & 65.7         & 82.1          &  75.0         & 63.6          &  65.7     \\
    \textbf{Mask}               & ResNet-101             &              &               &               &               &           \\ 
    \textbf{Mask\dag}           & ResNet-101             & 81.9         &  96.4         &  93.6         & 73.1          &  82.4    \\ 
    \textbf{Distance}           & ResNet-101             &              &               &               &               &           \\ 
    \textbf{Distance\dag}       & ResNet-101             & 80.3         &  95.1         &  91.2         & 69.5          &  80.7     \\ \hline
\end{tabular}
\caption{Ycb-video dataset}




==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ycbv_compare_mixpbr_detect.tex <==


% \rowcolors{2}{white}{gray!10}
\begin{tabular}{lccc}
    \toprule
    Method                              & AP             & AP$_{50}$     & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    \textbf{Ours}                       & {\bf 85.0}    & {\bf 99.4}    & {\bf 97.4}        \\
    PAA~\cite{PAA}                      & 83.5            & 98.3         & 93.2         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19  
    AutoAssign~\cite{autoassign}        & 83.3            & 98.1         & 91.7         \\%& 64.0$\pm$0.18          &  62.1$\pm$0.41     \\
    ATSS~\cite{ATSS}                    & 82.8            & 98.0         & 91.4         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    FCOSv2~\cite{fcosv2}                  & 80.0            & 98.6         & 89.1        \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    Faster R-CNN~\cite{faster-rcnn}     & 73.7            & 92.5         & 83.3 \\
    \bottomrule
\end{tabular}




==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ycbv_compare_r50.tex <==


% \rowcolors{2}{white}{gray!10}
\begin{tabular}{lccc}
    \toprule
    Method                              & AP             & AP$_{50}$     & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    AutoAssign~\cite{autoassign}        & 61.6            & 76.8         & 69.8         \\%& 64.0$\pm$0.18          &  62.1$\pm$0.41     \\
    FCOS~\cite{fcosv2}                  & 63.8            & 82.1         & 72.4        \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    Faster R-CNN~\cite{faster-rcnn}     & 66.1            & 87.9         & 75.5 \\
    PAA~\cite{PAA}                      & 66.9            & 86.6         & 73.8         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19     \\
    ATSS~\cite{ATSS}                    & 67.8            & 85.8         & 77.0         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    \cmidrule{2-4}
    \textbf{Ours-box}                   & 66.1            & 84.6         & 74.8 \\
    \textbf{Ours-center}                & 67.2            & 83.9         & 75.8       \\
    % \textbf{Ours-mask$^\dagger$}        & 68.8            & 86.1         & 78.4         \\ 
    \textbf{Ours-nofusion}              & 69.0              & 88.7          & 77.5\\
    \textbf{Ours}                       & \underline{69.6}& \underline{88.5}& \underline{78.7}        \\
    \textbf{Ours-oracle}              &\textbf{71.2}    & \textbf{91.7} &\textbf{79.9}\\
    % \textbf{Mask (oracle)}               & real               & \textbf{71.2}$\pm$0.27   & \textbf{91.7}$\pm$\textbf{0.08}& \textbf{79.9}$\pm$0.50\\%& 63.2$\pm$0.17          &  \textbf{71.8$\pm$0.31}    \\ 
    % \midrule
    % Faster R-CNN                & real+sync          & 77.2$\pm$0.80            &96.6$\pm$0.77           & 90.8$\pm$0.15          \\
    % FCOS                        & real+sync          & 76.6$\pm$0.83            & 94.0$\pm$0.76          &  88.8$\pm$0.83          \\%& 72.9$\pm$0.21          &  77.0$\pm$0.78        \\ 
    % ATSS                        & real+sync          & 76.3$\pm$0.24            & 92.4$\pm$0.14          &  88.4$\pm$0.82          \\%& 77.7$\pm$0.05          &  76.7$\pm$0.19        \\ 
    % PAA                         & real+sync          & 77.9$\pm$0.13            & 94.5$\pm$0.21          &  88.0$\pm$0.49          \\%&\textbf{78.1$\pm$0.91}  &  78.2$\pm$0.19        \\
    % AutoAssign                  & real+sync          & 60.6$\pm$0.11            & 76.2$\pm$0.23          &  67.8$\pm$0.18          \\%& 64.2$\pm$0.32          &  61.2$\pm$0.07        \\ 
    % \textbf{Ours}               & real+sync          & \textbf{78.2$\pm$0.07}   & \textbf{93.2$\pm$0.04} &  \textbf{90.1$\pm$0.12}          \\%& 75.8$\pm$0.67          & 78.6$\pm$0.05         \\ \hline
    % \textbf{Mask (oracle)}               & real+sync          &\textbf{79.7}$\pm$0.35 &\textbf{96.3}$\pm$0.19  &\textbf{90.5}$\pm$0.80   \\%& 74.9$\pm$0.22          & \textbf{80.1$\pm$0.30}\\ 
    \bottomrule
\end{tabular}




==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ycbv_compare_r50_mixpbr.tex <==
\begin{tabular}{ccc}
    Method              &  AP       & AP_{50}      & AP_{75}   \\
    
    {\bf Ours-box}      &           &               &           \\
    {\bf Ours-center}   &           &               &           \\
    {\bf Ours-nofusion} & 
    {\bf Ours}          & 85.0      & 99.4          & 97.4      \\
    {\bf Ours-oracle}   & 86.3      &               &           \\
\end{tabular}


\begin{tabular}{lccc}
    \toprule
    Method                              & AP             & AP$_{50}$     & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    AutoAssign~\cite{autoassign}        & 61.6            & 76.8         & 69.8         \\%& 64.0$\pm$0.18          &  62.1$\pm$0.41     \\
    FCOS~\cite{fcosv2}                  & 63.8            & 82.1         & 72.4        \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    Faster R-CNN~\cite{faster-rcnn}     & 66.1            & 87.9         & 75.5 \\
    PAA~\cite{PAA}                      & 66.9            & 86.6         & 73.8         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19     \\
    ATSS~\cite{ATSS}                    & 67.8            & 85.8         & 77.0         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    \cmidrule{2-4}
    \textbf{Ours-box}                   & 66.1            & 84.6         & 74.8 \\
    \textbf{Ours-center}                & 67.2            & 83.9         & 75.8       \\
    % \textbf{Ours-mask$^\dagger$}        & 68.8            & 86.1         & 78.4         \\ 
    \textbf{Ours-nofusion}              & 69.0              & 88.7          & 77.5\\
    \textbf{Ours}                       & \underline{69.6}& \underline{88.5}& \underline{78.7}        \\
    \textbf{Ours-oracle}              &\textbf{71.2}    & \textbf{91.7} &\textbf{79.9}\\
    % \textbf{Mask (oracle)}               & real               & \textbf{71.2}$\pm$0.27   & \textbf{91.7}$\pm$\textbf{0.08}& \textbf{79.9}$\pm$0.50\\%& 63.2$\pm$0.17          &  \textbf{71.8$\pm$0.31}    \\ 
    % \midrule
    % Faster R-CNN                & real+sync          & 77.2$\pm$0.80            &96.6$\pm$0.77           & 90.8$\pm$0.15          \\
    % FCOS                        & real+sync          & 76.6$\pm$0.83            & 94.0$\pm$0.76          &  88.8$\pm$0.83          \\%& 72.9$\pm$0.21          &  77.0$\pm$0.78        \\ 
    % ATSS                        & real+sync          & 76.3$\pm$0.24            & 92.4$\pm$0.14          &  88.4$\pm$0.82          \\%& 77.7$\pm$0.05          &  76.7$\pm$0.19        \\ 
    % PAA                         & real+sync          & 77.9$\pm$0.13            & 94.5$\pm$0.21          &  88.0$\pm$0.49          \\%&\textbf{78.1$\pm$0.91}  &  78.2$\pm$0.19        \\
    % AutoAssign                  & real+sync          & 60.6$\pm$0.11            & 76.2$\pm$0.23          &  67.8$\pm$0.18          \\%& 64.2$\pm$0.32          &  61.2$\pm$0.07        \\ 
    % \textbf{Ours}               & real+sync          & \textbf{78.2$\pm$0.07}   & \textbf{93.2$\pm$0.04} &  \textbf{90.1$\pm$0.12}          \\%& 75.8$\pm$0.67          & 78.6$\pm$0.05         \\ \hline
    % \textbf{Mask (oracle)}               & real+sync          &\textbf{79.7}$\pm$0.35 &\textbf{96.3}$\pm$0.19  &\textbf{90.5}$\pm$0.80   \\%& 74.9$\pm$0.22          & \textbf{80.1$\pm$0.30}\\ 
    \bottomrule
\end{tabular}


==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ycbv_compare_real.tex <==

\begin{tabular}{c|c|ccc|cc}
    \hline
    method                      & data                   & AP           & AP$_{50}$     & AP$_{75}$     & AP$_{m}$      & AP$_{l}$     \\ \hline
    FCOS\cite{fcosv2}           & ResNet-50              & 63.8         & 82.1          &  72.4         & 64.2          &  64.4        \\ 
    ATSS\cite{ATSS}             & ResNet-50              & 68.8         & 86.8          &  78.0         & 65.5          &  69.3        \\ 
    PAA\cite{PAA}               & ResNet-50              & 66.9         & 86.6          &  73.8         & 61.9          &  67.6        \\
    AutoAssign\cite{autoassign} & ResNet-50              & 61.6         & 76.8          &  69.8         & 64.0          &  62.1        \\ 
    \textbf{Mask\dag}           & ResNet-50              &\textbf{71.2} &\textbf{91.7}  &\textbf{79.9}  & 63.2          & \textbf{71.8} \\ 
    \textbf{Distance\dag}       & ResNet-50              & 69.6         & 88.5          &  78.7         & 63.9          &  70.0         \\ \hline
    FCOS\cite{fcosv2}           & ResNet-101             & 65.1         & 83.3          &  73.6         & 59.5          &   66.0         \\
    ATSS\cite{ATSS}             & ResNet-101             & 70.0         & 88.5          &    78.9       &  64.3         &  70.3          \\
    PAA\cite{PAA}               & ResNet-101             & 71.0         & 91.0          &    80.3       &  64.1         &  71.4           \\
    AutoAssign\cite{autoassign} & ResNet-101             &              &               &               &               &                    \\
    \textbf{Mask\dag}           & ResNet-101             &  72.4        &  91.6         &  82.9         &  63.8         &  72.9            \\ 
    \textbf{Distance\dag}       & ResNet-101             &              &               &               &               &           \\ \hline
\end{tabular}
\caption{Ycb-video real dataset}




==> Rigidity-Aware Detection for 6D Object Pose Estimation/tabs/ycbv_compare_resnext50.tex <==
\begin{tabular}{lcccc}
    \toprule
    method                      & data               & AP                                        & AP$_{50}$                    & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    Faster R-CNN                & real               & 67.0$\pm$0.15                             & 88.5$\pm$0.31                & 77.6$\pm$0.34                \\
    FCOS                        & real               & 61.0$\pm$0.19                             & 80.3$\pm$0.33                & 72.4$\pm$0.09         \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    ATSS                        & real               & 65.2$\pm$0.45                             & 83.2$\pm$0.52                & 78.0$\pm$0.09         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    PAA                         & real               & 63.4$\pm$0.38                             & 81.6$\pm$0.42                & 73.8$\pm$0.27         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19     \\
    \textbf{Ours}               & real               & \textbf{68.9$\pm$0.16}                     & \textbf{88.7$\pm$0.16}    &  \textbf{78.7$\pm$0.25}        \\%& 63.9$\pm$0.15          &  70.0$\pm$0.15     \\ \hline
   
    \midrule
    Faster R-CNN                & real+sync          & 77.4$\pm$0.16                             &  93.2$\pm$0.17               & 88.7$\pm$0.21                           \\
    FCOS                        & real+sync          & 73.9$\pm$0.07                             &  89.2$\pm$0.30               &83.4$\pm$0.26\\%& 72.9$\pm$0.21          &  77.0$\pm$0.78        \\ 
    ATSS                        & real+sync          & 78.6$\pm$0.25                             &  93.8$\pm$0.15               &90.4$\pm$0.54\\%& 77.7$\pm$0.05          &  76.7$\pm$0.19        \\ 
    PAA                         & real+sync          & 77.3$\pm$0.16                             &  94.0$\pm$0.33               &88.8$\pm$0.55\\%&\textbf{78.1$\pm$0.91}  &  78.2$\pm$0.19        \\
    \textbf{Ours}                & real+sync          & \textbf{79.1$\pm$0.18}                    & \textbf{94.8$\pm$0.16}       &\textbf{90.5$\pm$0.21}\\%& 75.8$\pm$0.67          & 78.6$\pm$0.05         \\ \hline
    \bottomrule
\end{tabular}

==> figures/distancemap_cases.tex <==
\setlength\tabcolsep{0.5pt}
% \begin{tabular}{cccc}
%     \includegraphics[width=0.25\linewidth, trim=70 125 240 25, clip]{figures/distancemap_cases/000022.png} & 
%     \includegraphics[width=0.25\linewidth, trim=200 300 260 0, clip]{figures/distancemap_cases/000047.png} & 
%     \includegraphics[width=0.25\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000065.png} & 
%     \includegraphics[width=0.25\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000075.png}\\
%     \includegraphics[width=0.25\linewidth, trim=70 125 240 25, clip]{figures/distancemap_cases/000054_000022_2_fuse.png} & 
%     \includegraphics[width=0.25\linewidth, trim=200 300 260 0, clip]{figures/distancemap_cases/000048_000047_2_fuse.png} &
%     \includegraphics[width=0.25\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000049_000065_3_fuse.png} &
%     \includegraphics[width=0.25\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000053_000075_1_fuse.png}\\
%     \multicolumn{2}{c}{\small (a) Simple cases} & \multicolumn{2}{c}{\small (b) Hard cases} & ~\\
% \end{tabular}

\begin{tabular}{cccc}
    \includegraphics[width=0.24\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000065.png} & 
    \includegraphics[width=0.24\linewidth, trim=230 50 160 180, clip]{figures/distancemap_cases/000049_000065_3_fuse.png} &
    \includegraphics[width=0.24\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000075.png} &
    \includegraphics[width=0.24\linewidth, trim=100 80 360 220, clip]{figures/distancemap_cases/000053_000075_1_fuse.png} &
\end{tabular}

==> figures/fusion.tex <==
\begin{figure}
    \centering
    \setlength\tabcolsep{2pt}
    \begin{tabular}{cccl}
      \includegraphics[width=0.3\linewidth, clip, trim=150 0 35 0]{figures/fusion/activate_cells.jpg} &
      \includegraphics[width=0.3\linewidth, clip, trim=150 0 35 0]{figures/fusion/cluster.jpg} &
      \includegraphics[width=0.3\linewidth]{figures/fusion/vote.png} &
      \hspace{-2mm}
      \includegraphics[width=0.05\linewidth]{figures/fusion/colormap.pdf}
    \end{tabular}
    \caption{{\bf Combining multiple candidates.} 
          {\bf (a)} During inference, multiple cells of the network will be activated thanks to the proposed mask-based sampling strategy during training. 
          Each network cell will generate one box prediction. Here we visualize the cells by different colors according to the confidence of their corresponding box predictions. Note that the cells with the most confident prediction do not come from the center region here, but from some cells with the most discriminative textures.
          {\bf (b)} With multiple detection candidates from each local cell, we cluster them according to some simple distance threshold to correspond them to different instances.
          {\bf (c)} After a simple fusion of multiple candidate results, we can obtain a single robust result.}
    \label{fig:fusion}
  \end{figure}

==> figures/more_visualization.tex <==
\begin{tabular}{cccc}
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000494.jpg} &  
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000521.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000560.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000002_000785.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000494.jpg} &  
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000521.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000560.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000002_000785.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000016_000381.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000018_000246.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000020_000094.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/detection_results/000020_000174.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000016_000381.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000018_000246.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000020_000094.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 50}, clip]{figures/qualitative results/refine_results/000020_000174.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000001_000036.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000001_000015.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000003_000014.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/detection_results/000003_000057.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000001_000036.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000001_000015.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000003_000014.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 50 0 0}, clip]{figures/qualitative results/refine_results/000003_000057.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000053_000103.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000054_000032.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000055_000618.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/detection_results/000056_00075.jpg} \\
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000053_000103.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000054_000032.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000055_000618.jpg} &
    \includegraphics[width=0.22\linewidth, trim={0 0 0 20}, clip]{figures/qualitative results/refine_results/000056_000075.jpg} \\ 
\end{tabular}

==> tabs/ablate_detector.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Detector                                      & Pose Regressor                              & LM-O          & T-LESS        & TUD-L         & IC-BIN        & ITODD         & HB            & YCB-V         & Avg. \\
    \midrule
    {\bf RADet} & \multirow{3}{*}{WDR~\cite{wdr}}                                 & \textbf{0.614}& \textbf{0.588}& \textbf{0.623}& \textbf{0.514}& \textbf{0.247}& \textbf{0.618}& \textbf{0.605}& \textbf{0.544} \\
    Mask R-CNN~\cite{maskrcnn}  &          & 0.588         & 0.575         & 0.620         & 0.491         & 0.217         & 0.600         & 0.587         & 0.525  \\
    FCOS~\cite{fcosv1}           &         & 0.597         & 0.561         & 0.602         & 0.434         & 0.223         & 0.589         & 0.585         & 0.513 \\
    % -               & Ours                               & 0.614     & 0.678     & 0.796     & 0.514     & 0.247     & 0.618     & 0.709     &      \\
    % -               & Mask R-CNN~\cite{maskrcnn}            & 0.588     & 0.659     & 0.790     & 0.491     & 0.217     & 0.600     & 0.704     &       \\
    % -               & FCOS~\cite{fcosv1}                  & 0.597     & 0.689     & 0.799     & 0.434     & 0.223     & 0.589     & 0.707     &       \\               
    % \midrule
    % \multirow{3}{*}{CosyPose\dag~\cite{cosypose}}& {\bf RADet}                                 & \textbf{0.541}& \textbf{0.542}& \textbf{0.591}& \textbf{0.521}& \textbf{0.139}& \textbf{0.334}& \textbf{0.340}    & \textbf{0.429}   \\
    % ~                                           & Mask R-CNN~\cite{maskrcnn}            & 0.533         & 0.520         & 0.582         & 0.515         & 0.129         & 0.334         & 0.333             & 0.421 \\
    % ~                                           & FCOS~\cite{fcosv1}                    & 0.537         & 0.514         & 0.572         & 0.501         & 0.132         & 0.331         & 0.329             & 0.416  \\
    \midrule
    {\bf RADet} & \multirow{3}{*}{CDPNv2~\cite{cdpn}}                                 & \textbf{0.628}& \textbf{0.414}& \textbf{0.585}& \textbf{0.519}& \textbf{0.102}    & \textbf{0.731}& \textbf{0.397}    & {\bf 0.482}  \\
    Mask R-CNN~\cite{maskrcnn} &           & 0.612         & 0.415         & 0.552         & 0.517         & 0.094             & 0.728         & 0.386             & 0.472  \\
    FCOS~\cite{fcosv1}          &          & 0.624         & 0.407         & 0.575         & 0.473         & \textbf{0.102}    & 0.721         & 0.390             & 0.472  \\
    \bottomrule
\end{tabular}

==> tabs/ablation/activation.tex <==

\begin{tabular}{llccc}
    \toprule
    methods             & fusion        & AP                        &  AP$_{50}$                    & AP$_{75}$ \\
    \midrule
    random$^\dagger$    & \xmark        & 66.8$\pm$0.22             & 86.9 $\pm$0.22                & 75.1$\pm$0.11           \\
    random$^\dagger$    & \cmark        & 66.9$\pm$0.19             & 86.8 $\pm$0.15                & 74.8$\pm$0.14           \\
    all                 & \xmark        & 67.4$\pm$0.29             & 88.5 $\pm$0.21                & 76.1$\pm$0.63           \\
    all                 & \cmark        & 68.1$\pm$0.29             & 88.4 $\pm$0.23                & 76.7$\pm$0.25            \\
    topk                & \xmark        & 67.6$\pm$0.10             & 88.4 $\pm$0.19                & 75.2$\pm$0.16             \\
    topk                & \cmark        & 68.4$\pm$0.13             & 88.4 $\pm$0.18                & 76.6$\pm$0.26  \\
    random              & \xmark        & 69.0$\pm$0.15             & \textbf{88.7 $\pm$0.17}       & 77.5$\pm$0.13           \\
    random              & \cmark        & \textbf{69.6$\pm$0.12}    & 88.5 $\pm$0.19                & \textbf{78.7$\pm$0.25}           \\

    \bottomrule
\end{tabular}


==> tabs/ablation/distance_transform_compare.tex <==




% \begin{tabular}{cc|ccc|ccc}
% \hline
%                                                                                         & vote              & AP                    & AP$_{50}$             & AP$_{75}$             & AP$_{s}$              & AP$_{m}$              & AP$_{l}$          \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}geodesic\\ distance\end{tabular}}            &                   & 68.4                  &    86.3               &      77.0             &    -                   &     63.6              &    68.7           \\ 
%                                                                                         &\cmark         & 68.8                  &    86.1               &      78.4             &    -                 &     63.8              &     69.4           \\ \hline
% \multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}minimum\\ barrier\\ distance\end{tabular}}   & \multirow{2}{*}{} &\multirow{2}{*}{69.0}  & \multirow{2}{*}{88.7} & \multirow{2}{*}{77.5} & \multirow{2}{*}{-}     & \multirow{2}{*}{63.7} &\multirow{2}{*}{69.4}\\  
%                                                                                         &                   &                       &                       &                       &                       &                       &                   \\
%                                                                                         & \cmark        &    69.6               &      88.5             &      78.7             &     -                 &        63.9           &     70.0          \\ \hline
% \end{tabular}




\resizebox{\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
    data                                                                           & method                                                                      &fusion                        & AP                                & AP$_{50}$             & AP$_{75}$         \\%&AP$_{s}$           & AP$_{m}$              & AP$_{l}$      \\ \hline
    \midrule
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}real\end{tabular}}                  & \multirow{2}{*}{Geodesic}                                                   &\xmark                        &68.4$\pm$0.20                      &86.3$\pm$0.24          &77.0$\pm$0.36      \\%&-                  &63.6$\pm$0.25          & 68.7$\pm$0.19                         \\ 
                                                                                   &                                                                             &\cmark                        &68.8$\pm$0.17                      &86.1$\pm$\textbf{0.12}          &78.4$\pm$\underline{0.25}      \\%&-                  &63.5$\pm$0.24          & 69.4$\pm$0.14                        \\ \cline{2-9} 
    \cline{2-6} 
                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MinBarrier\end{tabular}}         &\xmark                        &69.0$\pm$0.15                      &\textbf{88.7}$\pm$0.17          &77.5$\pm$0.31      \\%&-                  &63.7$\pm$0.24          &69.4$\pm$0.16                                           \\ 
                                                                                   &                                                                             &\cmark                        &\textbf{69.6}$\pm$\textbf{0.12}    &88.5$\pm$0.19          &\textbf{78.7}$\pm$\textbf{0.25}      \\%&-                  &63.9$\pm$0.15          &70.0$\pm$0.15                                           \\ \hline
    % \midrule                                                                        
    % \multirow{4}{*}{Cityscapes}                                                    & \multirow{2}{*}{Geodesic}                                                   &                           &39.3          &64.2                   &38.9               \\%&17.8               &40.3                   &58.2                         \\ 
    %                                                                                &                                                                             &\cmark                 &39.7          &64.1                   &39.4               \\%&17.7               &40.5                   &58.6                        \\ \cline{2-9} 
    %                                                                                & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Minimum\\ barrier\end{tabular}}  &                           &39.8          &64.7                   &39.7               \\%&18.2               &42.9                   &57.4                         \\ 
    %                                                                                &                                                                             &\cmark                 &40.2          &64.6                   &40.1               \\%&18.4               &43.2                   &57.7                         \\ \hline
    \midrule                                                                               
    \multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}real+sync\end{tabular}}             & \multirow{2}{*}{Geodesic}                                                  &\xmark                         &77.0$\pm$0.13 &92.1$\pm$0.16          &88.9$\pm$0.28      \\%&-                  &75.3$\pm$0.72          &77.6$\pm$0.17                         \\  
                                                                                   &                                                                            &\cmark                         &77.6$\pm$0.08 &92.0$\pm$0.13          &89.8$\pm$0.11      \\%&-                  &75.4$\pm$0.65          &78.3$\pm$0.09                         \\ \cline{2-9} 
    \cline{2-6}                                                                        
                                                                                   & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}MinBarrier\end{tabular}}        &\xmark                         &77.8$\pm$0.05 &93.3$\pm$0.07          &89.7$\pm$0.17      \\%&-                  &75.7$\pm$0.64          &78.1$\pm$0.08            \\  
                                                                                   &                                                                            &\cmark                         &\textbf{78.2}$\pm$\textbf{0.07}       &\textbf{93.2}$\pm$\textbf{0.04}          &\textbf{90.1}$\pm$\textbf{0.12}      \\%&-                  &75.8$\pm$0.67          &78.6$\pm$0.05            \\ \hline
    \bottomrule
\end{tabular}
}
   




==> tabs/ablation/hyper_parameters.tex <==

\begin{center}
    \resizebox{0.9\linewidth}{!}{
        \begin{tabular}{l|lccc}
            \toprule
            \multicolumn{2}{c}{setting}         & AP                & AP$_{50}$         & AP$_{75}$ \\
            \midrule
            $\mathcal{T} = 0.1$     & $k = 10$  & 84.2               &                   &        \\
            $\mathcal{T} = 0.2$     & $k = 10$  & 84.8              &99.4               &97.1 \\
            $\mathcal{T} = 0.25$    & $k = 10$  &\textbf{85.0}      &\textbf{99.4}      &\textbf{97.4} \\
            $\mathcal{T} = 0.3$     & $k = 10$  &84.8               &99.2               &97.3 \\
            $\mathcal{T} = 0.4$     & $k = 10$  &               &                   & \\
            $\mathcal{T} = 0.5$     & $k = 10$  &                   &                   & \\
            \midrule
            $\mathcal{T} = 0.25$    & $k = 6$   &66.4               &87.9               &74.1 \\
            $\mathcal{T} = 0.25$    & $k = 8$   &66.4               &87.9               &74.1 \\
            $\mathcal{T} = 0.25$    & $k = 10$  &\textbf{69.6}      &\textbf{88.5}      &\textbf{78.7} \\
            $\mathcal{T} = 0.25$    & $k = 12$  &68.4               &87.2               &78.3\\
            $\mathcal{T} = 0.25$    & $k = 14$  &68.4               &87.2               &78.3\\
            $\mathcal{T} = 0.25$    & $k = 16$  &68.4               &87.2               &78.3\\
            \bottomrule
        \end{tabular}
    }
\end{center}


% \begin{tabular}{cccc|cccc|cccc}
%         \toprule
%         $k$                         & AP        & AP$_{50}$     & AP$_{75}$    & $\tau$     & AP        & AP$_{50}$     & AP$_{75}$  & $\alpha$ & AP        & AP$_{50}$     & AP$_{75}$ \\
%         \midrule
%         4                           & 83.4      & 98.4           & 93.5         & 0.1       & 84.1      & 98.5          & 96.0           & 0     & 83.9     & 98.8          & 94.3 \\
%         10                          & 85.0      & 99.4          & 97.4          & 0.2       & 84.7      & 99.3          & 96.8          & 0.1   & 85.0      & 99.4          & 97.4\\
%         32                          & 84.7      & 99.2          & 96.9          & 0.25      & 85.0      & 99.4          & 97.4          & 0.2   & 84.2      & 99.2          & 95.9\\
%         64                          & 84.2      & 98.9          & 96.3          & 0.3       & 84.9      & 99.4          & 97.0          & 0.3   & 83.1      & 98.4          & 93.2\\
%         128                         & 83.5      & 98.5          & 93.7          & 0.4       & 84.0      & 98.6          & 96.6          & 0.4   & 81.2      &               &   \\
%         256                         & 82.2      & 97.6          & 91.2          & 0.5       & 83.3      & 98.1          & 93.8          & 0.5   & 80.4      &               &   \\
%         \bottomrule
%     \end{tabular}
% }

==> tabs/ablation/training_schedule.tex <==
\begin{center}
    \begin{tabular}{ccccc}
        \toprule
        schedule                    & method       & AP                     & AP$_{50}$                 & AP$_{75}$               \\
        \midrule
        \multirow{2}*{$0.5$x}       & ATSS         & 66.3$\pm$0.08          & 84.7$\pm$0.17             &76.5$\pm$0.10          \\
        ~                           & {\bf Ours}          & \textbf{66.9$\pm$0.07} & \textbf{86.9$\pm$0.07}    &\textbf{74.7$\pm$0.08}           \\
        \midrule
        \multirow{2}*{$1$x}         & ATSS         & 68.8$\pm$0.04          & 86.8$\pm$0.08             &78.0$\pm$0.09          \\
        ~                           & {\bf Ours}          & \textbf{69.6$\pm$0.12} & \textbf{88.5$\pm$0.19}    &\textbf{78.7$\pm$0.25}           \\
        \midrule
        \multirow{2}*{$2$x}         & ATSS         & 64.4$\pm$0.68          & 81.3$\pm$0.85             &71.9$\pm$0.83               \\
        ~                           & {\bf Ours}          & \textbf{66.3$\pm$0.18} & \textbf{85.0$\pm$0.16}    &\textbf{73.1$\pm$0.19}            \\
        \bottomrule
        
    \end{tabular}
\end{center}

==> tabs/ablation_activation.tex <==
\begin{tabular}{cccc}
    \toprule
    Method          & AP        & AP$_{50}$     & AP$_{75}$ \\
    \midrule
    all & 82.3      & 97.7         & 94.5       \\
    random$\dagger$ & 83.5      & 98.2          & 95.7       \\
    topk            & 84.0      & 99.0          & 96.1      \\
    {\bf random}    & {\bf 85.0}& {\bf 99.4}    & {\bf 97.4}      \\
    \bottomrule
\end{tabular}

==> tabs/cityscapes_compare.tex <==

\begin{tabular}{lccccccc}
    \toprule
    method                      & backbone             & AP           & AP$_{50}$      & AP$_{75}$      & AP$_{s}$      & AP$_{m}$       & AP$_{l}$        \\
    \midrule
    Faster R-CNN    & ResNet-50           &38.3          & 63.3           & 40.1          &  16.5         &  38.9           & \textbf{60.4}                 \\
    FCOS           & ResNet-50            &38.0          & 63.1           & 38.6           & 17.2          &  38.7          & 55.5            \\ 
    ATSS             & ResNet-50            &39.5          & 63.9           & 40.3           & 16.9          &  40.3          & 57.6            \\ 
    PAA               & ResNet-50            &40.0          & \textbf{65.4}  & \textbf{40.8}  & 15.9          &  40.8          & 59.3            \\ 
    AutoAssign & ResNet-50            &29.5          & 50.7           & 29.3           & 10.9          &  30.3          & 47.2            \\
    \textbf{Ours}               & ResNet-50             &\textbf{40.2} & 64.6           & 40.1           & \textbf{18.4} & \textbf{43.2}  &  57.7     \\
    % \textbf{Mask (oracle)}               & ResNet-50            &\textbf{41.0} &  64.5          &  \textbf{42.5} & \underline{17.8}           & \underline{41.6}          & \textbf{60.6}    \\ 
    \midrule
    Faster R-CNN    & ResNet-101           &37.4          & 62.1          & 39.6           & 13.9          & 37.6            & 59.3                \\
    FCOS           & ResNet-101           &37.5          & 61.8           & 38.1           & 14.7          &  37.3          & 56.6            \\     
    ATSS             & ResNet-101           &38.4          & 62.9           & 38.3           & 15.4          &  39.4          & 57.7            \\ 
    PAA               & ResNet-101           &39.6          & \textbf{64.8}  & 39.5           & 15.5          &  \textbf{42.0} & \textbf{59.5}            \\ 
    AutoAssign & ResNet-101           &31.3          & 54.3           & 30.2           & 9.6           &  31.3          & 50.2            \\   
    \textbf{Ours}                & ResNet-101           &\textbf{39.8} & 63.1           & \textbf{41.4}  & \textbf{16.3} &  41.0          & \textbf{59.5}            \\
    % \textbf{Mask (oracle)}      & ResNet-101           &\textbf{40.6} & \textbf{64.9}           & \underline{41.3}           & \textbf{16.7} & \underline{41.5}  & \textbf{60.9}   \\ 
    \bottomrule
\end{tabular}


==> tabs/coco_campare_category.tex <==

% \begin{table}
% 	\centering
% 	\tiny
% 	\begin{tabular}{cccc|cccc}
% 		\toprule
% 		                &  PAA       & \textbf{Ours}   	&\textcolor{green}{$\Delta$}    		&				& PAA 	& \textbf{Ours} &\textcolor{green}{$\Delta$}\\
% 		\midrule	
% 		parking meter   &  45.4      & 40.6           	&  \textcolor{green}{-4.8}           	&toaster 		& 22.4   & 31.8        	&\textcolor{green}{+9.4}\\
% 		scissors        &  29.6      & 24.8           	&  \textcolor{green}{-4.8}           	&bottle   		& 36.1   & 38.4        	&\textcolor{green}{+2.3}\\
% 		horse           &  58.1      & 54.7           	&  \textcolor{green}{-3.4}           	&handbag  		& 13.2   & 10.0        	&\textcolor{green}{+3.2}\\
% 		dog             &  62.6      & 59.9           	& \textcolor{green}{-2.7}            	&wine glasses  	& 33.8   & 35.8        	&\textcolor{green}{+2.0}\\
% 		carrot          &  22.5      & 19.8       	  	&\textcolor{green}{-2.7}			   	&skateboard    	& 50.9   & 52.6		   	&\textcolor{green}{+2.7}\\
% 		donut           &  47.3      & 44.8       		&\textcolor{green}{-2.5}				&banana        	& 23.2   & 24.6        	&\textcolor{green}{+1.4}\\
% 		cow             &  57.9      & 55.5             &\textcolor{green}{-2.4}				&car           	& 42.6   & 44.0			&\textcolor{green}{+1.4}\\
% 		keyboard        &  55.1      & 53.0       		&\textcolor{green}{-2.1}				&boat         	& 25.0   & 26.2			&\textcolor{green}{+1.2}\\
% 		umbrella        &  38.1      & 36.1       		&\textcolor{green}{-2.0}				&cell phone     & 34.4   & 33.3			&\textcolor{green}{+1.1}\\
% 		sandwich        &  23.3      & 21.6       		&\textcolor{green}{-1.7}  				&cup           	& 40.8   & 41.9			&\textcolor{green}{+1.1}\\
% 		knife           &  13.8      & 12.1       		&\textcolor{green}{-1.7}				&pizza          & 50.4   & 51.4 		&\textcolor{green}{+1.0}\\
% 		bench           &  23.3      & 21.6       		&\textcolor{green}{-1.7}				&bicycle       	& 29.0   & 29.9			&\textcolor{green}{+0.9}\\
% 		dining table    &  28.7      & 27.2       		&\textcolor{green}{-1.5}				&vase          	& 35.7   & 36.6			&\textcolor{green}{+0.9}\\
% 		hot dog         &  32.5      & 31.3       		&\textcolor{green}{-1.2}				&suitcase      	& 35.6   & 36.5			&\textcolor{green}{+0.9}\\
% 		laptop          &  58.0      & 56.8       		&\textcolor{green}{-1.2}				&fork          	& 26.7   & 27.5			&\textcolor{green}{+0.8}\\
% 		sink            &  36.1      & 35.0      		&\textcolor{green}{-1.1} 				&tie           	& 30.7   & 31.5			&\textcolor{green}{+0.8}\\
% 		% cat             &  68.2      & 67.4       		&\textcolor{green}{}&cell phone    & 33.3   & 34.4\\
% 		% airplane        &  66.6      & 65.6
% 		% bear            &  70.2      & 69.3
% 		% zebra           &  68.7      & 67.9

% 		\bottomrule
		

% 		% \toprule
% 		% PAA better 													& Ours better\\
% 		% \midrule
% 		% parking meter(40.6/45.4)                                 &  toaster(31.8/22.4) \\
% 		% scissors(24.8/29.6)										 &  bottle(38.4/36.1)  \\
% 		% horse(54.7/58.1)                                         &  handbag(13.2/10.0) \\
% 		% dog(59.9/62.6), carrot(19.8/22.5)                        &  wine glass(35.8/33.8)  \\
% 		% donut(44.8/47.3)                                         &  skateboard(52.6/50.9\\
% 		% cow(55.5/57.9)                                           &  banana(24.6/23.2), car(44.0/42.6)\\
% 		% keyboard(53.0/55.1)                                      &  truck(37.2/36.4), boat(26.2/25.0)\\
% 		% umbrella(36.1/38.1)                                      &  cell phone(34.4/33.3), cup(41.9/40.8)\\
% 		% cat(67.4/68.2), sandwich(34.4/36.2)                      &  pizza(51.4/50.4)\\
% 		% knife(12.1/13.8), bench(21.6/23.3)                       &  bicycle(29.9/29.0), vase(36.6/35.7), suitcase(36.5/35.6)\\
% 		% dining table(27.2/28.7)                                  &  fork(27.5/26.7), tie(31.5/30.7)\\
% 		% hot dog(31.3/32.5), laptop(56.8/58.0)                    &  \\
% 		% sink(35.0/36.1)                                          &    \\
% 		% airplane(65.6/66.6)                                      &   \\
% 		% bear(69.3/70.2),                                         &   \\
% 		% zebra(67.9/68.7)                                         &    \\
% 		% \bottomrule

% 	\end{tabular}
% \end{table}



% \begin{table}
%     \centering
%     \tiny
%     \begin{tabular}{cccc|cccc}
%         \toprule
%                 &  PAA       & \textbf{Ours}   	&$\Delta$    		&				& PAA 	& \textbf{Ours} &$\Delta$\\
%         \midrule
%         bottle   		& 36.1  & 38.4     &\textcolor{green}{+2.3}  &car           & 42.6   & 44.0     &\textcolor{green}{+1.4}\\
%         wine glasses  	& 33.8  & 35.8     &\textcolor{green}{+2.0}  &boat         & 25.0   & 26.2	    &\textcolor{green}{+1.2}\\
%         cup           	& 40.8  & 41.9     &\textcolor{green}{+1.1}  &bicycle       & 29.0   & 29.9		&\textcolor{green}{+0.9}\\
%         vase          	& 35.7  & 36.6	   &\textcolor{green}{+0.9}  &truck         & 36.4   & 37.2     &\textcolor{green}{+0.8}\\\cline{1-4}
%         horse           & 58.1  & 54.7     & \textcolor{red}{-3.4}  &airplane      & 66.6   & 65.6     &\textcolor{red}{-1.0}\\\cline{5-8}
%         dog             & 62.6  & 59.9     & \textcolor{red}{-2.7}  &carrot        & 22.5   & 19.8     &\textcolor{red}{-2.7}\\
%         cow             & 57.9  & 55.5     & \textcolor{red}{-2.4}  &donut         & 47.3   & 44.8     &\textcolor{red}{-2.5}\\
%         bear            & 70.2  & 69.3     & \textcolor{red}{-0.9} &sandwich      & 23.3   & 21.6     &\textcolor{red}{-1.7}\\
%         cat             & 68.2  & 67.4     & \textcolor{red}{-0.8} &hot dog       & 32.5   & 31.3     &\textcolor{red}{-1.2}\\
%         zebra           & 68.7  & 67.9     & \textcolor{red}{-0.8} &banana        & 23.2   & 24.6     &\textcolor{green}{+1.4}\\\cline{1-4}
%         scissors        & 29.6  & 24.8     &\textcolor{red}{-4.8} &pizza         & 50.4   & 51.4 	    &\textcolor{green}{+1.0}\\\cline{5-8}
%         knife           & 13.8  & 12.1     &\textcolor{red}{-1.7}   &bench         & 23.3   & 21.6      &\textcolor{red}{-1.7}\\
%         fork          	& 26.7  & 27.5	   &\textcolor{green}{+0.8}   &dining table  & 28.7   & 27.2      &\textcolor{red}{-1.5}\\\cline{1-4}
%         toaster 		& 22.4  & 31.8     &\textcolor{green}{+9.4}   &sink          & 36.1   & 35.0      &\textcolor{red}{-1.1}\\\cline{5-8}
%         skateboard    	& 50.9  & 52.6	   &\textcolor{green}{+2.7} &handbag  		& 13.2   & 10.0    &\textcolor{green}{+3.2}\\
%         suitcase      	& 35.6   & 36.5    &\textcolor{green}{+0.9} &tie           	& 30.7   & 31.5			&\textcolor{green}{+0.8}\\
%         keyboard        & 55.1  & 53.0     &\textcolor{red}{-2.1} &umbrella        &  38.1      & 36.1     &\textcolor{red}{-2.0}\\
%         &&&                                                       &laptop        &  58.0  & 56.8     &\textcolor{red}{-1.2}\\

%         \bottomrule
        

        
%     \end{tabular}

% \end{table}


\begin{table}[h]
    \centering
    
    \resizebox{\linewidth}{!}{
    \small
    \begin{tabular}{cccc|cccc}
        \toprule
                &  PAA       & \textbf{Ours}   	&$\Delta$    		&				& PAA 	& \textbf{Ours} &$\Delta$\\
        \midrule
        toaster 		& 22.4  & 31.8      &\textcolor{green}{+9.4}    & horse             & 58.1  & 54.7     & \textcolor{red}{-3.4}\\
        skateboard    	& 50.9  & 52.6	    &\textcolor{green}{+2.7}    & dog               & 62.6  & 59.9     & \textcolor{red}{-2.7}\\
        suitcase      	& 35.6  & 36.5      &\textcolor{green}{+0.9}    & cow               & 57.9  & 55.5     & \textcolor{red}{-2.4}\\
        keyboard        & 55.1  & 53.0      &\textcolor{red}{-2.1}      & bear              & 70.2  & 69.3     & \textcolor{red}{-0.9}\\\cline{1-4}
        bottle   		& 36.1  & 38.4      &\textcolor{green}{+2.3}    & cat               & 68.2  & 67.4     & \textcolor{red}{-0.8}\\
        wine glasses  	& 33.8  & 35.8      &\textcolor{green}{+2.0}    & zebra             & 68.7  & 67.9     & \textcolor{red}{-0.8}\\\cline{5-8}
        cup           	& 40.8  & 41.9      &\textcolor{green}{+1.1}    & scissors          & 29.6  & 24.8     &\textcolor{red}{-4.8}\\
        vase          	& 35.7  & 36.6	    &\textcolor{green}{+0.9}    & knife             & 13.8  & 12.1     &\textcolor{red}{-1.7}\\\cline{1-4}
        car             & 42.6  & 44.0      &\textcolor{green}{+1.4}    & fork          	& 26.7  & 27.5	   &\textcolor{green}{+0.8}\\\cline{5-8}
        boat            & 25.0  & 26.2	    &\textcolor{green}{+1.2}    & carrot            & 22.5   & 19.8     &\textcolor{red}{-2.7}\\
        bicycle         & 29.0  & 29.9		&\textcolor{green}{+0.9}    & donut             & 47.3   & 44.8     &\textcolor{red}{-2.5}\\
        truck           & 36.4  & 37.2      &\textcolor{green}{+0.8}    & sandwich          & 23.3   & 21.6     &\textcolor{red}{-1.7}\\
        airplane        & 66.6  & 65.6      &\textcolor{red}{-1.0}      & hot dog           & 32.5   & 31.3     &\textcolor{red}{-1.2}\\\cline{1-4}
        handbag  		& 13.2  & 10.0      &\textcolor{green}{+3.2}    & banana            & 23.2   & 24.6     &\textcolor{green}{+1.4}\\
        tie           	& 30.7  & 31.5	    &\textcolor{green}{+0.8}    & pizza             & 50.4   & 51.4 	&\textcolor{green}{+1.0}\\\cline{5-8}
        umbrella        & 38.1  & 36.1      &\textcolor{red}{-2.0}      & bench             & 23.3   & 21.6      &\textcolor{red}{-1.7}\\
        laptop          & 58.0  & 56.8      &\textcolor{red}{-1.2}      & dining table      & 28.7   & 27.2      &\textcolor{red}{-1.5}\\
                        &       &           &                           & sink              & 36.1   & 35.0      &\textcolor{red}{-1.1}\\

        \bottomrule
        

        
    \end{tabular}
    }

\end{table}

==> tabs/coco_compare.tex <==
\begin{tabular}{cc|ccc|ccc}
    \hline
    method                      & backbone              & AP        & AP$_{50}$ & AP$_{75}$     &AP$_{s}$   &AP$_{m}$   & AP$_{l}$  \\ \hline
    FCOS\cite{fcosv2}           & ResNet-50             & 38.9      &  57.5     & 42.2          &  23.1     & 42.7      &  50.2      \\ 
    ATSS\cite{ATSS}             & ResNet-50             & 39.2      &  57.3     & 42.4          &  22.7     & 43.1      &  51.5    \\ 
    PAA\cite{PAA}               & ResNet-50             & 40.4      &  58.4     & 43.9          &  22.9     & 44.3      &  54.0    \\
    AutoAssign\cite{autoassign} & ResNet-50             & 40.4      &  59.6     & 43.7          &  22.7     & 44.1      &  52.9     \\
    \textbf{Distance}           & ResNet-50             & 40.0      &  57.1     & 43.4          &  23.5     & 43.5      &  51.9     \\\hline
    FCOS\cite{fcosv2}           & ResNet-101            & 43.2      & 62.4      & 46.8          &  26.1     & 46.2      &   52.8    \\ 
    ATSS\cite{ATSS}             & ResNet-101            & 43.6      & 62.1      & 47.4          &  26.1     & 47.0      &   53.6    \\ 
    PAA\cite{PAA}               & ResNet-101            & 44.6      & 63.3      & 48.4          &  26.4     & 48.5      &   56.0    \\
    AutoAssign\cite{autoassign} & ResNet-101            & 44.5      & 64.3      & 48.4          &  25.9     & 47.4      &   55.0    \\
    \textbf{Distance}           & ResNet-101            & 44.1      & 62.2      & 48.1          &  26.7     & 47.2      &   54.8    \\\hline
\end{tabular}


==> tabs/compare_all_pose_rgb.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Method                      & Real            & LM-O              & T-LESS             & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V             & Avg.          \\
    \midrule
    \textbf{RADet+PFA}          & \checkmark           &\textbf{0.715}     & \textbf{0.778}    & \textbf{0.839}    & \textbf{0.600}    & 0.353             & \textbf{0.840}    & 0.806             & \textbf{0.704} \\
    % \textbf{RADet+WDR}          & \checkmark           & 0.614             & 0.678             & 0.796             & 0.514             & 0.247             & 0.618             & 0.722             & 0.598 \\
    SurfEmb~\cite{surfemb}      & \checkmark           & 0.663             & 0.770             & 0.805             & 0.588             & \textbf{0.413}    & 0.791             & 0.711             & 0.677             \\
    CosyPose~\cite{cosypose}    & \checkmark           & 0.633             & 0.728             & 0.823             & 0.583             & 0.216             & 0.656             & \textbf{0.821}             & 0.637 \\
    CDPNv2~\cite{cdpn}          & \checkmark           & 0.624             & 0.478             & 0.772             & 0.473             & 0.102             & 0.722             & 0.532             & 0.529 \\
    Pix2Pose~\cite{pix2pose}    & \checkmark           & 0.363             & 0.344             & 0.420             & 0.226             & 0.134             & 0.346             & 0.446             & 0.342 \\
    % PFA~\cite{pfa}              & \checkmark           & 0.701             & -                 & -                 & -                 & -                 & -                 & 0.738             & -     \\
    % DPODv2~\cite{dpodv2}        & \checkmark    & RGB       & 0.584             & 0.655             & -                 & -                 & -                 & 0.725             & -                 & -    \\
    % CIR~\cite{coupled_iterative}& \checkmark    & RGB       & 0.655             & 0.715             & -                 &   -               & -                 & -                 & \textbf{0.824}    &   - \\
    \midrule
    \textbf{RADet+PFA}          &                      & \textbf{0.715}    & 0.719             & \textbf{0.733}    & \textbf{0.600}    & 0.353             & \textbf{0.840}    & \textbf{0.648}    & \textbf{0.658} \\
    % \textbf{RADet+WDR}          &                      & 0.614             & 0.588             & 0.623             & 0.514             & 0.247             & 0.618             & 0.605             & 0.544 \\
    PFA~\cite{pfa}              &                      & 0.676             &  -                & -                 & -                 & -                 & -                 & 0.614             & -   \\
    SurfEmb~\cite{surfemb}      &                      & 0.663             & \textbf{0.735}    & 0.715             & 0.588             & \textbf{0.413}    & 0.791             & 0.647             & 0.650 \\
    CosyPose~\cite{cosypose}    &                      & 0.633             & 0.640             & 0.685             & 0.583             & 0.216             & 0.656             & 0.574             & 0.570 \\
    CDPNv2~\cite{cdpn}          &                      & 0.624             & 0.407             & 0.588             & 0.473             & 0.102             & 0.722             & 0.390             & 0.472 \\
    % PFA~\cite{pfa}              &                      & 0.701             &  -                & -                 & -                 & -                 & -                 & 0.615             & -   \\
    % DPODv2~\cite{dpodv2}        &               & RGB       & 0.584             & 0.636             & -                 & -                 & -                 & 0.725             & -                 & -    \\
    % \midrule
    % \textbf{RADet+PFA}          & \checkmark    & RGB-D     & \textbf{0.797}    & \textbf{0.850}    & 0.960             & \textbf{0.676}    & 0.469             & \textbf{0.869}    & 0.888             & \textbf{0.787} \\
    % SurfEmb~\cite{surfemb}      & \checkmark    & RGB-D     & 0.760             & 0.833             & 0.933             & 0.659             & \textbf{0.538}    & 0.866             & 0.824             & 0.773 \\
    % CIR~\cite{coupled_iterative}& \checkmark    & RGB-D     & 0.734             & 0.776             & \textbf{0.968}    & \textbf{0.676}    & 0.381             & 0.757             & \textbf{0.893}    & 0.741 \\
    % CosyPose+ICP~\cite{cosypose}& \checkmark    & RGB-D     & 0.714             & 0.701             & 0.939             & 0.647             & 0.313             & 0.712             & 0.861             & 0.698 \\
    % Pix2Pose+ICP~\cite{pix2pose}& \checkmark    & RGB-D     & 0.588             & 0.512	            & 0.820	            & 0.390	            & 0.351	            & 0.695	            & 0.780	            & 0.591 \\
    % CDPNv2+ICP~\cite{cdpn}      & \checkmark    & RGB-D     & 0.630             & 0.464             & 0.913             & 0.450             & 0.186             & 0.712             & 0.619             & 0.568 \\
    % PFA~\cite{pfa}              &               & RGB-D     & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.822             & -\\
    % % DPODv2~\cite{dpodv2}        & \checkmark    & RGB-D     & 0.700             & 0.720             & -                     & -                 & -                 & 0.840             & -                 & -    \\
    % \midrule
    % \textbf{RADet+PFA}         &                & RGB-D     & \textbf{0.797}    & 0.801             & \textbf{0.894}    & \textbf{0.676}    & 0.469             & \textbf{0.869}    & \textbf{0.826}    & \textbf{0.762} \\
    % SurfEmb~\cite{surfemb}     &                & RGB-D     & 0.760             & \textbf{0.828}    & 0.854             & 0.659             & \textbf{0.538}    & 0.866             & 0.799             & 0.758 \\
    % CDPNv2+ICP~\cite{cdpn}     &                & RGB-D     & 0.630             & 0.435             & 0.791             & 0.450             & 0.186             & 0.712             & 0.532             & 0.534 \\
    % % DPODv2~\cite{dpodv2}       &                & RGB-D     & 0.700             & 0.699             & -                 & -                 & -                 & 0.840             & -                 & -    \\
    % PFA~\cite{pfa}             &                & RGB-D     & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.800             & -\\
    \bottomrule
\end{tabular}

==> tabs/compare_all_pose_rgbd.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Method                      & Real          & LM-O              & T-LESS             & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V             & Avg.          \\
    \midrule
    \textbf{RADet+PFA}          & \checkmark    & \textbf{0.797}    & \textbf{0.850}    & 0.960             & \textbf{0.676}    & 0.469             & \textbf{0.869}    & 0.888             & \textbf{0.787} \\
    SurfEmb~\cite{surfemb}      & \checkmark    & 0.760             & 0.833             & 0.933             & 0.659             & \textbf{0.538}    & 0.866             & 0.824             & 0.773 \\
    CIR~\cite{coupled_iterative}& \checkmark    & 0.734             & 0.776             & \textbf{0.968}    & \textbf{0.676}    & 0.381             & 0.757             & \textbf{0.893}    & 0.741 \\
    CosyPose+ICP~\cite{cosypose}& \checkmark    & 0.714             & 0.701             & 0.939             & 0.647             & 0.313             & 0.712             & 0.861             & 0.698 \\
    Pix2Pose+ICP~\cite{pix2pose}& \checkmark    & 0.588             & 0.512	            & 0.820	            & 0.390	            & 0.351	            & 0.695	            & 0.780	            & 0.591 \\
    CDPNv2+ICP~\cite{cdpn}      & \checkmark    & 0.630             & 0.464             & 0.913             & 0.450             & 0.186             & 0.712             & 0.619             & 0.568 \\
    % PFA~\cite{pfa}              &               & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.822             & -\\
    % DPODv2~\cite{dpodv2}        & \checkmark    & RGB-D     & 0.700             & 0.720             & -                     & -                 & -                 & 0.840             & -                 & -    \\
    \midrule
    \textbf{RADet+PFA}         &                & \textbf{0.797}    & 0.801             & \textbf{0.894}    & \textbf{0.676}    & 0.469             & \textbf{0.869}    & \textbf{0.826}    & \textbf{0.762} \\
    SurfEmb~\cite{surfemb}     &                & 0.760             & \textbf{0.828}    & 0.854             & 0.659             & \textbf{0.538}    & 0.866             & 0.799             & 0.758 \\
    CDPNv2+ICP~\cite{cdpn}     &                & 0.630             & 0.435             & 0.791             & 0.450             & 0.186             & 0.712             & 0.532             & 0.534 \\
    % DPODv2~\cite{dpodv2}       &                & RGB-D     & 0.700             & 0.699             & -                 & -                 & -                 & 0.840             & -                 & -    \\
    % PFA~\cite{pfa}             &                & 0.749             & -                 &  -                & -                 & -                 & -                 & 0.800             & -\\
    \bottomrule
\end{tabular}

==> tabs/compare_allpose_mspd.tex <==
% \begin{tabular}{lll|lllllll|l}
%   \toprule
%   Method                      & Real    & Data        & LM-O$^{\ast}$     & T-LESS            & TUD-L             & IC-BIN$^{\ast}$   & ITODD$^{\ast}$    & HB$^{\ast}$       & YCB-V             & Avg.\\
%   \toprule
%   {\bf PFA + Ours}            &         & RGB         & {\bf 0.876}       & 0.832             & {\bf 0.890}       & {\bf 0.689}       & 0.484             & 0.879             & 0.771             & 0.774\\
%   PFA~\cite{pfa}              &         & RGB         & 0.819             & -                 &   -               &   -               &   -               & -                 & 0.739             &    -       \\
%   SurfEmb~\cite{surfemb}      &         & RGB         & 0.851             & {\bf 0.857}       & 0.889             & 0.678             & {\bf 0.552}       & {\bf 0.888}       & {\bf 0.773}       & {\bf 0.784}     \\
%   Cosypose~\cite{cosypose}    &         & RGB         & 0.812             & 0.761             & 0.847             & 0.675             & 0.300             & 0.721             & 0.653             & 0.681     \\
%   CDPNv2~\cite{cdpn}          &         & RGB         & 0.815             & 0.579             & 0.797             & 0.582             & 0.161             & 0.845             & 0.511             & 0.613     \\
%   \midrule
%   {\bf PFA+Ours}              & \cmark  & RGB         & {\bf 0.876}       & {\bf 0.877}       & {\bf 0.978}       & {\bf 0.689}       & {\bf 0.484}       & {\bf 0.879}       & {\bf 0.856}        & {\bf 0.806}\\
%   PFA~\cite{pfa}              & \cmark  & RGB         & 0.819             & -                 & -                 & -                 & -                 & -                 & 0.810                 & - \\
%   CIR~\cite{coupled_iterative}& \cmark  & RGB         & 0.831             & 0.798             & -                 &  -                &  -                &   -               & 0.852             & -     \\
%   Cosypose~\cite{cosypose}    & \cmark  & RGB         & 0.812             & 0.821             & 0.973             & 0.675             & 0.300             & 0.721             & 0.850             & 0.736\\
%   CDPNv2~\cite{cdpn}          & \cmark  & RGB         & 0.815             & 0.620             & 0.925             & 0.582             & 0.161             & 0.845             & 0.631             & 0.654 \\
%   \midrule
%   {\bf PFA+Ours}              &         & RGB-D       & {\bf 0.890}       & 0.833             & {\bf 0.929}       & {\bf 0.702}       & 0.498             & 0.888             & {\bf 0.819}        & {\bf 0.794}\\
%   PFA~\cite{pfa}              &         & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.793                 & - \\
%   SurfEmb~\cite{surfemb}      &         & RGB-D       & 0.856             & {\bf 0.859}       & 0.905             & 0.680             & {\bf 0.560}       & {\bf 0.893}       & 0.792                 & 0.792     \\
%   CDPNv2+ICP~\cite{cdpn}      &         & RGB-D       & 0.731             & 0.488             & 0.829             & 0.459             & 0.184             & 0.749             & 0.483                 & 0.560 \\
%   \midrule
%   {\bf PFA+Ours}              & \cmark  & RGB-D       & {\bf 0.890}       & {\bf 0.878}       & {\bf 0.989}       & {\bf 0.702}       & {\bf 0.498}       & {\bf 0.888}       & 0.881        & {\bf 0.818}\\
%   PFA~\cite{pfa}              & \cmark  & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.816                 & - \\
%   CIR~\cite{coupled_iterative}&\cmark   & RGB-D       & 0.824             & 0.795             & 0.991             & 0.683             & 0.370             & 0.757             & {\bf 0.885}                 &   0.758\\
%   Cosypose+ICP~\cite{cosypose}&\cmark   & RGB-D       & 0.826             & 0.767             & 0.976             & 0.666             & 0.315             & 0.737             & 0.849                 & 0.734    \\
%   CDPNv2+ICP~\cite{cdpn}      &         & RGB-D       & 0.731             & 0.516             & 0.947             & 0.459             & 0.184             & 0.749             & 0.565                 & 0.593 \\
%   \bottomrule
% \end{tabular}

\begin{tabular}{lll|lllllll|l}
  \toprule
  Method                      & Real    & Data        & LM-O$^{\ast}$     & T-LESS            & TUD-L             & IC-BIN$^{\ast}$   & ITODD$^{\ast}$    & HB$^{\ast}$       & YCB-V             & Avg.\\
  \toprule
  {\bf PFA + Ours}            &         & RGB         & {\bf 0.876}       & 0.832             & {\bf 0.890}       & {\bf 0.689}       & 0.484             & 0.879             & 0.771             & 0.774\\
  PFA                         &         & RGB         & 0.819             & -                 &   -               &   -               &   -               & -                 & 0.739             &    -       \\
  SurfEmb                     &         & RGB         & 0.851             & {\bf 0.857}       & 0.889             & 0.678             & {\bf 0.552}       & {\bf 0.888}       & {\bf 0.773}       & {\bf 0.784}     \\
  Cosypose                    &         & RGB         & 0.812             & 0.761             & 0.847             & 0.675             & 0.300             & 0.721             & 0.653             & 0.681     \\
  CDPNv2                      &          & RGB         & 0.815             & 0.579             & 0.797             & 0.582             & 0.161             & 0.845             & 0.511             & 0.613     \\
  \midrule
  {\bf PFA+Ours}              & \cmark  & RGB         & {\bf 0.876}       & {\bf 0.877}       & {\bf 0.978}       & {\bf 0.689}       & {\bf 0.484}       & {\bf 0.879}       & {\bf 0.856}        & {\bf 0.806}\\
  PFA                         & \cmark  & RGB         & 0.819             & -                 & -                 & -                 & -                 & -                 & 0.810                 & - \\
  CIR                         & \cmark  & RGB         & 0.831             & 0.798             & -                 &  -                &  -                &   -               & 0.852             & -     \\
  Cosypose                    & \cmark  & RGB         & 0.812             & 0.821             & 0.973             & 0.675             & 0.300             & 0.721             & 0.850             & 0.736\\
  CDPNv2                      & \cmark  & RGB         & 0.815             & 0.620             & 0.925             & 0.582             & 0.161             & 0.845             & 0.631             & 0.654 \\
  \midrule
  {\bf PFA+Ours}              &         & RGB-D       & {\bf 0.890}       & 0.833             & {\bf 0.929}       & {\bf 0.702}       & 0.498             & 0.888             & {\bf 0.819}        & {\bf 0.794}\\
  PFA                         &         & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.793                 & - \\
  SurfEmb                     &         & RGB-D       & 0.856             & {\bf 0.859}       & 0.905             & 0.680             & {\bf 0.560}       & {\bf 0.893}       & 0.792                 & 0.792     \\
  CDPNv2+ICP                  &         & RGB-D       & 0.731             & 0.488             & 0.829             & 0.459             & 0.184             & 0.749             & 0.483                 & 0.560 \\
  \midrule
  {\bf PFA+Ours}              & \cmark  & RGB-D       & {\bf 0.890}       & {\bf 0.878}       & {\bf 0.989}       & {\bf 0.702}       & {\bf 0.498}       & {\bf 0.888}       & 0.881        & {\bf 0.818}\\
  PFA                         & \cmark  & RGB-D       & 0.835             & -                 & -                 & -                 & -                 & -                 & 0.816                 & - \\
  CIR                         &\cmark   & RGB-D       & 0.824             & 0.795             & 0.991             & 0.683             & 0.370             & 0.757             & {\bf 0.885}                 &   0.758\\
  Cosypose+ICP                &\cmark   & RGB-D       & 0.826             & 0.767             & 0.976             & 0.666             & 0.315             & 0.737             & 0.849                 & 0.734    \\
  CDPNv2+ICP                  & \cmark    & RGB-D       & 0.731             & 0.516             & 0.947             & 0.459             & 0.184             & 0.749             & 0.565                 & 0.593 \\
   \bottomrule
\end{tabular}

==> tabs/compare_allpose_mssd.tex <==
% \begin{tabular}{lll|lllllll|l}
%   \toprule
%   Method                      & Real              & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$    & ITODD$^{\ast}$     & HB$^{\ast}$               & YCB-V             & Avg.\\
%   \midrule
%   {\bf PFA + Ours}            &                   & RGB       & {\bf 0.712}       & 0.682             & {\bf 0.721}       & {\bf 0.589}         & 0.306             & {\bf 0.840}               & {\bf 0.623}       & {\bf 0.639}      \\
%   PFA~\cite{pfa}              &                   & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.585             &    -       \\
%   SurfEmb~\cite{surfemb}      &                   & RGB       & 0.640             & {\bf 0.686}       & 0.687             & 0.573               & {\bf 0.363}       & 0.760                     & 0.620             & 0.618      \\
%   Cosypose~\cite{cosypose}    &                   & RGB       & 0.606             & 0.589             & 0.664             & 0.559               & 0.177             & 0.634                     & 0.554             & 0.540     \\
%   CDPNv2~\cite{cdpn}          &                   & RGB       & 0.612             & 0.338             & 0.577             & 0.438               & 0.087             & 0.708                     & 0.399             & 0.451     \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark            & RGB       & {\bf 0.712}       & {\bf 0.749}       & {\bf 0.820}       & {\bf 0.589}         & {\bf 0.306}       & {\bf 0.840}               & 0.809             & {\bf 0.689}  \\
%   PFA~\cite{pfa}              & \cmark            & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.742             &    -       \\
%   CIR~\cite{coupled_iterative}& \cmark            & RGB       & 0.633             & 0.684             & -                 &  -                  & -                 & -                         & {\bf 0.835}       & -         \\
%   Cosypose~\cite{cosypose}    & \cmark            & RGB       & 0.606             & 0.695             & 0.807             & 0.559               & 0.177             & 0.634                     & 0.842             & 0.617    \\
%   CDPNv2~\cite{cdpn}          & \cmark            & RGB       & 0.612             & 0.426             & 0.793             & 0.438               & 0.087             &0.708                      & 0.570             & 0.519\\
%   \midrule
%   {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.807}       & {\bf 0.930}       & {\bf 0.692}         & 0.495             & {\bf 0.879}               & {\bf 0.867}       & {\bf 0.788}      \\
%   PFA~\cite{pfa}              & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.842            &    -       \\
%   SurfEmb~\cite{surfemb}      & \cmark            & RGB-D     & 0.809             & 0.829             & 0.891             & 0.677               & {\bf 0.558}       & 0.875                     & 0.849             & 0.784      \\
%   CDPNv2+ICP~\cite{cdpn}      & \cmark            & RGB-D     & 0.689             & 0.449             & 0.847             & 0.458               & 0.206             & 0.757                     & 0.603             & 0.573    \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.856}       & {\bf 0.986}       & {\bf 0.692}         & {\bf 0.495}       & {\bf 0.879}               & 0.920             & {\bf 0.810}      \\
%   PFA~\cite{pfa}              & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.852             &    -       \\
%   CIR~\cite{coupled_iterative}& \cmark            & RGB-D     & 0.778             & 0.773             & 0.991             & 0.688               & 0.379             & 0.753                     & {\bf 0.924}       & 0.755 \\ 
%   Cosypose+ICP~\cite{cosypose}&\cmark             & RGB-D     & 0.748             & 0.749             & 0.972             & 0.652               & 0.341             & 0.719                     & 0.903             & 0.726  \\
%   CDPNv2+ICP~\cite{cdpn}      & \cmark            & RGB-D     & 0.689             & 0.489             & 0.962             & 0.458               & 0.206             & 0.757                     & 0.701             & 0.609    \\
%   \bottomrule
% \end{tabular}


\begin{tabular}{lll|lllllll|l}
  \toprule
  Method                      & Real              & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$    & ITODD$^{\ast}$     & HB$^{\ast}$               & YCB-V             & Avg.\\
  \midrule
  {\bf PFA + Ours}            &                   & RGB       & {\bf 0.712}       & 0.682             & {\bf 0.721}       & {\bf 0.589}         & 0.306             & {\bf 0.840}               & {\bf 0.623}       & {\bf 0.639}      \\
  PFA                         &                   & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.585             &    -       \\
  SurfEmb                     &                   & RGB       & 0.640             & {\bf 0.686}       & 0.687             & 0.573               & {\bf 0.363}       & 0.760                     & 0.620             & 0.618      \\
  Cosypose                    &                   & RGB       & 0.606             & 0.589             & 0.664             & 0.559               & 0.177             & 0.634                     & 0.554             & 0.540     \\
  CDPNv2                      &                   & RGB       & 0.612             & 0.338             & 0.577             & 0.438               & 0.087             & 0.708                     & 0.399             & 0.451     \\
  \midrule
  {\bf PFA + Ours}            & \cmark            & RGB       & {\bf 0.712}       & {\bf 0.749}       & {\bf 0.820}       & {\bf 0.589}         & {\bf 0.306}       & {\bf 0.840}               & 0.809             & {\bf 0.689}  \\
  PFA                         & \cmark            & RGB       & 0.673             & -                 &   -               &   -                 &   -               & -                         & 0.742             &    -       \\
  CIR                         & \cmark            & RGB       & 0.633             & 0.684             & -                 &  -                  & -                 & -                         & {\bf 0.835}       & -         \\
  Cosypose                    & \cmark            & RGB       & 0.606             & 0.695             & 0.807             & 0.559               & 0.177             & 0.634                     & 0.842             & 0.617    \\
  CDPNv2                      & \cmark            & RGB       & 0.612             & 0.426             & 0.793             & 0.438               & 0.087             &0.708                      & 0.570             & 0.519\\
  \midrule
  {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.807}       & {\bf 0.930}       & {\bf 0.692}         & 0.495             & {\bf 0.879}               & {\bf 0.867}       & {\bf 0.788}      \\
  PFA                         & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.842            &    -       \\
  SurfEmb                     & \cmark            & RGB-D     & 0.809             & 0.829             & 0.891             & 0.677               & {\bf 0.558}       & 0.875                     & 0.849             & 0.784      \\
  CDPNv2+ICP                  & \cmark            & RGB-D     & 0.689             & 0.449             & 0.847             & 0.458               & 0.206             & 0.757                     & 0.603             & 0.573    \\
  \midrule
  {\bf PFA + Ours}            & \cmark            & RGB-D     & {\bf 0.843}       & {\bf 0.856}       & {\bf 0.986}       & {\bf 0.692}         & {\bf 0.495}       & {\bf 0.879}               & 0.920             & {\bf 0.810}      \\
  PFA                         & \cmark            & RGB-D     & 0.798             & -                 &   -               &   -                 &   -               & -                         & 0.852             &    -       \\
  CIR                      & \cmark            & RGB-D     & 0.778             & 0.773             & 0.991             & 0.688               & 0.379             & 0.753                     & {\bf 0.924}       & 0.755 \\ 
  Cosypose+ICP                &\cmark             & RGB-D     & 0.748             & 0.749             & 0.972             & 0.652               & 0.341             & 0.719                     & 0.903             & 0.726  \\
  CDPNv2+ICP                  & \cmark            & RGB-D     & 0.689             & 0.489             & 0.962             & 0.458               & 0.206             & 0.757                     & 0.701             & 0.609    \\
  \bottomrule
\end{tabular}

==> tabs/compare_allpose_vsd.tex <==
% \begin{tabular}{lll|lllllll|l}
%   \toprule
%   Method                      & Real        & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$   & ITODD$^{\ast}$      & HB$^{\ast}$         & YCB-V             & Avg.\\
%   \midrule
%   {\bf PFA + Ours}            &             & RGB       & {\bf 0.559}       & {\bf 0.643}       & {\bf 0.594}       & {\bf 0.521}       & 0.269               & {\bf 0.804}         & {\bf 0.550}       & {\bf 0.563}     \\
%   PFA~\cite{pfa}              &             & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.522             &   -       \\
%   SurfEmb~\cite{surfemb}      &             & RGB       & 0.497             & 0.661             & 0.569             & 0.514             & {\bf 0.324}         & 0.725               & 0.548             & 0.548     \\
%   Cosypose~\cite{cosypose}    &             & RGB       & 0.480             & 0.571             & 0.544             & 0.515             & 0.172               & 0.613               & 0.516             & 0.487  \\
%   CDPNv2~\cite{cdpn}          &             & RGB       & 0.445             & 0.303             & 0.391             & 0.399             & 0.059               & 0.614               & 0.260             & 0.353     \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark      & RGB       & {\bf 0.559}       & {\bf 0.709}       & {\bf 0.719}       & {\bf 0.521}       & {\bf 0.269}         & {\bf 0.804}         & 0.751             & {\bf 0.619} \\
%   PFA~\cite{pfa}              & \cmark      & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.694             &   -       \\
%   CIR~\cite{coupled_iterative}& \cmark      & RGB       & 0.501             & 0.663             & -                 & -                 & -                   & -                   & {\bf 0.783}       & -     \\
%   Cosypose~\cite{cosypose}    & \cmark      & RGB       & 0.480             & 0.669             & 0.689             & 0.515             & 0.172               & 0.613               & 0.772             & 0.559  \\
%   % SurfEmb~\cite{surfemb}      & \cmark             & RGB       & 0.497             & -                 & -                 & 0.514                     & 0.324                     &0.725                      & -                 & -     \\
%   CDPNv2~\cite{cdpn}          & \cmark      & RGB       & 0.445             & 0.386             & 0.597             & 0.399             & 0.059               & 0.614               & 0.396             & 0.414 \\
%   \midrule
%   {\bf PFA + Ours}            &             & RGB-D     & {\bf 0.658}       & 0.764             & {\bf 0.821}       & {\bf 0.636}       & {\bf 0.413}         & {\bf 0.839}         & {\bf 0.792}       & {\bf 0.703}     \\
%   PFA~\cite{pfa}              &             & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.775             &   -       \\
%   SurfEmb~\cite{surfemb}      &             & RGB-D     & 0.615             & {\bf 0.797}       & 0.767             & 0.621             & 0.497               & 0.829               & 0.757             & 0.698     \\
%   CDPNv2+ICP~\cite{cdpn}      &             & RGB-D     & 0.469             & 0.368             & 0.698             & 0.433             & 0.168               & 0.629               & 0.511             & 0.468     \\
%   \midrule
%   {\bf PFA + Ours}            & \cmark      & RGB-D     & {\bf 0.658}       & {\bf 0.816}       & 0.904             & 0.636             & {\bf 0.413}         & {\bf 0.839}         & 0.863             & {\bf 0.733}     \\
%   PFA~\cite{pfa}              & \cmark      & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.803             &   -       \\
%   CIR~\cite{coupled_iterative}& \cmark      & RGB-D     & 0.601             & 0.760             & {\bf 0.920}       & {\bf 0.656}       & 0.394               & 0.760               & {\bf 0.871}       & 0.709\\
%   % SurfEmb~\cite{surfemb}      \cmark&             & R-DGB      & 0.615             & -                 & -                 & 0.621                     & 0.497                     & 0.829                     & -                 & 0.698     \\
%   Cosypose+ICP~\cite{cosypose}& \cmark      & RGB-D     & 0.567             & 0.587             & 0.869             & 0.624             & 0.282               & 0.679               & 0.831             & 0.634\\
%   CDPNv2+ICP~\cite{cdpn}      & \cmark      & RGB-D     & 0.469             & 0.385             & 0.832             & 0.433             & 0.168               & 0.629               & 0.590             & 0.501     \\
%   \bottomrule
% \end{tabular}


\begin{tabular}{lll|lllllll|l}
  \toprule
  Method                      & Real        & Data      & LM-O$^{\ast}$     & T-LESS             & TUD-L            & IC-BIN$^{\ast}$   & ITODD$^{\ast}$      & HB$^{\ast}$         & YCB-V             & Avg.\\
  \midrule
  {\bf PFA + Ours}            &             & RGB       & {\bf 0.559}       & {\bf 0.643}       & {\bf 0.594}       & {\bf 0.521}       & 0.269               & {\bf 0.804}         & {\bf 0.550}       & {\bf 0.563}     \\
  PFA                         &             & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.522             &   -       \\
  SurfEmb                     &             & RGB       & 0.497             & 0.661             & 0.569             & 0.514             & {\bf 0.324}         & 0.725               & 0.548             & 0.548     \\
  Cosypose                    &             & RGB       & 0.480             & 0.571             & 0.544             & 0.515             & 0.172               & 0.613               & 0.516             & 0.487  \\
  CDPNv2                      &             & RGB       & 0.445             & 0.303             & 0.391             & 0.399             & 0.059               & 0.614               & 0.260             & 0.353     \\
  \midrule
  {\bf PFA + Ours}            & \cmark      & RGB       & {\bf 0.559}       & {\bf 0.709}       & {\bf 0.719}       & {\bf 0.521}       & {\bf 0.269}         & {\bf 0.804}         & 0.751             & {\bf 0.619} \\
  PFA                         & \cmark      & RGB       & 0.531             & -                 &   -               &   -               &   -                 & -                   & 0.694             &   -       \\
  CIR                         & \cmark      & RGB       & 0.501             & 0.663             & -                 & -                 & -                   & -                   & {\bf 0.783}       & -     \\
  Cosypose                    & \cmark      & RGB       & 0.480             & 0.669             & 0.689             & 0.515             & 0.172               & 0.613               & 0.772             & 0.559  \\
  % SurfEmb~\cite{surfemb}      & \cmark             & RGB       & 0.497             & -                 & -                 & 0.514                     & 0.324                     &0.725                      & -                 & -     \\
  CDPNv2                      & \cmark      & RGB       & 0.445             & 0.386             & 0.597             & 0.399             & 0.059               & 0.614               & 0.396             & 0.414 \\
  \midrule
  {\bf PFA + Ours}            &             & RGB-D     & {\bf 0.658}       & 0.764             & {\bf 0.821}       & {\bf 0.636}       & 0.413              & {\bf 0.839}         & {\bf 0.792}       & {\bf 0.703}     \\
  PFA                         &             & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.775             &   -       \\
  SurfEmb                     &             & RGB-D     & 0.615             & {\bf 0.797}       & 0.767             & 0.621             & {\bf 0.497}         & 0.829               & 0.757             & 0.698     \\
  CDPNv2+ICP                  &             & RGB-D     & 0.469             & 0.368             & 0.698             & 0.433             & 0.168               & 0.629               & 0.511             & 0.468     \\
  \midrule
  {\bf PFA + Ours}            & \cmark      & RGB-D     & {\bf 0.658}       & {\bf 0.816}       & 0.904             & 0.636             & {\bf 0.413}         & {\bf 0.839}         & 0.863             & {\bf 0.733}     \\
  PFA                         & \cmark      & RGB-D     & 0.621             & -                 &   -               &   -               &   -                 & -                   & 0.803             &   -       \\
  CIR                         & \cmark      & RGB-D     & 0.601             & 0.760             & {\bf 0.920}       & {\bf 0.656}       & 0.394               & 0.760               & {\bf 0.871}       & 0.709\\
  % SurfEmb~\cite{surfemb}      \cmark&             & R-DGB      & 0.615             & -                 & -                 & 0.621                     & 0.497                     & 0.829                     & -                 & 0.698     \\
  Cosypose+ICP                & \cmark      & RGB-D     & 0.567             & 0.587             & 0.869             & 0.624             & 0.282               & 0.679               & 0.831             & 0.634\\
  CDPNv2+ICP                  & \cmark      & RGB-D     & 0.469             & 0.385             & 0.832             & 0.433             & 0.168               & 0.629               & 0.590             & 0.501     \\
  \bottomrule
\end{tabular}

==> tabs/compare_coco_cityscapes.tex <==
\begin{tabular}{lccc}
    \toprule
    Method                        & AP        & AP$_{50}$ & AP$_{75}$       \\
    \midrule
    FCOS\cite{fcosv2}             & 38.9      &  \underline{57.5}     & 42.2          \\ 
    ATSS\cite{ATSS}             & 39.2      &  57.3     & 42.4          \\ 
    PAA\cite{PAA}                 & {\bf 40.4}      &  {\bf 58.4}     & {\bf 43.9}         \\
    % AutoAssign\cite{autoassign}  & 40.4      &  59.6     & 43.7         \\
    \textbf{Ours}              & \underline{40.0}      &  57.1     & \underline{43.4}      \\
    % \midrule
    % \multirow{5}{*}{Cityscapes} & FCOS~\cite{fcosv2}                &38.0          & 63.1           & 38.6         \\ 
    %     ～                      & ATSS~\cite{ATSS}                  &39.5          & 63.9           & 40.3          \\ 
    %      ～                      &PAA~\cite{PAA}                    &40.0          & \textbf{65.4}  & \textbf{40.8}  \\ 
    %       ～                     &   AutoAssign~\cite{autoassign}   &29.5          & 50.7           & 29.3                     \\
    %                             &\textbf{RADet}                 &\textbf{40.2} & 64.6           & 40.1             \\
    \bottomrule
\end{tabular}

==> tabs/compare_detect_more.tex <==
% \begin{tabular}{c|ccc|ccc|ccc}
% \toprule
%     \multirow{2}{*}{Data}    & \multicolumn{2}{c|}{{\bf Ours}}    &  \multicolumn{2}{c|}{FCOSv2} & \multicolumn{2}{c}{Mask R-CNN} \\
%     ~       & AP$_{50}$     & AP$_{75}$         & AP$_{50}$     & AP$_{75}$      & AP$_{50}$     & AP$_{75}$ \\
%     \midrule
%     LM-O    &{\bf 94.2}     &{\bf 80.7}         &   90.0        & 62.8          &87.2           &  64.7\\
%     T-LESS  & 88.9          & {\bf 86.4}        &{\bf 89.1}          & 80.6          &   83.9        &  75.3  \\
%     TUD-L   & {\bf 100.0}         & {\bf 97.9}        & {\bf 100.0}       & 97.8          & {\bf 100.0}       &    96.8    \\
%     IC-BIN  & {\bf 88.2}          &  {\bf 75.9}       &   50.0        & 27.1          & 74.6          & 39.8   \\
%     ITODD   & {\bf 62.3}    & {\bf 55.4}        & 40.5          & 34.0         & 50.2          & 40.5  \\
%     HB      &{\bf 89.7}     & {\bf 81.7}        &  81.9         & 63.8          & 86.8          & 69.3       \\
%     YCB-V   & {\bf 99.4}    & {\bf 97.4}        & 98.6          & 89.1          &  92.7         & 84.2       \\
%     Avg.    & {\bf 89.0}    & {\bf 82.2}         & 78.6         & 65.0        & 82.2          & 67.2      \\
%     \bottomrule
% \end{tabular}  


% \begin{tabular}{c|ccc|ccc|ccc}
%   \toprule
%   \multirow{2}{*}{Data}    & \multicolumn{3}{c|}{AP}                        &  \multicolumn{3}{c|}{AP$_{50}$}   & \multicolumn{3}{c}{AP$_{75}$} \\
% %   ~                        & Ours & FCOSv2  & Mask R-CNN                    & Ours & FCOSv2  & Mask R-CNN       & Ours & FCOSv2  & Mask R-CNN\\
%     ~           & {\bf Ours} & ~\cite{fcosv2}  & ~\cite{maskrcnn}    & {\bf Ours} & ~\cite{fcosv2}  & ~\cite{maskrcnn} & {\bf Ours} & ~\cite{fcosv2}  & ~\cite{maskrcnn}\\
%   \midrule
%   LM-O                     & {\bf 67.5} &57.0&56.6&{\bf 94.2}     & 90.0          & 87.2          &{\bf 80.7}     & 62.8  & 64.7\\
%   T-LESS                   & {\bf 79.8} &75.0&69.3& 88.9          & {\bf 89.1}    & 83.9          & {\bf 86.4}    & 80.6  & 75.3  \\
%   TUD-L                    & {\bf 86.6} &86.0&82.6& {\bf 100.0}   & {\bf 100.0}   & {\bf 100.0}   & {\bf 97.9}    & 97.8  & 96.8    \\
%   IC-BIN                   & {\bf 63.8 }&27.2&40.1 & {\bf 88.2}    & 50.0          & 74.6          & {\bf 75.9}    & 27.1  & 39.8   \\
%   ITODD                    & {\bf 48.6} &30.4&36.5& {\bf 62.3}    & 40.5          & 50.2          & {\bf 55.4}    & 34.0  & 40.5  \\
%   HB                       &{\bf 73.5}  &60.4&63.5 &{\bf 89.7}     & 81.9          & 86.8          & {\bf 81.7}    & 63.8  & 69.3       \\
%   YCB-V                    &{\bf 85.0}  &80.0& 74.5& {\bf 99.4}    & 98.6          & 92.7          & {\bf 97.4}    & 89.1  & 84.2       \\
%   Avg.                     &{\bf 72.1}  &66.7&60.5& {\bf 89.0}    & 78.6          & 82.2          & {\bf 82.2}    & 65.0  & 67.2      \\
%   \bottomrule
% \end{tabular}


\begin{tabular}{cccc}
  \toprule
  Data        & {\bf Ours}        & \cite{fcosv2}        & ~\cite{maskrcnn}    \\
  \midrule
  \multicolumn{4}{c}{\textit{AP}}\\
  \midrule
  LM-O                     & {\bf 67.5} &57.0&56.6   \\
  T-LESS                   & {\bf 79.8} &75.0&69.3     \\
  TUD-L                    & {\bf 86.6} &86.0&82.6       \\
  IC-BIN                   & {\bf 63.8 }&27.2&40.1      \\
  ITODD                    & {\bf 48.6} &30.4&36.5     \\
  HB                       &{\bf 73.5}  &60.4&63.5          \\
  YCB-V                    &{\bf 85.0}  &80.0& 74.5         \\
  Avg.                     &{\bf 72.1}  &66.7&60.5         \\
  \midrule
  \multicolumn{4}{c}{\textit{AP$_{50}$}}\\
  \midrule
  LM-O                     &{\bf 94.2}     & 90.0          & 87.2        \\
  T-LESS                   & 88.9          & {\bf 89.1}    & 83.9          \\
  TUD-L                    & {\bf 100.0}   & {\bf 100.0}   & {\bf 100.0}     \\
  IC-BIN                   & {\bf 88.2}    & 50.0          & 74.6           \\
  ITODD                    & {\bf 62.3}    & 40.5          & 50.2          \\
  HB                       &{\bf 89.7}     & 81.9          & 86.8               \\
  YCB-V                    & {\bf 99.4}    & 98.6          & 92.7               \\
  Avg.                     & {\bf 89.0}    & 78.6          & 82.2              \\
  \midrule
  \multicolumn{4}{c}{\textit{AP$_{75}$}}\\
  \midrule
  LM-O                    &{\bf 80.7}     & 62.8  & 64.7\\
  T-LESS                  & {\bf 86.4}    & 80.6  & 75.3  \\
  TUD-L                   & {\bf 97.9}    & 97.8  & 96.8    \\
  IC-BIN                   & {\bf 75.9}    & 27.1  & 39.8   \\
  ITODD                   & {\bf 55.4}    & 34.0  & 40.5  \\
  HB                       & {\bf 81.7}    & 63.8  & 69.3       \\
  YCB-V                    & {\bf 97.4}    & 89.1  & 84.2       \\
  Avg.                    & {\bf 82.2}    & 65.0  & 67.2      \\
\bottomrule
\end{tabular}

==> tabs/compare_detector_ap50.tex <==
\begin{tabular}{c|ccccccc|c}
    \toprule
    Method      & LM-O       & T-LESS   & TUD-L     & IC-BIN    & ITODD     & HB        & YCB-V     & Avg.  \\
    \midrule
    Ours        & {\bf 94.2}& 88.9      & {\bf 100.0} & {\bf 88.2}& {\bf 62.3}& {\bf 89.7}& {\bf 99.4}&{\bf 89.0}     \\
    FCOSv2      & 90.0      & {\bf 89.1}& {\bf 100.0} & 50.0      & 40.5      & 81.9      & 98.6      &78.6  \\
    Mask R-CNN  & 87.2      & 83.9      & {\bf 100.0} & 74.6      & 50.2      & 86.8      & 92.7      &82.2    \\
    \bottomrule
\end{tabular}

==> tabs/compare_detector_ap75.tex <==
\begin{tabular}{c|ccccccc|c}
    \toprule
    Method      & LM-O          & T-LESS        & TUD-L         & IC-BIN    & ITODD     & HB        & YCB-V         & Avg.  \\
    \midrule
    Ours        & {\bf 80.7}    & {\bf 86.4}    & {\bf 97.9}    & {\bf 75.9}& {\bf 55.4}& {\bf 81.7}& {\bf 97.4}    & {\bf 82.2}     \\
    FCOSv2      & 62.8          & 80.6          & 97.8          & 27.1      & 34.0      & 63.8      & 89.1          & 65.0   \\
    Mask R-CNN  & 64.7          & 75.3          & 96.8          & 39.8      & 40.5      & 69.3      & 84.2          & 67.2  \\
    \bottomrule
\end{tabular}

==> tabs/compare_estimator.tex <==
\begin{tabular}{cc|ccccccc|c}
    \toprule
    Method                      & Real          & LM-O              & T-LESS            & TUD-L             & IC-BIN            & ITODD             & HB                & YCB-V     & Avg.\\
    \midrule
    \textbf{WDR+Ours}          &               & 0.614             & \textbf{0.588}    & \textbf{0.623}    & 0.514             & \textbf{0.247}    & 0.618             & \textbf{0.605}    & \textbf{0.544} \\
    CDPNv2~\cite{cdpn}          &               & \textbf{0.624}    & 0.407             & 0.588             & 0.473             & 0.102             & \textbf{0.722}    & 0.390             & 0.472 \\
    EPOS~\cite{epos}            &               & 0.547             & 0.467             & 0.558             & 0.363             & 0.186             & 0.580             & 0.499             & 0.457  \\
    CosyPose\dag~\cite{cosypose}&               & 0.533             & 0.520             & 0.582             & \textbf{0.515}    & 0.129             & 0.334             & 0.333             & 0.421 \\
    \midrule
    \textbf{WDR+Ours}          & \cmark    & 0.614             & \textbf{0.678}    & \textbf{0.796}    & 0.514             & \textbf{0.247}    & 0.618             & \textbf{0.722}    & \textbf{0.598} \\
    CDPNv2~\cite{cdpn}          & \cmark    & \textbf{0.624}    & 0.478             & 0.772             & 0.473             & 0.102             & \textbf{0.722}    & 0.532             & 0.529 \\
    CosyPose\dag~\cite{cosypose}& \cmark    & 0.533             & 0.616             & 0.742             & \textbf{0.515}    & 0.129             & 0.334             & 0.655             & 0.503 \\
    Pix2Pose~\cite{pix2pose}    & \cmark    & 0.363             & 0.344             & 0.420             & 0.226             & 0.134             & 0.346             & 0.446             & 0.342 \\
    % SO-Pose~\cite{so-pose}      & \checkmark    & 0.613             & -                 & -                 & -                 & -                 &   -               & 0.715             & -      \\
    \bottomrule
\end{tabular}

==> tabs/compare_ycbv_lmo.tex <==
\begin{tabular}{c|c|cccccc}
    \toprule
        Data & Metric    &CDPNv2~\cite{cdpn}     & NCF~\cite{ncf}   & SurfEmb~\cite{surfemb}    & CIR~\cite{coupled_iterative}    &PFA~\cite{pfa}   & \textbf{RADet+PFA} \\
    \midrule
        \multirow{4}{*}{LM-O}           & MSPD          & 0.815     & -     & 0.851      & 0.831    & 0.821 &\textbf{0.876}\\
        ~                              & MSSD           & 0.612     & -     & 0.641      & 0.633    & 0.674 &\textbf{0.712} \\
        ~                              & VSD       & 0.445	    & -     & 0.497     & 0.501     & 0.531 & \textbf{0.559} \\
        ~                              & Avg.      & 0.624     & 0.632 & 0.663      & 0.655    & 0.676 & \textbf{0.715}\\
    \midrule
        \multirow{4}{*}{YCB-V}          & MSPD      & 0.511    & -      & \textbf{0.773}      & -     & 0.736      &\underline{0.771}  \\
        ~                              & MSSD      & 0.399    &-       & 0.620      & -     & 0.583      & \textbf{0.623} \\
        ~                              & VSD       & 0.260    &-       & 0.548      & -     & 0.524    & \textbf{0.550}    \\
        ~                               & Avg.      & 0.390    & \textbf{0.673}& 0.647      & -     & 0.614     & \underline{0.648}       \\
    \midrule
        \multirow{4}{*}{\makecell[c]{YCB-V\\(with Real)}}& MSPD     & 0.631 &-     & -        & \underline{0.852}    &  -        & \textbf{0.856}  \\
        ~                                             & MSSD      & 0.570 &-   &  -        & \textbf{0.835}     &    -     &\underline{0.809} \\
        ~                                             & VSD       & 0.396 &-   &  -        & \textbf{0.783}     &    -     & \underline{0.751}    \\
        ~                                           & Avg.      & 0.532 & 0.775    &  0.711    & \textbf{0.824}     &-       & \underline{0.806}       \\
    
    \bottomrule
 \end{tabular}

==> tabs/detector_for_onestage.tex <==
\begin{tabular}{lcccc}
    \toprule
      Method          & Avg.      &  MSPD     & MSSD   & VSD  \\
    \midrule
    \multicolumn{5}{c}{on LM-O}\\
    \midrule
    WDR         & 0.544    & 0.758    & 0.501    & 0.373  \\
    WDR+Detect   & 0.614    & 0.841    & 0.559    & 0.441   \\
    EPOS        & 0.547    & 0.750    & 0.501    & 0.389     \\
    EPOS+Detect  & 0.605    & 0.832    & 0.552    & 0.431     \\
    \midrule
    \multicolumn{5}{c}{on YCB-V}\\
    \midrule
    WDR         & 0.514     & 0.632    & 0.491    & 0.420  \\
    WDR+Detect  & 0.605     & 0.694    & 0.598    & 0.522   \\
    EPOS        & 0.499     & 0.621    & 0.464    & 0.411  \\
    EPOS+Detect & 0.572     & 0.675    & 0.536    & 0.506     \\
    \bottomrule
\end{tabular}

==> tabs/distance_transform_acc.tex <==
\begin{tabular}{c|c}
     &  \\
    LM-O  & 
    YCB-V
\end{tabular}

==> tabs/effect_detect.tex <==
\begin{tabular}{lcccc}
    \toprule
      Method          & Avg.      &  MSPD     & MSSD   & VSD  \\
    % \midrule
    % \multicolumn{5}{c}{on LM-O}\\
    % \midrule
    % WDR         & 0.544    & 0.758    & 0.501    & 0.373  \\
    % Detect + WDR   & 0.614    & 0.841    & 0.559    & 0.441   \\
    % EPOS        & 0.547    & 0.750    & 0.501    & 0.389     \\
    % Detect + EPOS  & 0.605    & 0.832    & 0.552    & 0.431     \\
    % \midrule
    % \multicolumn{5}{c}{on YCB-V}\\
    \midrule
    WDR             & 0.514     & 0.631     & 0.492     & 0.420 \\
    % WDR (960)             & 0.558     & 0.682     & 0.543     & 0.450\\
    % WDR (1280)            & \underline{0.594}     & {\bf 0.719}     & \underline{0.587}     & \underline{0.476}\\
    WDR + FCOS          & 0.707             & 0.785             & 0.708         & 0.629\\
    WDR + RCNN          & 0.705             & 0.779             & 0.704         & 0.631\\
    WDR + GT            & {\bf 0.724}       & {\bf 0.800}       & {\bf 0.723}         & {\bf 0.648} \\
    WDR + {\bf Ours}    & \underline{0.722}     & \underline{0.798}         & {\bf 0.723}    & \underline{0.647}   \\
    \cmidrule{2-5}
    CDPNv2 + FCOS       & 0.402             & 0.523             & 0.416         & 0.268 \\
    CDPNv2 + RCNN       & 0.388             & 0.506             & 0.401         & 0.258\\
    CDPNv2 + GT         & {\bf 0.412}       & {\bf 0.536}       & \underline{0.425}         & {\bf 0.275}\\
    CDPNv2 + {\bf Ours} & {\bf 0.412}       & \underline{0.534} & {\bf 0.428}   & {\bf 0.275}\\

    % EPOS        & 0.499     & 0.621    & 0.464    & 0.411  \\
    % EPOS + {\bf Ours}  & {\bf 0.572}     & {\bf 0.675}    & {\bf 0.536}    & {\bf 0.506}     \\
    \bottomrule
\end{tabular}

==> tabs/efficiency.tex <==
\begin{tabular}{ccc}
    \toprule
                    & WDR(1280) & Detect+WDR\\
    \midrule
    \multicolumn{3}{c}{Testing Speed(fps)} \\
    \midrule
    LM-O            & 3.58    & 6.46\\
    YCB-V           &  2.96     & 8.71\\
    \midrule
    \multicolumn{3}{c}{Training Time(hours)}\\
    \midrule
                    & 73.42     &  18.71\\
    \bottomrule
\end{tabular}

==> tabs/resolution_for_wdr.tex <==
\begin{tabular}{ccccc}
    \toprule
    resolution      & Avg.      &  MSPD     & MSSD   & VSD  \\
    % \midrule
    % \multicolumn{5}{c}{on LM-O}\\
    % \midrule
    % 640             & 0.544       &0.758    & 0.501   & 0.373  \\
    % 960             & 0.583       &0.800     & 0.541  & 0.408     \\
    % 1280            & 0.608       &0.829     & 0.566  & 0.430\\
    % \midrule
    % \multicolumn{5}{c}{on YCB-V}\\
    \midrule
    640             & 0.514     & 0.631     & 0.492     & 0.420 \\
    960             & 0.558     & 0.682     & 0.543     & 0.450\\
    1280            & 0.594     & 0.719     & 0.587     & 0.476\\
    \bottomrule
\end{tabular}

==> tabs/time_report.tex <==
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cccccc}
    \toprule
        & FCOS & ATSS & PAA & AutoAssign & {\bf Ours} \\
    \midrule
        Timings & {\bf 0.67} & {\bf 0.67}  & 0.90  &  0.95        & \underline{0.80}   \\
    \bottomrule
\end{tabular}
}

==> tabs/visibilty_modling_acc.tex <==
\begin{tabular}{c|ccccc}
    \toprule
    Threshold($\tau$)  & 0.1   & 0.2   & 0.3   & 0.4   & 0.5 \\
    \midrule    
    LM-O    & 60.3  & 68.8  & 63.4  & 52.7  & 48.3 \\
    YCB-V   & 58.4  & 67.3  & 72.1  & 59.6   & 52.1   \\
    \bottomrule
\end{tabular}

==> tabs/ycbv_compare.tex <==

\begin{tabular}{c|c|ccc|cc}
    \hline
    method                      & backbone               & AP           & AP$_{50}$     & AP$_{75}$     & AP$_{m}$      & AP$_{l}$     \\ \hline
    FCOS\cite{fcosv2}           & ResNet-50              & 76.6         & 94.0          &  88.8         & 72.9          &  77.0        \\ 
    ATSS\cite{ATSS}             & ResNet-50              & 76.5         & 92.5          &  89.2         & 77.7          &  76.8        \\ 
    PAA\cite{PAA}           & ResNet-50              & 77.9         & 94.5          &  88.0         &\textbf{78.1}  &  78.2        \\
    AutoAssign\cite{autoassign} & ResNet-50              & 60.6         & 76.0          &  68.0         & 64.4          &  61.2        \\ 
    \textbf{Mask}               & ResNet-50              &\textbf{79.7} &\textbf{96.3}  &\textbf{90.5}  & 74.9          & \textbf{80.1}\\ 
    \textbf{Distance}           & ResNet-50              & 78.2         & 93.2          & 90.1          & 75.8          & 78.6         \\ \hline
    FCOS\cite{fcosv2}           & ResNet-101             & 81.8         & 96.5          &  93.8         & 79.3          &  82.1     \\
    ATSS\cite{ATSS}             & ResNet-101             & 79.9         & 94.5          &  92.2         & 77.2          &  80.4     \\
    PAA\cite{PAA}           & ResNet-101             & 81.3         & 96.9          &  93.9         & 74.3          &  81.6     \\
    AutoAssign\cite{autoassign} & ResNet-101             & 65.7         & 82.1          &  75.0         & 63.6          &  65.7     \\
    \textbf{Mask}               & ResNet-101             &              &               &               &               &           \\ 
    \textbf{Mask\dag}           & ResNet-101             & 81.9         &  96.4         &  93.6         & 73.1          &  82.4    \\ 
    \textbf{Distance}           & ResNet-101             &              &               &               &               &           \\ 
    \textbf{Distance\dag}       & ResNet-101             & 80.3         &  95.1         &  91.2         & 69.5          &  80.7     \\ \hline
\end{tabular}
\caption{Ycb-video dataset}




==> tabs/ycbv_compare_r50.tex <==


% \rowcolors{2}{white}{gray!10}
\begin{tabular}{lccc}
    \toprule
    Method                              & AP             & AP$_{50}$     & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    AutoAssign~\cite{autoassign}        & 61.6            & 76.8         & 69.8         \\%& 64.0$\pm$0.18          &  62.1$\pm$0.41     \\
    FCOS~\cite{fcosv2}                  & 63.8            & 82.1         & 72.4        \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    Faster R-CNN~\cite{faster-rcnn}     & 66.1            & 87.9         & 75.5 \\
    PAA~\cite{PAA}                      & 66.9            & 86.6         & 73.8         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19     \\
    ATSS~\cite{ATSS}                    & 67.8            & 85.8         & 77.0         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    \cmidrule{2-4}
    \textbf{Ours-box}                   & 66.1            & 84.6         & 74.8 \\
    \textbf{Ours-center}                & 67.2            & 83.9         & 75.8       \\
    % \textbf{Ours-mask$^\dagger$}        & 68.8            & 86.1         & 78.4         \\ 
    \textbf{Ours-nofusion}              & 69.0              & 88.7          & 77.5\\
    \textbf{Ours}                       & \underline{69.6}& \underline{88.5}& \underline{78.7}        \\
    \textbf{Ours-oracle}              &\textbf{71.2}    & \textbf{91.7} &\textbf{79.9}\\
    % \textbf{Mask (oracle)}               & real               & \textbf{71.2}$\pm$0.27   & \textbf{91.7}$\pm$\textbf{0.08}& \textbf{79.9}$\pm$0.50\\%& 63.2$\pm$0.17          &  \textbf{71.8$\pm$0.31}    \\ 
    % \midrule
    % Faster R-CNN                & real+sync          & 77.2$\pm$0.80            &96.6$\pm$0.77           & 90.8$\pm$0.15          \\
    % FCOS                        & real+sync          & 76.6$\pm$0.83            & 94.0$\pm$0.76          &  88.8$\pm$0.83          \\%& 72.9$\pm$0.21          &  77.0$\pm$0.78        \\ 
    % ATSS                        & real+sync          & 76.3$\pm$0.24            & 92.4$\pm$0.14          &  88.4$\pm$0.82          \\%& 77.7$\pm$0.05          &  76.7$\pm$0.19        \\ 
    % PAA                         & real+sync          & 77.9$\pm$0.13            & 94.5$\pm$0.21          &  88.0$\pm$0.49          \\%&\textbf{78.1$\pm$0.91}  &  78.2$\pm$0.19        \\
    % AutoAssign                  & real+sync          & 60.6$\pm$0.11            & 76.2$\pm$0.23          &  67.8$\pm$0.18          \\%& 64.2$\pm$0.32          &  61.2$\pm$0.07        \\ 
    % \textbf{Ours}               & real+sync          & \textbf{78.2$\pm$0.07}   & \textbf{93.2$\pm$0.04} &  \textbf{90.1$\pm$0.12}          \\%& 75.8$\pm$0.67          & 78.6$\pm$0.05         \\ \hline
    % \textbf{Mask (oracle)}               & real+sync          &\textbf{79.7}$\pm$0.35 &\textbf{96.3}$\pm$0.19  &\textbf{90.5}$\pm$0.80   \\%& 74.9$\pm$0.22          & \textbf{80.1$\pm$0.30}\\ 
    \bottomrule
\end{tabular}




==> tabs/ycbv_compare_r50_mixpbr.tex <==
\begin{tabular}{ccc}
    Method              &  AP       & AP_{50}      & AP_{75}   \\
    
    {\bf Ours-box}      &           &               &           \\
    {\bf Ours-center}   &           &               &           \\
    {\bf Ours-nofusion} & 
    {\bf Ours}          & 85.0      & 99.4          & 97.4      \\
    {\bf Ours-oracle}   & 86.3      &               &           \\
\end{tabular}


\begin{tabular}{lccc}
    \toprule
    Method                              & AP             & AP$_{50}$     & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    AutoAssign~\cite{autoassign}        & 61.6            & 76.8         & 69.8         \\%& 64.0$\pm$0.18          &  62.1$\pm$0.41     \\
    FCOS~\cite{fcosv2}                  & 63.8            & 82.1         & 72.4        \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    Faster R-CNN~\cite{faster-rcnn}     & 66.1            & 87.9         & 75.5 \\
    PAA~\cite{PAA}                      & 66.9            & 86.6         & 73.8         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19     \\
    ATSS~\cite{ATSS}                    & 67.8            & 85.8         & 77.0         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    \cmidrule{2-4}
    \textbf{Ours-box}                   & 66.1            & 84.6         & 74.8 \\
    \textbf{Ours-center}                & 67.2            & 83.9         & 75.8       \\
    % \textbf{Ours-mask$^\dagger$}        & 68.8            & 86.1         & 78.4         \\ 
    \textbf{Ours-nofusion}              & 69.0              & 88.7          & 77.5\\
    \textbf{Ours}                       & \underline{69.6}& \underline{88.5}& \underline{78.7}        \\
    \textbf{Ours-oracle}              &\textbf{71.2}    & \textbf{91.7} &\textbf{79.9}\\
    % \textbf{Mask (oracle)}               & real               & \textbf{71.2}$\pm$0.27   & \textbf{91.7}$\pm$\textbf{0.08}& \textbf{79.9}$\pm$0.50\\%& 63.2$\pm$0.17          &  \textbf{71.8$\pm$0.31}    \\ 
    % \midrule
    % Faster R-CNN                & real+sync          & 77.2$\pm$0.80            &96.6$\pm$0.77           & 90.8$\pm$0.15          \\
    % FCOS                        & real+sync          & 76.6$\pm$0.83            & 94.0$\pm$0.76          &  88.8$\pm$0.83          \\%& 72.9$\pm$0.21          &  77.0$\pm$0.78        \\ 
    % ATSS                        & real+sync          & 76.3$\pm$0.24            & 92.4$\pm$0.14          &  88.4$\pm$0.82          \\%& 77.7$\pm$0.05          &  76.7$\pm$0.19        \\ 
    % PAA                         & real+sync          & 77.9$\pm$0.13            & 94.5$\pm$0.21          &  88.0$\pm$0.49          \\%&\textbf{78.1$\pm$0.91}  &  78.2$\pm$0.19        \\
    % AutoAssign                  & real+sync          & 60.6$\pm$0.11            & 76.2$\pm$0.23          &  67.8$\pm$0.18          \\%& 64.2$\pm$0.32          &  61.2$\pm$0.07        \\ 
    % \textbf{Ours}               & real+sync          & \textbf{78.2$\pm$0.07}   & \textbf{93.2$\pm$0.04} &  \textbf{90.1$\pm$0.12}          \\%& 75.8$\pm$0.67          & 78.6$\pm$0.05         \\ \hline
    % \textbf{Mask (oracle)}               & real+sync          &\textbf{79.7}$\pm$0.35 &\textbf{96.3}$\pm$0.19  &\textbf{90.5}$\pm$0.80   \\%& 74.9$\pm$0.22          & \textbf{80.1$\pm$0.30}\\ 
    \bottomrule
\end{tabular}


==> tabs/ycbv_compare_real.tex <==

\begin{tabular}{c|c|ccc|cc}
    \hline
    method                      & data                   & AP           & AP$_{50}$     & AP$_{75}$     & AP$_{m}$      & AP$_{l}$     \\ \hline
    FCOS\cite{fcosv2}           & ResNet-50              & 63.8         & 82.1          &  72.4         & 64.2          &  64.4        \\ 
    ATSS\cite{ATSS}             & ResNet-50              & 68.8         & 86.8          &  78.0         & 65.5          &  69.3        \\ 
    PAA\cite{PAA}               & ResNet-50              & 66.9         & 86.6          &  73.8         & 61.9          &  67.6        \\
    AutoAssign\cite{autoassign} & ResNet-50              & 61.6         & 76.8          &  69.8         & 64.0          &  62.1        \\ 
    \textbf{Mask\dag}           & ResNet-50              &\textbf{71.2} &\textbf{91.7}  &\textbf{79.9}  & 63.2          & \textbf{71.8} \\ 
    \textbf{Distance\dag}       & ResNet-50              & 69.6         & 88.5          &  78.7         & 63.9          &  70.0         \\ \hline
    FCOS\cite{fcosv2}           & ResNet-101             & 65.1         & 83.3          &  73.6         & 59.5          &   66.0         \\
    ATSS\cite{ATSS}             & ResNet-101             & 70.0         & 88.5          &    78.9       &  64.3         &  70.3          \\
    PAA\cite{PAA}               & ResNet-101             & 71.0         & 91.0          &    80.3       &  64.1         &  71.4           \\
    AutoAssign\cite{autoassign} & ResNet-101             &              &               &               &               &                    \\
    \textbf{Mask\dag}           & ResNet-101             &  72.4        &  91.6         &  82.9         &  63.8         &  72.9            \\ 
    \textbf{Distance\dag}       & ResNet-101             &              &               &               &               &           \\ \hline
\end{tabular}
\caption{Ycb-video real dataset}




==> tabs/ycbv_compare_resnext50.tex <==
\begin{tabular}{lcccc}
    \toprule
    method                      & data               & AP                                        & AP$_{50}$                    & AP$_{75}$     \\%& AP$_{m}$      & AP$_{l}$     \\ \hline
    \midrule
    Faster R-CNN                & real               & 67.0$\pm$0.15                             & 88.5$\pm$0.31                & 77.6$\pm$0.34                \\
    FCOS                        & real               & 61.0$\pm$0.19                             & 80.3$\pm$0.33                & 72.4$\pm$0.09         \\%& 64.2$\pm$0.48          &  64.4$\pm$0.11     \\
    ATSS                        & real               & 65.2$\pm$0.45                             & 83.2$\pm$0.52                & 78.0$\pm$0.09         \\%& \textbf{65.5$\pm$0.50} &  69.3$\pm$0.04     \\
    PAA                         & real               & 63.4$\pm$0.38                             & 81.6$\pm$0.42                & 73.8$\pm$0.27         \\%& 61.9$\pm$0.14          &  67.6$\pm$0.19     \\
    \textbf{Ours}               & real               & \textbf{68.9$\pm$0.16}                     & \textbf{88.7$\pm$0.16}    &  \textbf{78.7$\pm$0.25}        \\%& 63.9$\pm$0.15          &  70.0$\pm$0.15     \\ \hline
   
    \midrule
    Faster R-CNN                & real+sync          & 77.4$\pm$0.16                             &  93.2$\pm$0.17               & 88.7$\pm$0.21                           \\
    FCOS                        & real+sync          & 73.9$\pm$0.07                             &  89.2$\pm$0.30               &83.4$\pm$0.26\\%& 72.9$\pm$0.21          &  77.0$\pm$0.78        \\ 
    ATSS                        & real+sync          & 78.6$\pm$0.25                             &  93.8$\pm$0.15               &90.4$\pm$0.54\\%& 77.7$\pm$0.05          &  76.7$\pm$0.19        \\ 
    PAA                         & real+sync          & 77.3$\pm$0.16                             &  94.0$\pm$0.33               &88.8$\pm$0.55\\%&\textbf{78.1$\pm$0.91}  &  78.2$\pm$0.19        \\
    \textbf{Ours}                & real+sync          & \textbf{79.1$\pm$0.18}                    & \textbf{94.8$\pm$0.16}       &\textbf{90.5$\pm$0.21}\\%& 75.8$\pm$0.67          & 78.6$\pm$0.05         \\ \hline
    \bottomrule
\end{tabular}
